Crosstalk Attack Resilient RNS Quantum Addition

As quantum computers scale, the rise of multi-user and cloud-based quantum platforms can lead to new security challenges. Attacks within shared execution environments become increasingly feasible due to the crosstalk noise that, in combination with quantum computer's hardware specifications, can be exploited in form of crosstalk attack. Our work pursues crosstalk attack implementation in ion-trap quantum computers. We propose three novel quantum crosstalk attacks designed for ion trap qubits: (i) Alternate CNOT attack (ii) Superposition Alternate CNOT (SAC) attack (iii) Alternate Phase Change (APC) attack. We demonstrate the effectiveness of proposed attacks by conducting noise-based simulations on a commercial 20-qubit ion-trap quantum computer. The proposed attacks achieve an impressive reduction of up to 42.2% in output probability for Quantum Full Adders (QFA) having 6 to 9-qubit output. Finally, we investigate the possibility of mitigating crosstalk attacks by using Residue Number System (RNS) based Parallel Quantum Addition (PQA). We determine that PQA achieves higher attack resilience against crosstalk attacks in the form of 24.3% to 133.5% improvement in output probability against existing Non Parallel Quantum Addition (NPQA). Through our systematic methodology, we demonstrate how quantum properties such as superposition and phase transition can lead to crosstalk attacks and also how parallel quantum computing can help secure against these attacks.

==> ISCAS2024_Xtalk_attack_RNS_distributed_quantum/latex_images/quantikz_figures1.tex <==
\usepackage{tikz}
\usepackage{quantikz}
\usepackage{amsmath}


\newcommand{\rowSep}{0.6cm}
\newcommand{\colSep}{0.2cm}

\newcommand{\myCnot}{
\begin{quantikz} [row sep= \rowSep, column sep= \colSep]
	\lstick{$a$} & \qw	& \ctrl{1} & \qw & \rstick{$a$}\\
	\lstick{$b$} & \qw	& \targ{}  & \qw & \rstick{$a \oplus b$}
\end{quantikz}
}

\newcommand{\myToffoli}{
\begin{quantikz} [row sep= \rowSep, column sep= \colSep]
	\lstick{$a$} & \ctrl{1} & \qw & \rstick{$a$} \\
	\lstick{$b$} & \ctrl{1} & \qw & \rstick{$b$} \\
	\lstick{$c$} & \targ{}  & \qw & \rstick{$a \cdot b \oplus c$}
\end{quantikz}
}

\newcommand{\QMAone}{
%\begin{quantikz} [row sep= 0.06cm, column sep= 0.025cm, transparent]
	%\gategroup[17,steps=22,style={blue!75!black, ultra thick, dashed, rounded corners, inner xsep=2pt}, background]{{\sc Quantum Full Adder}}
\begin{quantikz} [row sep= {0.5cm, between origins}, column sep= {0.05cm}, transparent]
	\lstick{$\ket{0}$}   & \qw	& \qw\gategroup[17,steps=22,style={blue!75!black, ultra thick, dashed, rounded corners, inner xsep=-2pt}, background]{{\sc Quantum Full Adder}}		& \qw		& \qw	    & \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw	& \qw		& \qw	& \qw	& \qw	& \qw\gategroup[17,steps=3,style={green!50!black, ultra thick, dashed, rounded corners, inner xsep=-3pt}, background]{{\sc NOR}} 		& \targ{}	& \qw 		& \qw	& \qw	& \qw	& \qw	& \qw\gategroup[17,steps=22,style={blue!75!black, ultra thick, dashed, rounded corners, inner xsep=-2pt}, background]{{\sc Quantum Full Adder}} 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw		& \qw 		& \qw 		& \targ{}	& \qw & \rstick{$m_0$} \\
	\lstick{$a_0$} 		 & \qw	& \qw	    & \qw	   	& \qw		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw		& \qw 		& \qw      & \targ{}	& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw 		& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \qw		& \qw 		& \qw 		& \ctrl{-1}	& \qw & \rstick{$s_0$} \\
	\lstick{$b_0$} 		 & \qw	& \qw	    & \qw 	   	& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \qw		& \qw 		& \qw      & \ctrl{-1}	& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw 		& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_0$} \\
	\lstick{$\ket{0}$}   & \qw	& \qw	    & \qw	   	& \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw 		& \qw	& \qw	& \qw	& \qw	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw		& \qw 		& \targ{}	& \qw & \rstick{$m_1$} \\
	\lstick{$a_1$} 		 & \qw	& \targ{} 	& \qw	   	& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw 		& \qw	& \qw	& \qw	& \qw	& \ctrl{-1}	& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \targ{}	& \ctrl{3}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \ctrl{3}	& \qw		& \qw 		& \ctrl{-1}	& \qw & \rstick{$s_1$} \\
	\lstick{$b_1$} 		 & \qw	& \ctrl{-1} & \qw	   	& \qw 		& \qw 		& \ctrl{3}	& \targ{}	& \ctrl{3}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \ctrl{3}	& \qw 		& \qw      & \ctrl{-1}	& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw 		& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_1$} \\
	\lstick{$\ket{0}$}   & \qw	& \qw	   	& \qw	   	& \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw 		& \qw	& \qw	& \qw	& \qw	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \qw & \rstick{$m_2$} \\
	\lstick{$a_2$} 		 & \qw	& \targ{} 	& \qw	   	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw 		& \qw	& \qw	& \qw	& \qw	& \ctrl{-1}	& \qw 		& \qw 		& \ctrl{3}	& \targ{}	& \qw 		& \targ{}	& \ctrl{3}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \targ{}	& \ctrl{3}	& \qw 		& \ctrl{-1}	& \qw & \rstick{$s_2$} \\
	\lstick{$b_2$} 		 & \qw	& \ctrl{-1} & \qw	   	& \qw 		& \ctrl{3}	& \targ{}	& \qw 		& \targ{}	& \ctrl{3}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \targ{}	& \ctrl{3}	& \qw      & \ctrl{-1}	& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw 		& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_2$} \\
	\lstick{$\ket{0}$}   & \qw	& \qw	   	& \qw	   	& \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw 		& \qw	& \qw	& \qw	& \qw	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \qw & \rstick{$m_3$} \\
	\lstick{$a_3$} 		 & \qw	& \targ{} 	& \qw	   	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw  		& \qw  		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw 		& \qw	& \qw	& \qw	& \qw	& \ctrl{-1}	& \qw 		& \ctrl{5}	& \targ{}	& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{5}	& \qw		& \qw 		& \ctrl{5}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{5}	& \ctrl{-1}	& \qw & \rstick{$s_3$} \\
	\lstick{$b_3$} 		 & \qw	& \ctrl{-1} & \qw	   	& \ctrl{3}  & \targ{}	& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{3}	& \qw  		& \qw  		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{3} & \ctrl{-1}	& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw 		& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_3$} \\
	\lstick{$\ket{0}$}   & \qw	& \qw	   	& \qw	   	& \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw 		& \qw	& \qw	& \qw	& \qw	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \qw & \rstick{$m_4$} \\
	\lstick{$a_4$} 		 & \qw	& \targ{} 	& \qw	   	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}  & \targ{}  	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw      & \targ{}	& \qw	& \qw	& \qw	& \qw	& \targ{}	& \ctrl{-13}& \targ{}	& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$s_4$} \\		
	\lstick{$b_4$} 		 & \qw	& \ctrl{-1} & \ctrl{1}  & \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \ctrl{1}  & \ctrl{-1}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}  & \ctrl{-1}	& \qw	& \qw	& \qw	& \qw	& \qw	 	& \qw		& \qw		& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_4$} \\		
	\lstick{$\ket{0}$}   & \qw	& \qw     	& \targ{}   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw 		& \targ{}  	& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \qw 		& \qw	& \qw	& \qw	& \qw	& \targ{}	& \ctrl{-2}	& \targ{}	& \qw	& \qw	& \qw	& \qw	& \ctrl{-3}	& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{1}	& \ctrl{-3}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{-3}	& \qw & \rstick{$s_5$} \\
	\lstick{$\ket{0}$}   & \qw	& \qw	   	& \qw	   	& \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw	& \qw	& \qw	& \qw	& \qw	 	& \qw		& \qw		& \qw	& \qw	& \qw	& \qw	& \qw 		& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$s_6$}			
\end{quantikz}
}

\newcommand{\QMAtwo}{
%\begin{quantikz} [row sep= 0.02cm, column sep= 0.01cm, transparent]
\begin{quantikz} [row sep= {0.5cm, between origins}, column sep= {0.05cm}, transparent]
	\lstick{$\ket{0}$}  & \qw	 & \qw\gategroup[16,steps=22,style={blue!75!black, ultra thick, dashed, rounded corners, inner xsep=-2pt}, background]{{\sc Quantum Full Adder}}	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw	& \qw	& \qw	& \qw	& \qw\gategroup[16,steps=3,style={green!50!black, ultra thick, dashed, rounded corners, inner xsep=-3pt}, background]{{\sc NOR}} 		& \targ{}	& \qw  		& \qw	& \qw	& \qw	& \qw\gategroup[16,steps=6,style={red!70!green!40!blue!80, ultra thick, dashed, rounded corners, inner xsep=-3pt}, background]{{\sc Half Adder}}	& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$m_0$} \\
	\lstick{$a_0$} 		& \qw	 & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw		& \qw 		& \qw      & \targ{}	& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw  		& \qw	& \qw	& \qw	& \qw	& \ctrl{2}	& \ctrl{-1}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$s_0$} \\
	\lstick{$b_0$} 		& \qw	 & \qw	   & \qw 	   & \qw 		& \qw 		& \qw 		& \ctrl{3}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \qw		& \qw 		& \qw      & \ctrl{-1}	& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw  		& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_0$} \\
	\lstick{$\ket{0}$}  & \qw	 & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw  		& \qw	& \qw	& \qw	& \qw	& \targ{}	& \ctrl{1}	& \targ{  }	& \qw 		& \qw 		& \qw 		& \qw & \rstick{$m_1$} \\
	\lstick{$a_1$} 		& \qw	 & \targ{} & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw  		& \qw	& \qw	& \qw	& \qw	& \qw 		& \ctrl{2}	& \ctrl{-1}	& \qw 		& \qw 		& \qw 		& \qw & \rstick{$s_1$} \\
	\lstick{$b_1$} 		& \qw	& \ctrl{-1}& \qw	   & \qw 		& \qw 		& \ctrl{3}	& \targ{}	& \ctrl{3}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \ctrl{3}	& \qw 		& \qw      & \ctrl{-1}	& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw  		& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_1$} \\
	\lstick{$\ket{0}$}  & \qw	 & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw  		& \qw	& \qw	& \qw	& \qw	& \qw 		& \targ{}	& \ctrl{1}	& \targ{  }	& \qw 		& \qw 		& \qw & \rstick{$m_2$} \\
	\lstick{$a_2$} 		& \qw	& \targ{}  & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw  		& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \qw 		& \qw 		& \qw & \rstick{$s_2$} \\
	\lstick{$b_2$} 		& \qw	& \ctrl{-1}& \qw	   & \qw 		& \ctrl{3}	& \targ{}	& \qw 		& \targ{}	& \ctrl{3}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \targ{}	& \ctrl{3}	& \qw      & \ctrl{-1}	& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw  		& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_2$} \\
	\lstick{$\ket{0}$}  & \qw	 & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw  		& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \targ{}	& \ctrl{1}	& \targ{  }	& \qw 		& \qw & \rstick{$m_3$} \\
	\lstick{$a_3$} 		& \qw	 & \targ{} & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw  		& \qw  		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw  		& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \qw 		& \qw & \rstick{$s_3$} \\
	\lstick{$b_3$} 		& \qw	& \ctrl{-1}& \qw	   & \ctrl{3}  	& \targ{}	& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{3}	& \qw  		& \qw  		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{3} & \ctrl{-1}	& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw  		& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_3$} \\
	\lstick{$\ket{0}$}  & \qw	 & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw  		& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw 		& \targ{}	& \targ{}	& \qw 		& \qw & \rstick{$m_4$} \\
	\lstick{$a_4$} 		& \qw	 & \targ{} & \qw	   & \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}  & \targ{}  	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw      & \targ{}	& \qw	& \qw	& \qw	& \qw	& \targ{}	& \ctrl{-13}& \targ{}	& \qw	& \qw	& \qw	& \qw	& \qw		& \qw 		& \qw 		& \qw 		& \qw		& \qw 		& \qw & \rstick{$s_4$} \\		
	\lstick{$b_4$} 		& \qw	& \ctrl{-1}& \ctrl{1}  & \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \ctrl{1}  & \ctrl{-1}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}  & \ctrl{-1}	& \qw	& \qw	& \qw	& \qw	& \qw	 	& \qw		& \qw  		& \qw	& \qw	& \qw	& \qw	& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_4$} \\		
	\lstick{$\ket{0}$}  & \qw	 & \qw     & \targ{}   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw 		& \targ{}  	& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \qw 		& \qw	& \qw	& \qw	& \qw	& \targ{}	& \ctrl{-2}	& \targ{}	& \qw	& \qw	& \qw	& \qw	& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{-3}	& \qw 		& \qw & \rstick{$s_5$}
\end{quantikz}
}

\newcommand{\QMAtwobk}{
%\begin{quantikz} [row sep= 0.02cm, column sep= 0.01cm, transparent]
\begin{quantikz} [row sep= {0.5cm, between origins}, column sep= {0.05cm}, transparent]
	\lstick{$\ket{0}$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw 		& \targ{}	& \qw  		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$m_0$} \\
	\lstick{$a_0$} & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw		& \qw 		& \qw      & \targ{}	& \qw 		& \qw 		& \qw  		& \ctrl{2}	& \ctrl{-1}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$s_0$} \\
	\lstick{$b_0$} & \qw	   & \qw 	   & \qw 		& \qw 		& \qw 		& \ctrl{3}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \qw		& \qw 		& \qw      & \ctrl{-1}	& \qw 		& \qw 		& \qw  		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_0$} \\
	\lstick{$\ket{0}$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw 		& \qw 		& \qw  		& \targ{}	& \ctrl{1}	& \targ{  }	& \qw 		& \qw 		& \qw 		& \qw & \rstick{$m_1$} \\
	\lstick{$a_1$} & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw 		& \qw 		& \qw  		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \qw 		& \qw 		& \qw 		& \qw & \rstick{$s_1$} \\
	\lstick{$b_1$} & \ctrl{-1} & \qw	   & \qw 		& \qw 		& \ctrl{3}	& \targ{}	& \ctrl{3}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \ctrl{3}	& \qw 		& \qw      & \ctrl{-1}	& \qw 		& \qw 		& \qw  		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_1$} \\
	\lstick{$\ket{0}$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw 		& \qw 		& \qw  		& \qw 		& \targ{}	& \ctrl{1}	& \targ{  }	& \qw 		& \qw 		& \qw & \rstick{$m_2$} \\
	\lstick{$a_2$} & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw 		& \qw 		& \qw  		& \qw 		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \qw 		& \qw 		& \qw & \rstick{$s_2$} \\
	\lstick{$b_2$} & \ctrl{-1} & \qw	   & \qw 		& \ctrl{3}	& \targ{}	& \qw 		& \targ{}	& \ctrl{3}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \targ{}	& \ctrl{3}	& \qw      & \ctrl{-1}	& \qw 		& \qw 		& \qw  		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_2$} \\
	\lstick{$\ket{0}$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw 		& \qw 		& \qw  		& \qw 		& \qw 		& \targ{}	& \ctrl{1}	& \targ{  }	& \qw 		& \qw & \rstick{$m_3$} \\
	\lstick{$a_3$} & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw  		& \qw  		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw 		& \qw 		& \qw  		& \qw 		& \qw 		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \qw 		& \qw & \rstick{$s_3$} \\
	\lstick{$b_3$} & \ctrl{-1} & \qw	   & \ctrl{3}  	& \targ{}	& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{3}	& \qw  		& \qw  		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{3} & \ctrl{-1}	& \qw 		& \qw 		& \qw  		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_3$} \\
	\lstick{$\ket{0}$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw 		& \qw 		& \qw  		& \qw 		& \qw 		& \qw 		& \targ{}	& \targ{}	& \qw 		& \qw & \rstick{$m_4$} \\
	\lstick{$a_4$} & \targ{}   & \qw	   & \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}  & \targ{}  	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw      & \targ{}	& \targ{}	& \ctrl{-13}& \targ{}	& \qw		& \qw 		& \qw 		& \qw 		& \qw		& \qw 		& \qw & \rstick{$s_4$} \\		
	\lstick{$b_4$} & \ctrl{-1} & \ctrl{1}  & \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \ctrl{1}  & \ctrl{-1}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}  & \ctrl{-1}	& \qw	 	& \qw		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_4$} \\		
	\lstick{$\ket{0}$}   & \qw       & \targ{}   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw 		& \targ{}  	& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \qw 		& \targ{}	& \ctrl{-2}	& \targ{}	& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{-3}	& \qw 		& \qw & \rstick{$s_5$}
\end{quantikz}
}


\newcommand{\QMAthree}{
\begin{quantikz} [row sep= {0.5cm, between origins}, column sep= {0.05cm}, transparent]
	\lstick{$\ket{0}$}   	& \qw	    & \qw	   	& \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw	& \qw 		& \targ{}	& \qw  		& \qw				& \ctrl{1}		& \targ{}		& \qw 			& \qw 			& \qw 		& \qw 		& \qw & \rstick{$m_0$} \\
	\lstick{$a_0$} 			& \qw	    & \qw	   	& \qw		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw		& \qw 		& \qw      & \targ{}	& \qw	& \qw 		& \qw 		& \qw  		& \qw				& \ctrl{1}		& \ctrl{-1}		& \qw 			& \qw 			& \qw 		& \qw 		& \qw & \rstick{$s_0$} \\
	\lstick{$b_0$} 			& \qw	    & \qw 	   	& \qw 		& \qw 		& \qw 		& \ctrl{2}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{2}	& \qw		& \qw 		& \qw      & \ctrl{-1}	& \qw	& \qw 		& \qw 		& \qw  		& \gate{\ket{0}}	& \targ{}		& \ctrl{1}		& \targ{  }		& \qw 			& \qw 		& \qw 		& \qw & \rstick{$m_1$} \\
	\lstick{$a_1$} 			& \targ{}   & \qw	   	& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw	& \qw 		& \qw 		& \qw  		& \qw				& \qw 			& \ctrl{1}		& \ctrl{-1}		& \qw 			& \qw 		& \qw 		& \qw & \rstick{$s_1$} \\
	\lstick{$b_1$} 			& \ctrl{-1} & \qw	   	& \qw 		& \qw 		& \ctrl{2}	& \targ{}	& \ctrl{2}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \targ{}	& \ctrl{2}	& \qw 		& \qw      & \ctrl{-1}	& \qw	& \qw 		& \qw 		& \qw  		& \qw				& \gate{\ket{0}}& \targ{}		& \ctrl{1}		& \targ{  }		& \qw 		& \qw 		& \qw & \rstick{$m_2$} \\
	\lstick{$a_2$} 			& \targ{}   & \qw	   	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw	& \qw 		& \qw 		& \qw  		& \qw				& \qw 			& \qw 			& \ctrl{1}		& \ctrl{-1}		& \qw 		& \qw 		& \qw & \rstick{$s_2$} \\
	\lstick{$b_2$} 			& \ctrl{-1} & \qw	   	& \qw 		& \ctrl{2}	& \targ{}	& \qw 		& \targ{}	& \ctrl{2}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \targ{}	& \ctrl{2}	& \qw      & \ctrl{-1}	& \qw	& \qw 		& \qw 		& \qw  		& \qw				& \qw 			& \gate{\ket{0}}& \targ{}		& \ctrl{1}		& \targ{  }	& \qw 		& \qw & \rstick{$m_3$} \\
	\lstick{$a_3$} 			& \targ{}   & \qw	   	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw  		& \qw  		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw	& \qw 		& \qw 		& \qw  		& \qw				& \qw 			& \qw 			& \qw 			& \ctrl{1}		& \ctrl{-1}	& \qw 		& \qw & \rstick{$s_3$} \\
	\lstick{$b_3$} 			& \ctrl{-1} & \qw	   	& \ctrl{2}  & \targ{}	& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{2}	& \qw  		& \qw  		& \ctrl{2}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{2} & \ctrl{-1}	& \qw	& \qw 		& \qw 		& \qw  		& \qw				& \qw 			& \qw 			& \gate{\ket{0}}& \targ{}		& \targ{}	& \qw 		& \qw & \rstick{$m_4$} \\
	\lstick{$a_4$} 			& \targ{}   & \qw	   	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}  & \targ{}  	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw      & \targ{}	& \qw	& \targ{}	& \ctrl{-9} & \targ{}	& \qw				& \qw			& \qw 			& \qw 			& \qw 			& \qw		& \qw 		& \qw & \rstick{$s_4$} \\		
	\lstick{$b_4$} 			& \ctrl{-1} & \ctrl{1}  & \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \ctrl{1}  & \ctrl{-1}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}  & \ctrl{-1}	& \qw	& \qw	 	& \qw		& \qw  		& \qw				& \qw			& \qw 			& \qw 			& \gate{\ket{0}}& \qw 		& \qw 		& \qw & \rstick{$\ket{0}$} \\		
	\lstick{$\ket{0}$}   	& \qw       & \targ{}   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw 		& \targ{}  	& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \qw 		& \qw	& \targ{}	& \ctrl{-2}	& \targ{}	& \qw				& \qw			& \qw 			& \qw 			& \qw 			& \ctrl{-3}	& \qw 		& \qw & \rstick{$s_5$}
\end{quantikz}
}

\newcommand{\QMAfour}{
\begin{quantikz} [row sep= {0.5cm, between origins}, column sep= {0.05cm}, transparent]
	\lstick{$\ket{0}$}   	& \qw	    & \qw	   	& \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw	& \qw				& \qw	& \qw 		& \targ{}	& \qw  		& \qw				& \ctrl{1}		& \targ{}		& \qw 			& \qw 			& \qw 		& \qw 		& \qw & \rstick{$m_0$} \\
	\lstick{$a_0$} 			& \qw	    & \qw	   	& \qw		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw		& \qw 		& \qw      & \targ{}	& \qw	& \qw				& \qw	& \qw 		& \qw 		& \qw  		& \qw				& \ctrl{1}		& \ctrl{-1}		& \qw 			& \qw 			& \qw 		& \qw 		& \qw & \rstick{$s_0$} \\
	\lstick{$b_0$} 			& \qw	    & \qw 	   	& \qw 		& \qw 		& \qw 		& \ctrl{2}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{2}	& \qw		& \qw 		& \qw      & \ctrl{-1}	& \qw	& \gate{\ket{0}}	& \qw	& \qw 		& \qw 		& \qw  		& \gate{\ket{0}}	& \targ{}		& \ctrl{1}		& \targ{  }		& \qw 			& \qw 		& \qw 		& \qw & \rstick{$m_1$} \\
	\lstick{$a_1$} 			& \targ{}   & \qw	   	& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw	& \qw				& \qw	& \qw 		& \qw 		& \qw  		& \qw				& \qw 			& \ctrl{1}		& \ctrl{-1}		& \qw 			& \qw 		& \qw 		& \qw & \rstick{$s_1$} \\
	\lstick{$b_1$} 			& \ctrl{-1} & \qw	   	& \qw 		& \qw 		& \ctrl{2}	& \targ{}	& \ctrl{2}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \targ{}	& \ctrl{2}	& \qw 		& \qw      & \ctrl{-1}	& \qw	& \gate{\ket{0}}	& \qw	& \qw 		& \qw 		& \qw  		& \qw				& \gate{\ket{0}}& \targ{}		& \ctrl{1}		& \targ{  }		& \qw 		& \qw 		& \qw & \rstick{$m_2$} \\
	\lstick{$a_2$} 			& \targ{}   & \qw	   	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw	& \qw				& \qw	& \qw 		& \qw 		& \qw  		& \qw				& \qw 			& \qw 			& \ctrl{1}		& \ctrl{-1}		& \qw 		& \qw 		& \qw & \rstick{$s_2$} \\
	\lstick{$b_2$} 			& \ctrl{-1} & \qw	   	& \qw 		& \ctrl{2}	& \targ{}	& \qw 		& \targ{}	& \ctrl{2}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \targ{}	& \ctrl{2}	& \qw      & \ctrl{-1}	& \qw	& \gate{\ket{0}}	& \qw	& \qw 		& \qw 		& \qw  		& \qw				& \qw 			& \gate{\ket{0}}& \targ{}		& \ctrl{1}		& \targ{  }	& \qw 		& \qw & \rstick{$m_3$} \\
	\lstick{$a_3$} 			& \targ{}   & \qw	   	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw  		& \qw  		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw	& \qw				& \qw	& \qw 		& \qw 		& \qw  		& \qw				& \qw 			& \qw 			& \qw 			& \ctrl{1}		& \ctrl{-1}	& \qw 		& \qw & \rstick{$s_3$} \\
	\lstick{$b_3$} 			& \ctrl{-1} & \qw	   	& \ctrl{2}  & \targ{}	& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{2}	& \qw  		& \qw  		& \ctrl{2}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{2} & \ctrl{-1}	& \qw	& \gate{\ket{0}}	& \qw	& \qw 		& \qw 		& \qw  		& \qw				& \qw 			& \qw 			& \gate{\ket{0}}& \targ{}		& \targ{}	& \qw 		& \qw & \rstick{$m_4$} \\
	\lstick{$a_4$} 			& \targ{}   & \qw	   	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}  & \targ{}  	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw      & \targ{}	& \qw	& \qw				& \qw	& \targ{}	& \ctrl{-9} & \targ{}	& \qw				& \qw			& \qw 			& \qw 			& \qw 			& \qw		& \qw 		& \qw & \rstick{$s_4$} \\		
	\lstick{$b_4$} 			& \ctrl{-1} & \ctrl{1}  & \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \ctrl{1}  & \ctrl{-1}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}  & \ctrl{-1}	& \qw	& \gate{\ket{0}}	& \qw	& \qw	 	& \qw		& \qw  		& \qw				& \qw			& \qw 			& \qw 			& \gate{\ket{0}}& \qw 		& \qw 		& \qw & \rstick{$\ket{0}$} \\		
	\lstick{$\ket{0}$}   	& \qw       & \targ{}   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw 		& \targ{}  	& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \qw 		& \qw	& \qw				& \qw	& \targ{}	& \ctrl{-2}	& \targ{}	& \qw				& \qw			& \qw 			& \qw 			& \qw 			& \ctrl{-3}	& \qw 		& \qw & \rstick{$s_5$}
\end{quantikz}
}

\newcommand{\QMAfourNEW}{
\begin{quantikz} [row sep= {0.5cm, between origins}, column sep= {0.05cm}, transparent]
	\lstick{$\ket{0}$}   	& \qw	    & \qw	   	& \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw	& \qw\gategroup[12,steps=5,style={blue!75!black, ultra thick, dashed, rounded corners, inner xsep=-3pt}, background]{{\sc QMA4 Zero Resets}}	& \qw	& \qw				& \qw	& \qw	& \qw	& \qw 		& \targ{}	& \qw  		& \qw				& \ctrl{1}		& \targ{}		& \qw 			& \qw 			& \qw 		& \qw 		& \qw & \rstick{$m_0$} \\
	\lstick{$a_0$} 			& \qw	    & \qw	   	& \qw		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw		& \qw 		& \qw      & \targ{}	& \qw	& \qw	& \qw	& \qw				& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw  		& \qw				& \ctrl{1}		& \ctrl{-1}		& \qw 			& \qw 			& \qw 		& \qw 		& \qw & \rstick{$s_0$} \\
	\lstick{$b_0$} 			& \qw	    & \qw 	   	& \qw 		& \qw 		& \qw 		& \ctrl{2}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{2}	& \qw		& \qw 		& \qw      & \ctrl{-1}	& \qw	& \qw	& \qw	& \gate{\ket{0}}	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw  		& \gate{\ket{0}}	& \targ{}		& \ctrl{1}		& \targ{  }		& \qw 			& \qw 		& \qw 		& \qw & \rstick{$m_1$} \\
	\lstick{$a_1$} 			& \targ{}   & \qw	   	& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw	& \qw	& \qw	& \qw				& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw  		& \qw				& \qw 			& \ctrl{1}		& \ctrl{-1}		& \qw 			& \qw 		& \qw 		& \qw & \rstick{$s_1$} \\
	\lstick{$b_1$} 			& \ctrl{-1} & \qw	   	& \qw 		& \qw 		& \ctrl{2}	& \targ{}	& \ctrl{2}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \targ{}	& \ctrl{2}	& \qw 		& \qw      & \ctrl{-1}	& \qw	& \qw	& \qw	& \gate{\ket{0}}	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw  		& \qw				& \gate{\ket{0}}& \targ{}		& \ctrl{1}		& \targ{  }		& \qw 		& \qw 		& \qw & \rstick{$m_2$} \\
	\lstick{$a_2$} 			& \targ{}   & \qw	   	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw	& \qw	& \qw	& \qw				& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw  		& \qw				& \qw 			& \qw 			& \ctrl{1}		& \ctrl{-1}		& \qw 		& \qw 		& \qw & \rstick{$s_2$} \\
	\lstick{$b_2$} 			& \ctrl{-1} & \qw	   	& \qw 		& \ctrl{2}	& \targ{}	& \qw 		& \targ{}	& \ctrl{2}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \targ{}	& \ctrl{2}	& \qw      & \ctrl{-1}	& \qw	& \qw	& \qw	& \gate{\ket{0}}	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw  		& \qw				& \qw 			& \gate{\ket{0}}& \targ{}		& \ctrl{1}		& \targ{  }	& \qw 		& \qw & \rstick{$m_3$} \\
	\lstick{$a_3$} 			& \targ{}   & \qw	   	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw  		& \qw  		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw	& \qw	& \qw	& \qw				& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw  		& \qw				& \qw 			& \qw 			& \qw 			& \ctrl{1}		& \ctrl{-1}	& \qw 		& \qw & \rstick{$s_3$} \\
	\lstick{$b_3$} 			& \ctrl{-1} & \qw	   	& \ctrl{2}  & \targ{}	& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{2}	& \qw  		& \qw  		& \ctrl{2}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{2} & \ctrl{-1}	& \qw	& \qw	& \qw	& \gate{\ket{0}}	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw  		& \qw				& \qw 			& \qw 			& \gate{\ket{0}}& \targ{}		& \targ{}	& \qw 		& \qw & \rstick{$m_4$} \\
	\lstick{$a_4$} 			& \targ{}   & \qw	   	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}  & \targ{}  	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw      & \targ{}	& \qw	& \qw	& \qw	& \qw				& \qw	& \qw	& \qw	& \targ{}	& \ctrl{-9} & \targ{}	& \qw				& \qw			& \qw 			& \qw 			& \qw 			& \qw		& \qw 		& \qw & \rstick{$s_4$} \\		
	\lstick{$b_4$} 			& \ctrl{-1} & \ctrl{1}  & \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \ctrl{1}  & \ctrl{-1}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}  & \ctrl{-1}	& \qw	& \qw	& \qw	& \gate{\ket{0}}	& \qw	& \qw	& \qw	& \qw	 	& \qw		& \qw  		& \qw				& \qw			& \qw 			& \qw 			& \gate{\ket{0}}& \qw 		& \qw 		& \qw & \rstick{$\ket{0}$} \\		
	\lstick{$\ket{0}$}   	& \qw       & \targ{}   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw 		& \targ{}  	& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \qw 		& \qw	& \qw	& \qw	& \qw				& \qw	& \qw	& \qw	& \targ{}	& \ctrl{-2}	& \targ{}	& \qw				& \qw			& \qw 			& \qw 			& \qw 			& \ctrl{-3}	& \qw 		& \qw & \rstick{$s_5$}
\end{quantikz}
}

\newcommand{\QMAfourCombined}{
\begin{quantikz} [row sep= {0.5cm, between origins}, column sep= {0.05cm}, transparent]
	\lstick{$\ket{0}$}   	& \qw	    & \qw	   	& \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw	& \qw\gategroup[12,steps=5,style={blue!75!black, ultra thick, dashed, rounded corners, inner xsep=-3pt}, background]{{\sc QMA4 Zero Resets}}	& \qw	& \qw				& \qw	& \qw	& \qw	& \qw 		& \targ{}	& \qw  		& \qw				& \ctrl{1}		& \targ{}		& \qw 			& \qw 			& \qw 		& \qw 		& \qw & \rstick{$m_0$} \\
	\lstick{$a_0$} 			& \qw	    & \qw	   	& \qw		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw		& \qw 		& \qw      & \targ{}	& \qw	& \qw	& \qw	& \qw				& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw  		& \qw				& \ctrl{1}		& \ctrl{-1}		& \qw 			& \qw 			& \qw 		& \qw 		& \qw & \rstick{$s_0$} \\
	\lstick{$b_0$} 			& \qw	    & \qw 	   	& \qw 		& \qw 		& \qw 		& \ctrl{2}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{2}	& \qw		& \qw 		& \qw      & \ctrl{-1}	& \qw	& \qw	& \qw	& \gate{\ket{0}}	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw  		& \gate{\ket{0}}	& \targ{}		& \ctrl{1}		& \targ{  }		& \qw 			& \qw 		& \qw 		& \qw & \rstick{$m_1$} \\
	\lstick{$a_1$} 			& \targ{}   & \qw	   	& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw	& \qw	& \qw	& \qw				& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw  		& \qw				& \qw 			& \ctrl{1}		& \ctrl{-1}		& \qw 			& \qw 		& \qw 		& \qw & \rstick{$s_1$} \\
	\lstick{$b_1$} 			& \ctrl{-1} & \qw	   	& \qw 		& \qw 		& \ctrl{2}	& \targ{}	& \ctrl{2}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \targ{}	& \ctrl{2}	& \qw 		& \qw      & \ctrl{-1}	& \qw	& \qw	& \qw	& \gate{\ket{0}}	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw  		& \qw				& \gate{\ket{0}}& \targ{}		& \ctrl{1}		& \targ{  }		& \qw 		& \qw 		& \qw & \rstick{$m_2$} \\
	\lstick{$a_2$} 			& \targ{}   & \qw	   	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw	& \qw	& \qw	& \qw				& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw  		& \qw				& \qw 			& \qw 			& \ctrl{1}		& \ctrl{-1}		& \qw 		& \qw 		& \qw & \rstick{$s_2$} \\
	\lstick{$b_2$} 			& \ctrl{-1} & \qw	   	& \qw 		& \ctrl{2}	& \targ{}	& \qw 		& \targ{}	& \ctrl{2}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \targ{}	& \ctrl{2}	& \qw      & \ctrl{-1}	& \qw	& \qw	& \qw	& \gate{\ket{0}}	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw  		& \qw				& \qw 			& \gate{\ket{0}}& \targ{}		& \ctrl{1}		& \targ{  }	& \qw 		& \qw & \rstick{$m_3$} \\
	\lstick{$a_3$} 			& \targ{}   & \qw	   	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw  		& \qw  		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw	& \qw	& \qw	& \qw				& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw  		& \qw				& \qw 			& \qw 			& \qw 			& \ctrl{1}		& \ctrl{-1}	& \qw 		& \qw & \rstick{$s_3$} \\
	\lstick{$b_3$} 			& \ctrl{-1} & \qw	   	& \ctrl{2}  & \targ{}	& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{2}	& \qw  		& \qw  		& \ctrl{2}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{2} & \ctrl{-1}	& \qw	& \qw	& \qw	& \gate{\ket{0}}	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw  		& \qw				& \qw 			& \qw 			& \gate{\ket{0}}& \targ{}		& \targ{}	& \qw 		& \qw & \rstick{$m_4$} \\
	\lstick{$a_4$} 			& \targ{}   & \qw	   	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}  & \targ{}  	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw      & \targ{}	& \qw	& \qw	& \qw	& \qw				& \qw	& \qw	& \qw	& \targ{}	& \ctrl{-9} & \targ{}	& \qw				& \qw			& \qw 			& \qw 			& \qw 			& \qw		& \qw 		& \qw & \rstick{$s_4$} \\		
	\lstick{$b_4$} 			& \ctrl{-1} & \ctrl{1}  & \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \ctrl{1}  & \ctrl{-1}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}  & \ctrl{-1}	& \qw	& \qw	& \qw	& \gate{\ket{0}}	& \qw	& \qw	& \qw	& \qw	 	& \qw		& \qw  		& \qw				& \qw			& \qw 			& \qw 			& \gate{\ket{0}}& \qw 		& \qw 		& \qw & \rstick{$\ket{0}$} \\		
	\lstick{$\ket{0}$}   	& \qw       & \targ{}   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw 		& \targ{}  	& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \qw 		& \qw	& \qw	& \qw	& \qw				& \qw	& \qw	& \qw	& \targ{}	& \ctrl{-2}	& \targ{}	& \qw				& \qw			& \qw 			& \qw 			& \qw 			& \ctrl{-3}	& \qw 		& \qw & \rstick{$s_5$}
\end{quantikz}
}

==> ISCAS2024_Xtalk_attack_RNS_distributed_quantum/latex_images/quantikz_figures2.tex <==
\usepackage{tikz}
\usepackage{quantikz}
\usepackage{amsmath}

\newcommand{\rowSep}{0.25cm}
\newcommand{\colSep}{0.2cm}


\newcommand{\myCnot}{
\begin{quantikz} [row sep= \rowSep, column sep= \colSep]
	\lstick{$a$} & \ctrl{1} & \qw & \rstick{$a$}\\
	\lstick{$b$} & \targ{}  & \qw & \rstick{$a \oplus b$}
\end{quantikz}
}

\newcommand{\mySwap}{
\begin{quantikz}
	\qw & \swap{1} & \qw \\
	\qw & \targX{} & \qw
\end{quantikz} = \begin{quantikz}
	\qw & \ctrl{1} & \targ{} 	& \ctrl{1} & \qw \\
	\qw & \targ{}  & \ctrl{-1} 	& \targ{}  & \qw
\end{quantikz}
}

\newcommand{\myToffoli}{
\begin{quantikz} [row sep= \rowSep, column sep= \colSep]
	\lstick{$a$} & \ctrl{1} & \qw & \rstick{$a$} \\
	\lstick{$b$} & \ctrl{1} & \qw & \rstick{$b$} \\
	\lstick{$c$} & \targ{}  & \qw & \rstick{$a \cdot b \oplus c$}
\end{quantikz}
}

\newcommand{\ModFour}{
	\begin{quantikz} [row sep= \rowSep, column sep= \colSep, transparent]
		\lstick{$A_0$} & \ctrl{1} 	& \targ{}	&	\rstick{$M_0$} \\
		\lstick{$B_0$} & \ctrl{1} 	& \ctrl{-1}	&	\rstick{$B_0$} \\
		\lstick{$A_1$} & \targ{}  	& \targ{}	&	\rstick{$M_1$} \\
		\lstick{$B_1$} & \qw		& \ctrl{-1}	&	\rstick{$B_1$} 
	\end{quantikz}
}

\newcommand{\ModEight}{
\begin{quantikz} [row sep= \rowSep, column sep= \colSep, transparent]
	\lstick{$A_0$} & \qw	    & \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw		& \targ{}	& \rstick{$M_0$} \\
	\lstick{$B_0$} & \qw 	   	& \qw 		& \ctrl{2}	& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{2}	& \qw		& \ctrl{-1}	& \rstick{$B_0$} \\
	\lstick{$A_1$} & \targ{}   	& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \targ{}	& \rstick{$M_1$} \\
	\lstick{$B_1$} & \ctrl{-1} 	& \ctrl{2}	& \targ{}	& \ctrl{2}	& \qw 		& \ctrl{2}	& \ctrl{-1}	& \targ{}	& \ctrl{2}	& \ctrl{-1}	& \rstick{$B_1$} \\
	\lstick{$A_2$} & \targ{}   	& \qw 		& \qw 		& \qw 		& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \rstick{$M_2$} \\
	\lstick{$B_2$} & \ctrl{-1} 	& \targ{}	& \qw 		& \targ{}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \targ{}	& \ctrl{-1}	& \rstick{$B_2$} 
\end{quantikz}
}

\newcommand{\KimModuloAdder}{
	\begin{quantikz} [row sep= \rowSep, column sep= \colSep, transparent]
		\lstick{$0$}   & \targ{}	& \qw		& \ctrl{2}	& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{2}	& \targ{}	& \targ{}	& \ctrl{2}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{2}	& \qw		& \qw		& \qw		& \ctrl{2}		& \targ{}	& \qw  & \rstick{$0$} \\
		\lstick{$a_0$} & \ctrl{1} 	& \ctrl{1} 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		&  \qw 	 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 	 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		&  \qw 	  	& \ctrl{1} 	& \ctrl{2} 	& \ctrl{1} 	& \qw 		 	& \qw 		& \qw  & \rstick{$a_0$} \\
		\lstick{$b_0$} & \ctrl{1}	& \targ{}	& \ctrl{1}	& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}	& \qw		& \qw		& \ctrl{1}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1} 	& \targ{} 	& \ctrl{1} 	& \targ{} 	& \targ{} 		& \qw		& \qw  & \rstick{$s_0$} \\
		\lstick{$0$}   & \targ{}	& \qw		& \targ{}	& \ctrl{2}	& \qw		& \qw		& \qw		& \ctrl{2}	& \targ{}	& \qw		& \qw		& \targ{}	& \ctrl{2}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{2}	& \qw		& \qw		& \qw		& \ctrl{2}	& \targ{}	& \qw		& \targ{}	& \qw		& \qw			& \qw		& \qw  & \rstick{$c_1$} \\
		\lstick{$a_1$} & \ctrl{1} 	& \ctrl{1} 	& \qw 		&  \qw 	 	& \qw 		& \qw 		& \qw 		&  \qw 	 	& \qw 		& \qw 		& \qw 		& \qw 		&  \qw 	 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 	 	& \qw 		& \qw 		&  \qw 	  	& \ctrl{1} 	& \ctrl{2} 	& \ctrl{1} 	& \qw 		& \qw 		& \qw	 	& \qw		& \qw		& \qw 			& \qw 		& \qw  & \rstick{$a_1$} \\
		\lstick{$b_1$} & \ctrl{1} 	& \targ{} 	& \qw 		& \ctrl{1} 	& \qw 		& \qw 		& \qw 		& \ctrl{1} 	& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1} 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 	 	& \qw 		& \qw 		& \ctrl{1} 	& \targ{} 	& \ctrl{1} 	& \targ{} 	& \targ{} 	& \qw 		& \qw	 	& \qw		& \qw		& \qw 			& \qw 		& \qw  & \rstick{$s_1$} \\
		\lstick{$0$}   & \targ{}	& \qw		& \qw		& \targ{}	& \ctrl{2}	& \qw		& \ctrl{2}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \targ{}	& \ctrl{2}	& \qw		& \ctrl{2}	& \qw		& \qw		& \qw		& \ctrl{2}	& \targ{}	& \qw		& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw			& \qw		& \qw  & \rstick{$c_2$} \\
		\lstick{$a_2$} & \ctrl{1} 	& \ctrl{1} 	& \qw 		& \qw 		&  \qw 	 	& \qw 		&  \qw 	 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		&  \qw 	 	& \qw 		&  \qw 	  	& \ctrl{1} 	& \ctrl{2} 	& \ctrl{1} 	& \qw 		& \qw 		& \qw	 	& \qw 		& \qw	 	& \qw 		& \qw 		& \qw	 	& \qw 		& \qw	 	& \qw 			& \qw 		& \qw  & \rstick{$a_2$} \\
		\lstick{$b_2$} & \ctrl{1} 	& \targ{} 	& \qw 		& \qw 		& \ctrl{1} 	& \qw 		& \ctrl{1} 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1} 	& \qw 		& \ctrl{1} 	& \targ{} 	& \ctrl{1} 	& \targ{} 	& \targ{} 	& \qw 		& \qw	 	& \qw 		& \qw	 	& \qw 		& \qw 		& \qw	 	& \qw 		& \qw	 	& \qw 			& \qw 		& \qw  & \rstick{$s_2$} \\
		\lstick{$0$}   & \targ{}	& \qw		& \qw		& \qw		& \targ{}	& \ctrl{2}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \ctrl{2}	& \targ{}	& \qw		& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw			& \qw		& \qw  & \rstick{$c_3$} \\
		\lstick{$a_3$} & \ctrl{1} 	& \ctrl{1} 	& \qw 		& \qw 		& \qw 		&  \qw 	 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 	 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw	 	& \qw 		& \qw	 	& \qw 		& \qw 		& \qw	 	& \qw 		& \qw	 	& \qw 			& \qw 		& \qw  & \rstick{$a_3$} \\
		\lstick{$b_3$} & \ctrl{1} 	& \targ{} 	& \qw 		& \qw 		& \qw 		& \ctrl{1} 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{} 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw	 	& \qw 		& \qw	 	& \qw 		& \qw 		& \qw	 	& \qw 		& \qw	 	& \qw 			& \qw 		& \qw  & \rstick{$s_3$} \\
		\lstick{$0$}   & \targ{} 	& \qw 		& \qw 		& \qw 		& \qw 		& \targ{} 	& \qw 		& \qw 		& \qw 		& \ctrl{-12}& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw	 	& \qw 		& \qw	 	& \qw 		& \qw 		& \qw	 	& \qw 		& \qw	 	& \qw 			& \ctrl{-12}& \qw  & \rstick{$c_4$}
	\end{quantikz}
}

\newcommand{\KimModuloAdderThree}{
	\begin{quantikz} [row sep= \rowSep, column sep= \colSep, transparent]
		\lstick{$0$}   & \targ{}	& \qw		& \ctrl{2}	& \qw		& \ctrl{2}	& \targ{}	& \targ{}	& \ctrl{2}	& \qw		& \ctrl{2}	& \qw		& \qw		& \qw		& \ctrl{2}	& \targ{}	& \qw		& \rstick{$0$} \\
		\lstick{$A_0$} & \ctrl{1} 	& \ctrl{1} 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		&  \qw 	 	& \ctrl{1}	& \ctrl{1}	& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \rstick{$A_0$} \\
		\lstick{$B_0$} & \ctrl{1}	& \targ{}	& \ctrl{1}	& \qw		& \ctrl{1}	& \qw		& \qw		& \ctrl{1}	& \qw		& \ctrl{1}	& \targ{}	& \ctrl{1}	& \targ{}	& \targ{}	& \qw		& \qw		& \rstick{$M_0$} \\
		\lstick{$0$}   & \targ{}	& \qw		& \targ{}	& \ctrl{2}	& \targ{}	& \qw		& \qw		& \targ{}	& \ctrl{2}	& \targ{}	& \qw		& \targ{}	& \qw		& \qw		& \qw		& \qw		& \rstick{$Carry_0$} \\
		\lstick{$A_1$} & \ctrl{1} 	& \ctrl{1} 	& \qw 		&  \qw 	 	& \qw 		& \qw 		& \qw		& \qw 		& \qw 	 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 	 	& \qw 		& \qw 		& \rstick{$A_1$} \\
		\lstick{$B_1$} & \ctrl{1} 	& \targ{} 	& \qw 		& \ctrl{1} 	& \qw 		& \qw 		& \qw		& \qw 		& \targ{} 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw	 	& \qw 		& \qw 		& \rstick{$M_1$} \\
		\lstick{$0$}   & \targ{}	& \qw		& \qw		& \targ{}	& \qw		& \ctrl{-6}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{-6}	& \qw		& \rstick{$Carry_1$}
	\end{quantikz}
}

\newcommand{\ProposedModuloAdderThree}{
	\begin{quantikz} [row sep= \rowSep, column sep= \colSep, transparent]
		\lstick{$0$}   & \qw		& \qw		& \targ{}	& \qw		& \ctrl{2}	& \targ{}	&\rstick{$M_0$}   \\
		\lstick{$A_0$} & \ctrl{1}	& \ctrl{1}	& \qw		& \qw		& \qw		& \qw		&\rstick{$A_0$} \\
		\lstick{$B_0$} & \ctrl{2}	& \targ{}	& \qw		& \qw		& \ctrl{1}	& \ctrl{-2}	&\rstick{$S_0$} \\
		\lstick{$0$}   & \qw		& \qw		& \qw		& \targ{}	& \targ{}	& \qw		&\rstick{$M_1$} \\
		\lstick{$0$}   & \targ{}	& \targ{}	& \ctrl{-4}	& \qw		& \targ{}	& \qw		&\rstick{$Carry_1$} \\
		\lstick{$0$}   & \qw		& \targ{}	& \ctrl{-1}	& \qw		& \qw		& \qw		&\rstick{$\overline{A_1}.\overline{B_1}$} \\
		\lstick{$A_1$} & \targ{}	& \ctrl{-1}	& \targ{}	& \ctrl{-3}	& \qw		& \qw		&\rstick{$A_1$} \\
		\lstick{$B_1$} & \targ{}	& \ctrl{-1}	& \targ{}	& \ctrl{-1}	& \qw		& \qw		&\rstick{$B_1$}
	\end{quantikz}
}

\newcommand{\ProposedModuloAdderNine}{
	\begin{quantikz} [row sep= \rowSep, column sep= \colSep, transparent]
		\lstick{$0$}   & \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \qw		& \ctrl{1}	& \qw		& \qw		& \targ{}	& \rstick{$M_0$} \\
		\lstick{$A_0$} & \qw		& \qw		& \qw		& \ctrl{1}	& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}	& \qw		& \targ{}	& \qw		& \qw		& \ctrl{2}	& \qw		& \qw		& \ctrl{-1}	& \rstick{$S_0$} \\
		\lstick{$B_0$} & \qw		& \qw		& \qw		& \ctrl{3}	& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{3}	& \qw		& \ctrl{-1}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \rstick{$B_0$} \\
		\lstick{$0$}   & \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \ctrl{1}	& \qw		& \targ{}	& \rstick{$M_1$} \\
		\lstick{$A_1$} & \targ{}	& \qw		& \qw		& \qw		& \ctrl{1}	& \qw		& \qw		& \ctrl{1}	& \targ{}	& \qw		& \qw		& \targ{}	& \qw		& \qw		& \qw		& \ctrl{2}	& \qw		& \ctrl{-1}	& \rstick{$S_1$} \\
		\lstick{$B_1$} & \ctrl{-1}	& \qw		& \ctrl{3}	& \targ{}	& \ctrl{3}	& \qw		& \qw		& \ctrl{3}	& \ctrl{-1} & \targ{}	& \ctrl{3}	& \ctrl{-1}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \rstick{$B_1$} \\
		\lstick{$0$}   & \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \ctrl{1}	& \targ{}	& \rstick{$M_2$} \\
		\lstick{$A_2$} & \targ{}	& \qw		& \qw		& \qw		& \qw		& \ctrl{1}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \targ{}	& \qw		& \qw		& \qw		& \qw		& \ctrl{2}	& \ctrl{-1}	& \rstick{$S_2$} \\
		\lstick{$B_2$} & \ctrl{-1}	& \ctrl{2}	& \targ{}	& \qw		& \targ{}	& \ctrl{2}	& \ctrl{-1}	& \targ{}	& \qw		& \qw		& \targ{}	& \ctrl{-1}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \rstick{$B_2$} \\
		\lstick{$0$}   & \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \qw		& \targ{}	& \qw		& \rstick{$M_3$} \\
		\lstick{$0$}   & \qw		& \targ{}	& \qw		& \qw		& \qw		& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \ctrl{-10}& \targ{}	& \qw		& \qw		& \qw		& \qw		& \rstick{$Carry_3$} \\
		\lstick{$0$}   & \qw		& \qw		& \qw		& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \ctrl{-1}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \rstick{$\overline{A_3}.\overline{B_3}$} \\
		\lstick{$A_3$} & \qw		& \qw		& \targ{}	& \ctrl{-1}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{-3}	& \qw		& \qw		& \qw		& \rstick{$A_3$} \\
		\lstick{$B_3$} & \qw		& \qw		& \targ{}	& \ctrl{-1}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{-1}	& \qw		& \qw		& \qw		& \rstick{$B_3$} \\
	\end{quantikz}
}


==> ISCAS2024_Xtalk_attack_RNS_distributed_quantum/latex_images/quantikz_figures_bk.tex <==
\usepackage{tikz}
\usepackage{quantikz}
\usepackage{amsmath}

\newcommand{\rowSep}{0.25cm}
\newcommand{\colSep}{0.2cm}


\newcommand{\myCnot}{
\begin{quantikz} [row sep= \rowSep, column sep= \colSep]
	\lstick{$a$} & \ctrl{1} & \qw & \rstick{$a$}\\
	\lstick{$b$} & \targ{}  & \qw & \rstick{$a \oplus b$}
\end{quantikz}
}

\newcommand{\mySwap}{
\begin{quantikz}
	\qw & \swap{1} & \qw \\
	\qw & \targX{} & \qw
\end{quantikz} = \begin{quantikz}
	\qw & \ctrl{1} & \targ{} 	& \ctrl{1} & \qw \\
	\qw & \targ{}  & \ctrl{-1} 	& \targ{}  & \qw
\end{quantikz}
}

\newcommand{\myToffoli}{
\begin{quantikz} [row sep= \rowSep, column sep= \colSep]
	\lstick{$a$} & \ctrl{1} & \qw & \rstick{$a$} \\
	\lstick{$b$} & \ctrl{1} & \qw & \rstick{$b$} \\
	\lstick{$c$} & \targ{}  & \qw & \rstick{$a \cdot b \oplus c$}
\end{quantikz}
}

\newcommand{\KimModuloAdderBoxed}{
\begin{quantikz} [row sep= 0.2cm, column sep= 0.17cm, transparent]
	\lstick{$0$}   & \targ{} &\qw	& \qw\gategroup[13,steps=9,style={blue!75!black, ultra thick, dashed, rounded corners, inner xsep=2pt}, background]{{\sc QRCA based Carry Generation Logic}}
												& \qw		& \ctrl{2}	& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{2}	& \qw  & \targ{}	& \targ{}	& \qw	& \ctrl{2}\gategroup[13,steps=19,style={green!50!black, ultra thick, dashed, rounded corners, inner xsep=2pt}, background]{{\sc QRCA based Carryout Truncated Full Adder}}		
																																																	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{2}	& \qw		& \qw		& \qw		& \ctrl{2}		& \qw  & \targ{}	& \qw  & \rstick{$0$} \\
	\lstick{$a_0$} & \qw  	 &\qw	& \ctrl{1} 	& \ctrl{1} 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		&  \qw 	 	& \qw  & \qw 		& \qw 		& \qw	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 	 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		&  \qw 	  	& \ctrl{1} 	& \ctrl{2} 	& \ctrl{1} 	& \qw 		 	& \qw  & \qw 		& \qw  & \rstick{$a_0$} \\
	\lstick{$b_0$} & \qw  	 &\qw	& \ctrl{1}	& \targ{}	& \ctrl{1}	& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}	& \qw  & \qw		& \qw		& \qw	& \ctrl{1}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1} 	& \targ{} 	& \ctrl{1} 	& \targ{} 	& \targ{} 		& \qw  & \qw		& \qw  & \rstick{$s_0$} \\
	\lstick{$0$}   & \qw  	 &\qw	& \targ{}	& \qw		& \targ{}	& \ctrl{2}	& \qw		& \qw		& \qw		& \ctrl{2}	& \targ{}	& \qw  & \qw		& \qw		& \qw	& \targ{}	& \ctrl{2}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{2}	& \qw		& \qw		& \qw		& \ctrl{2}	& \targ{}	& \qw		& \targ{}	& \qw		& \qw			& \qw  & \qw		& \qw  & \rstick{$c_1$} \\
	\lstick{$a_1$} & \qw  	 &\qw	& \ctrl{1} 	& \ctrl{1} 	& \qw 		&  \qw 	 	& \qw 		& \qw 		& \qw 		&  \qw 	 	& \qw 		& \qw  & \qw 		& \qw 		& \qw	& \qw 		&  \qw 	 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 	 	& \qw 		& \qw 		&  \qw 	  	& \ctrl{1} 	& \ctrl{2} 	& \ctrl{1} 	& \qw 		& \qw 		& \qw	 	& \qw		& \qw		& \qw 			& \qw  & \qw 		& \qw  & \rstick{$a_1$} \\
	\lstick{$b_1$} & \qw  	 &\qw	& \ctrl{1} 	& \targ{} 	& \qw 		& \ctrl{1} 	& \qw 		& \qw 		& \qw 		& \ctrl{1} 	& \qw 		& \qw  & \qw 		& \qw 		& \qw	& \qw 		& \ctrl{1} 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 	 	& \qw 		& \qw 		& \ctrl{1} 	& \targ{} 	& \ctrl{1} 	& \targ{} 	& \targ{} 	& \qw 		& \qw	 	& \qw		& \qw		& \qw 			& \qw  & \qw 		& \qw  & \rstick{$s_1$} \\
	\lstick{$0$}   & \qw  	 &\qw	& \targ{}	& \qw		& \qw		& \targ{}	& \ctrl{2}	& \qw		& \ctrl{2}	& \targ{}	& \qw		& \qw  & \qw		& \qw		& \qw	& \qw		& \targ{}	& \ctrl{2}	& \qw		& \ctrl{2}	& \qw		& \qw		& \qw		& \ctrl{2}	& \targ{}	& \qw		& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw			& \qw  & \qw		& \qw  & \rstick{$c_2$} \\
	\lstick{$a_2$} & \qw  	 &\qw	& \ctrl{1} 	& \ctrl{1} 	& \qw 		& \qw 		&  \qw 	 	& \qw 		&  \qw 	 	& \qw 		& \qw 		& \qw  & \qw 		& \qw 		& \qw	& \qw 		& \qw 		&  \qw 	 	& \qw 		&  \qw 	  	& \ctrl{1} 	& \ctrl{2} 	& \ctrl{1} 	& \qw 		& \qw 		& \qw	 	& \qw 		& \qw	 	& \qw 		& \qw 		& \qw	 	& \qw 		& \qw	 	& \qw 			& \qw  & \qw 		& \qw  & \rstick{$a_2$} \\
	\lstick{$b_2$} & \qw  	 &\qw	& \ctrl{1} 	& \targ{} 	& \qw 		& \qw 		& \ctrl{1} 	& \qw 		& \ctrl{1} 	& \qw 		& \qw 		& \qw  & \qw 		& \qw 		& \qw	& \qw 		& \qw 		& \ctrl{1} 	& \qw 		& \ctrl{1} 	& \targ{} 	& \ctrl{1} 	& \targ{} 	& \targ{} 	& \qw 		& \qw	 	& \qw 		& \qw	 	& \qw 		& \qw 		& \qw	 	& \qw 		& \qw	 	& \qw 			& \qw  & \qw 		& \qw  & \rstick{$s_2$} \\
	\lstick{$0$}   & \qw  	 &\qw	& \targ{}	& \qw		& \qw		& \qw		& \targ{}	& \ctrl{2}	& \targ{}	& \qw		& \qw		& \qw  & \qw		& \qw		& \qw	& \qw		& \qw		& \targ{}	& \ctrl{2}	& \targ{}	& \qw		& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw			& \qw  & \qw		& \qw  & \rstick{$c_3$} \\
	\lstick{$a_3$} & \qw  	 &\qw	& \ctrl{1} 	& \ctrl{1} 	& \qw 		& \qw 		& \qw 		&  \qw 	 	& \qw 		& \qw 		& \qw 		& \qw  & \qw 		& \qw 		& \qw	& \qw 		& \qw 		& \qw 		& \qw 	 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw	 	& \qw 		& \qw	 	& \qw 		& \qw 		& \qw	 	& \qw 		& \qw	 	& \qw 			& \qw  & \qw 		& \qw  & \rstick{$a_3$} \\
	\lstick{$b_3$} & \qw  	 &\qw	& \ctrl{1} 	& \targ{} 	& \qw 		& \qw 		& \qw 		& \ctrl{1} 	& \qw 		& \qw 		& \qw 		& \qw  & \qw 		& \qw 		& \qw	& \qw 		& \qw 		& \qw 		& \targ{} 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw	 	& \qw 		& \qw	 	& \qw 		& \qw 		& \qw	 	& \qw 		& \qw	 	& \qw 			& \qw  & \qw 		& \qw  & \rstick{$s_3$} \\
	\lstick{$0$}   & \qw  	 &\qw	& \targ{} 	& \qw 		& \qw 		& \qw 		& \qw 		& \targ{} 	& \qw 		& \qw 		& \qw 		& \qw  & \ctrl{-12}& \qw 		& \qw	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw	 	& \qw 		& \qw	 	& \qw 		& \qw 		& \qw	 	& \qw 		& \qw	 	& \qw 			& \qw  & \ctrl{-12}& \qw  & \rstick{$c_4$}
\end{quantikz}
}

\newcommand{\KimModuloAdder}{
\begin{quantikz} [row sep= \rowSep, column sep= \colSep, transparent]
	\lstick{$0$}   & \targ{}	& \qw		& \ctrl{2}	& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{2}	& \targ{}	& \targ{}	& \ctrl{2}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{2}	& \qw		& \qw		& \qw		& \ctrl{2}		& \targ{}	& \qw  & \rstick{$0$} \\
	\lstick{$a_0$} & \ctrl{1} 	& \ctrl{1} 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		&  \qw 	 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 	 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		&  \qw 	  	& \ctrl{1} 	& \ctrl{2} 	& \ctrl{1} 	& \qw 		 	& \qw 		& \qw  & \rstick{$a_0$} \\
	\lstick{$b_0$} & \ctrl{1}	& \targ{}	& \ctrl{1}	& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}	& \qw		& \qw		& \ctrl{1}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1} 	& \targ{} 	& \ctrl{1} 	& \targ{} 	& \targ{} 		& \qw		& \qw  & \rstick{$s_0$} \\
	\lstick{$0$}   & \targ{}	& \qw		& \targ{}	& \ctrl{2}	& \qw		& \qw		& \qw		& \ctrl{2}	& \targ{}	& \qw		& \qw		& \targ{}	& \ctrl{2}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{2}	& \qw		& \qw		& \qw		& \ctrl{2}	& \targ{}	& \qw		& \targ{}	& \qw		& \qw			& \qw		& \qw  & \rstick{$c_1$} \\
	\lstick{$a_1$} & \ctrl{1} 	& \ctrl{1} 	& \qw 		&  \qw 	 	& \qw 		& \qw 		& \qw 		&  \qw 	 	& \qw 		& \qw 		& \qw 		& \qw 		&  \qw 	 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 	 	& \qw 		& \qw 		&  \qw 	  	& \ctrl{1} 	& \ctrl{2} 	& \ctrl{1} 	& \qw 		& \qw 		& \qw	 	& \qw		& \qw		& \qw 			& \qw 		& \qw  & \rstick{$a_1$} \\
	\lstick{$b_1$} & \ctrl{1} 	& \targ{} 	& \qw 		& \ctrl{1} 	& \qw 		& \qw 		& \qw 		& \ctrl{1} 	& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1} 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 	 	& \qw 		& \qw 		& \ctrl{1} 	& \targ{} 	& \ctrl{1} 	& \targ{} 	& \targ{} 	& \qw 		& \qw	 	& \qw		& \qw		& \qw 			& \qw 		& \qw  & \rstick{$s_1$} \\
	\lstick{$0$}   & \targ{}	& \qw		& \qw		& \targ{}	& \ctrl{2}	& \qw		& \ctrl{2}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \targ{}	& \ctrl{2}	& \qw		& \ctrl{2}	& \qw		& \qw		& \qw		& \ctrl{2}	& \targ{}	& \qw		& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw			& \qw		& \qw  & \rstick{$c_2$} \\
	\lstick{$a_2$} & \ctrl{1} 	& \ctrl{1} 	& \qw 		& \qw 		&  \qw 	 	& \qw 		&  \qw 	 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		&  \qw 	 	& \qw 		&  \qw 	  	& \ctrl{1} 	& \ctrl{2} 	& \ctrl{1} 	& \qw 		& \qw 		& \qw	 	& \qw 		& \qw	 	& \qw 		& \qw 		& \qw	 	& \qw 		& \qw	 	& \qw 			& \qw 		& \qw  & \rstick{$a_2$} \\
	\lstick{$b_2$} & \ctrl{1} 	& \targ{} 	& \qw 		& \qw 		& \ctrl{1} 	& \qw 		& \ctrl{1} 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1} 	& \qw 		& \ctrl{1} 	& \targ{} 	& \ctrl{1} 	& \targ{} 	& \targ{} 	& \qw 		& \qw	 	& \qw 		& \qw	 	& \qw 		& \qw 		& \qw	 	& \qw 		& \qw	 	& \qw 			& \qw 		& \qw  & \rstick{$s_2$} \\
	\lstick{$0$}   & \targ{}	& \qw		& \qw		& \qw		& \targ{}	& \ctrl{2}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \ctrl{2}	& \targ{}	& \qw		& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw			& \qw		& \qw  & \rstick{$c_3$} \\
	\lstick{$a_3$} & \ctrl{1} 	& \ctrl{1} 	& \qw 		& \qw 		& \qw 		&  \qw 	 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 	 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw	 	& \qw 		& \qw	 	& \qw 		& \qw 		& \qw	 	& \qw 		& \qw	 	& \qw 			& \qw 		& \qw  & \rstick{$a_3$} \\
	\lstick{$b_3$} & \ctrl{1} 	& \targ{} 	& \qw 		& \qw 		& \qw 		& \ctrl{1} 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{} 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw	 	& \qw 		& \qw	 	& \qw 		& \qw 		& \qw	 	& \qw 		& \qw	 	& \qw 			& \qw 		& \qw  & \rstick{$s_3$} \\
	\lstick{$0$}   & \targ{} 	& \qw 		& \qw 		& \qw 		& \qw 		& \targ{} 	& \qw 		& \qw 		& \qw 		& \ctrl{-12}& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw	 	& \qw 		& \qw	 	& \qw 		& \qw 		& \qw	 	& \qw 		& \qw	 	& \qw 			& \ctrl{-12}& \qw  & \rstick{$c_4$}
\end{quantikz}
}

\newcommand{\ProposedModuloAdderBoxed}{
\begin{quantikz} [row sep= \rowSep, column sep= \colSep, transparent]
	\lstick{$1$}   & \qw		& \qw\gategroup[16,steps=7,style={blue!75!black, ultra thick, dashed, rounded corners, inner xsep=2pt}, background]{{\sc Carry-lookahead Generation Logic}}		
											& \qw		& \ctrl{3}	& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \targ{}	& \qw		& \qw\gategroup[16,steps=14,style={green!50!black, ultra thick, dashed, rounded corners, inner xsep=2pt}, background]{{\sc Carry-lookahead Truncated Full Adder}}
																																												& \qw		& \ctrl{4}	& \qw		& \qw		& \ctrl{2}	& \qw		& \qw		& \qw		& \qw		& \ctrl{4}	& \qw		& \qw		& \qw		& \qw		& \targ{}	& \qw		& \rstick{$0$} \\
	%\lstick{$0$}   & \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \rstick{$0$} \\
	\lstick{$a_0$} & \qw		& \ctrl{2}	& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}	& \qw		& \qw		& \qw		& \qw		& \ctrl{3}	& \ctrl{1}	& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}	& \qw		& \qw		& \qw		& \ctrl{1}	& \ctrl{3}	& \qw		& \qw		& \qw		& \qw		& \rstick{$a_0$} \\
	\lstick{$b_0$} & \qw		& \ctrl{1}	& \ctrl{1}	& \ctrl{1}	& \qw		& \qw		& \qw		& \targ{}	& \qw		& \qw		& \qw		& \qw		& \ctrl{2}	& \targ{}	& \ctrl{2}	& \qw		& \qw		& \targ{}	& \targ{}	& \targ{}	& \qw		& \qw		& \ctrl{2}	& \targ{}	& \ctrl{2}	& \targ{}	& \qw		& \qw		& \qw		& \rstick{$s_0$} \\
	\lstick{$0$}   & \qw		& \targ{}	& \targ{}	& \targ{}	& \ctrl{4}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \rstick{$c_1$} \\
	\lstick{$0$}   & \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \qw		& \targ{}	& \ctrl{4}	& \qw		& \ctrl{2}	& \qw		& \qw		& \qw		& \ctrl{4}	& \targ{}	& \qw		& \targ{}	& \qw		& \qw		& \qw		& \qw		& \rstick{$0$} \\
	\lstick{$a_1$} & \qw		& \ctrl{2}	& \ctrl{1}	& \qw		& \qw		& \qw		& \qw		& \ctrl{1}	& \qw		& \qw		& \qw		& \qw		& \ctrl{3}	& \ctrl{1}	& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}	& \qw		& \qw		& \qw		& \ctrl{1}	& \ctrl{3}	& \qw		& \qw		& \qw		& \qw		& \rstick{$a_1$} \\
	\lstick{$b_1$} & \qw		& \ctrl{1}	& \targ{}	& \qw		& \ctrl{1}	& \qw		& \qw		& \targ{}	& \qw		& \qw		& \qw		& \qw		& \ctrl{2}	& \targ{}	& \qw		& \ctrl{2}	& \qw		& \targ{}	& \targ{}	& \targ{}	& \qw		& \ctrl{2}	& \qw		& \targ{}	& \ctrl{2}	& \targ{}	& \qw		& \qw		& \qw		& \rstick{$s_1$} \\
	\lstick{$0$}   & \qw		& \targ{}	& \qw		& \qw		& \targ{}	& \ctrl{8}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \rstick{$c_2$} \\
	\lstick{$0$}   & \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \qw		& \qw		& \targ{}	& \ctrl{3}	& \ctrl{2}	& \qw		& \qw		& \ctrl{3}	& \targ{}	& \qw		& \qw		& \targ{}	& \qw		& \qw		& \qw		& \qw		& \rstick{$0$} \\
	\lstick{$a_2$} & \qw		& \ctrl{3}	& \ctrl{1}	& \qw		& \qw		& \qw		& \qw		& \ctrl{1}	& \qw		& \qw		& \qw		& \qw		& \ctrl{2}	& \ctrl{1}	& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}	& \qw		& \qw		& \qw		& \ctrl{1}	& \ctrl{2}	& \qw		& \qw		& \qw		& \qw		& \rstick{$a_2$} \\
	\lstick{$b_2$} & \qw		& \ctrl{2}	& \targ{}	& \ctrl{1}	& \qw		& \qw		& \ctrl{1}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \ctrl{1}	& \targ{}	& \qw		& \qw		& \ctrl{1}	& \targ{}	& \targ{}	& \targ{}	& \ctrl{1}	& \qw		& \qw		& \targ{}	& \ctrl{1}	& \targ{}	& \qw		& \qw		& \qw		& \rstick{$s_2$} \\
	\lstick{$0$}   & \qw		& \qw		& \qw		& \targ{}	& \qw		& \ctrl{4}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \qw		& \qw		& \qw		& \targ{}	& \ctrl{3}	& \qw		& \qw		& \targ{}	& \qw		& \qw		& \qw		& \targ{}	& \qw		& \qw		& \qw		& \qw		& \rstick{$0$} \\
	\lstick{$0$}   & \qw		& \targ{}	& \qw		& \qw		& \ctrl{3}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \rstick{$c_3$} \\
	\lstick{$a_3$} & \qw		& \ctrl{2}	& \ctrl{1}	& \qw		& \qw		& \qw		& \qw		& \ctrl{1}	& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}	& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}	& \qw		& \qw		& \qw		& \ctrl{1}	& \qw		& \qw		& \qw		& \qw		& \qw		& \rstick{$a_3$} \\
	\lstick{$b_3$} & \qw		& \ctrl{1}	& \targ{}	& \ctrl{-3}	& \ctrl{1}	& \qw		& \ctrl{-3}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \qw		& \qw		& \qw		& \targ{}	& \targ{}	& \targ{}	& \qw		& \qw		& \qw		& \targ{}	& \qw		& \targ{}	& \qw		& \qw		& \qw		& \rstick{$s_3$} \\
	\lstick{$0$}   & \qw		& \targ{}	& \qw		& \qw		& \targ{}	& \targ{}	& \qw		& \qw		& \qw		& \ctrl{-15}& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{-15}& \qw		& \rstick{$c_4$}
\end{quantikz}
}

\newcommand{\ProposedModuloAdder}{
\begin{quantikz} [row sep= \rowSep, column sep= \colSep, transparent]
	\lstick{$1$}   & \qw		& \qw		& \qw		& \ctrl{3}	& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \targ{}	& \qw		& \qw		& \qw		& \ctrl{4}	& \qw		& \qw		& \ctrl{2}	& \qw		& \qw		& \qw		& \qw		& \ctrl{4}	& \qw		& \qw		& \qw		& \qw		& \targ{}	& \qw		& \rstick{$1$} \\
	%\lstick{$0$}   & \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \rstick{$0$} \\
	\lstick{$a_0$} & \qw		& \ctrl{2}	& \qw		& \qw		& \ctrl{1}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{3}	& \ctrl{1}	& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}	& \qw		& \qw		& \qw		& \ctrl{1}	& \ctrl{3}	& \qw		& \qw		& \qw		& \qw		& \rstick{$a_0$} \\
	\lstick{$b_0$} & \qw		& \ctrl{1}	& \ctrl{1}	& \ctrl{1}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{2}	& \targ{}	& \ctrl{2}	& \qw		& \qw		& \targ{}	& \targ{}	& \targ{}	& \qw		& \qw		& \ctrl{2}	& \targ{}	& \ctrl{2}	& \targ{}	& \qw		& \qw		& \qw		& \rstick{$s_0$} \\
	\lstick{$0$}   & \qw		& \targ{}	& \targ{}	& \targ{}	& \ctrl{4}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \rstick{$c_1$} \\
	\lstick{$0$}   & \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \qw		& \targ{}	& \ctrl{4}	& \qw		& \ctrl{2}	& \qw		& \qw		& \qw		& \ctrl{4}	& \targ{}	& \qw		& \targ{}	& \qw		& \qw		& \qw		& \qw		& \rstick{$0$} \\
	\lstick{$a_1$} & \qw		& \ctrl{2}	& \ctrl{1}	& \qw		& \qw		& \ctrl{1}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{3}	& \ctrl{1}	& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}	& \qw		& \qw		& \qw		& \ctrl{1}	& \ctrl{3}	& \qw		& \qw		& \qw		& \qw		& \rstick{$a_1$} \\
	\lstick{$b_1$} & \qw		& \ctrl{1}	& \targ{}	& \qw		& \ctrl{1}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{2}	& \targ{}	& \qw		& \ctrl{2}	& \qw		& \targ{}	& \targ{}	& \targ{}	& \qw		& \ctrl{2}	& \qw		& \targ{}	& \ctrl{2}	& \targ{}	& \qw		& \qw		& \qw		& \rstick{$s_1$} \\
	\lstick{$0$}   & \qw		& \targ{}	& \qw		& \qw		& \targ{}	& \ctrl{8}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \rstick{$c_2$} \\
	\lstick{$0$}   & \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \qw		& \qw		& \targ{}	& \ctrl{3}	& \ctrl{2}	& \qw		& \qw		& \ctrl{3}	& \targ{}	& \qw		& \qw		& \targ{}	& \qw		& \qw		& \qw		& \qw		& \rstick{$0$} \\
	\lstick{$a_2$} & \qw		& \ctrl{3}	& \ctrl{1}	& \qw		& \qw		& \qw		& \qw		& \ctrl{1}	& \qw		& \qw		& \qw		& \qw		& \ctrl{2}	& \ctrl{1}	& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}	& \qw		& \qw		& \qw		& \ctrl{1}	& \ctrl{2}	& \qw		& \qw		& \qw		& \qw		& \rstick{$a_2$} \\
	\lstick{$b_2$} & \qw		& \ctrl{2}	& \targ{}	& \ctrl{1}	& \qw		& \qw		& \ctrl{1}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \ctrl{1}	& \targ{}	& \qw		& \qw		& \ctrl{1}	& \targ{}	& \targ{}	& \targ{}	& \ctrl{1}	& \qw		& \qw		& \targ{}	& \ctrl{1}	& \targ{}	& \qw		& \qw		& \qw		& \rstick{$s_2$} \\
	\lstick{$0$}   & \qw		& \qw		& \qw		& \targ{}	& \qw		& \ctrl{4}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \qw		& \qw		& \qw		& \targ{}	& \ctrl{3}	& \qw		& \qw		& \targ{}	& \qw		& \qw		& \qw		& \targ{}	& \qw		& \qw		& \qw		& \qw		& \rstick{$0$} \\
	\lstick{$0$}   & \qw		& \targ{}	& \qw		& \qw		& \ctrl{3}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \rstick{$c_3$} \\
	\lstick{$a_3$} & \qw		& \ctrl{2}	& \ctrl{1}	& \qw		& \qw		& \qw		& \qw		& \ctrl{1}	& \qw		& \qw		& \qw		& \qw		& \ctrl{1}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}	& \qw		& \qw		& \qw		& \ctrl{1}	& \qw		& \qw		& \qw		& \qw		& \qw		& \rstick{$a_3$} \\
	\lstick{$b_3$} & \qw		& \ctrl{1}	& \targ{}	& \ctrl{-3}	& \ctrl{1}	& \qw		& \ctrl{-3}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \targ{}	& \qw		& \qw		& \qw		& \qw		& \targ{}	& \targ{}	& \targ{}	& \qw		& \qw		& \qw		& \targ{}	& \qw		& \targ{}	& \qw		& \qw		& \qw		& \rstick{$s_3$} \\
	\lstick{$0$}   & \qw		& \targ{}	& \qw		& \qw		& \targ{}	& \targ{}	& \qw		& \qw		& \qw		& \ctrl{-15}& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{-15}& \qw		& \rstick{$c_4$}
\end{quantikz}
}


\newcommand{\thapliyalThirteen}{
\begin{quantikz} [row sep= \rowSep, column sep= \colSep, transparent]
	\lstick{$a_0$} & \qw	   & \qw		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw & \rstick{$s_0$} \\
	\lstick{$b_0$} & \qw 	   & \qw 		& \qw 		& \qw 		& \ctrl{2}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \qw 		& \qw		& \qw & \rstick{$b_0$} \\
	\lstick{$a_1$} & \targ{}   & \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \targ{}	& \qw & \rstick{$s_1$} \\
	\lstick{$b_1$} & \ctrl{-1} & \qw 		& \qw 		& \ctrl{2}	& \targ{}	& \ctrl{2}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \targ{}	& \ctrl{2}	& \qw 		& \ctrl{-1}	& \qw & \rstick{$b_1$} \\
	\lstick{$a_2$} & \targ{}   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \qw & \rstick{$s_2$} \\
	\lstick{$b_2$} & \ctrl{-1} & \qw 		& \ctrl{2}	& \targ{}	& \qw 		& \targ{}	& \ctrl{2}	& \qw 		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \targ{}	& \ctrl{2}	& \ctrl{-1}	& \qw & \rstick{$b_2$} \\
	\lstick{$a_3$} & \targ{}   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \qw & \rstick{$s_3$} \\
	\lstick{$b_3$} & \ctrl{-1} & \ctrl{1} 	& \targ{}	& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{1}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{-1}	& \qw & \rstick{$b_3$} \\
	\lstick{$z$}   & \qw       & \targ{} 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$z \oplus s_4$}			
\end{quantikz}
}

\newcommand{\thapliyalThirteenFive}{
\begin{quantikz} [row sep= \rowSep, column sep= \colSep, transparent]
	\lstick{$a_0$} & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw		& \qw 		& \qw      & \targ{}	& \qw & \rstick{$s_0$} \\
	\lstick{$b_0$} & \qw	   & \qw 	   & \qw 		& \qw 		& \qw 		& \ctrl{2}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{2}	& \qw		& \qw 		& \qw      & \ctrl{-1}	& \qw & \rstick{$b_0$} \\
	\lstick{$a_1$} & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw & \rstick{$s_1$} \\
	\lstick{$b_1$} & \ctrl{-1} & \qw	   & \qw 		& \qw 		& \ctrl{2}	& \targ{}	& \ctrl{2}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \targ{}	& \ctrl{2}	& \qw 		& \qw      & \ctrl{-1}	& \qw & \rstick{$b_1$} \\
	\lstick{$a_2$} & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw & \rstick{$s_2$} \\
	\lstick{$b_2$} & \ctrl{-1} & \qw	   & \qw 		& \ctrl{2}	& \targ{}	& \qw 		& \targ{}	& \ctrl{2}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \targ{}	& \ctrl{2}	& \qw      & \ctrl{-1}	& \qw & \rstick{$b_2$} \\
	\lstick{$a_3$} & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw  		& \qw  		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw & \rstick{$s_3$} \\
	\lstick{$b_3$} & \ctrl{-1} & \qw	   & \ctrl{2}  	& \targ{}	& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{2}	& \qw  		& \qw  		& \ctrl{2}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{2} & \ctrl{-1}	& \qw & \rstick{$b_3$} \\
	\lstick{$a_4$} & \targ{}   & \qw	   & \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}  & \targ{}  	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw      & \targ{}	& \qw & \rstick{$s_4$} \\		
	\lstick{$b_4$} & \ctrl{-1} & \ctrl{1}  & \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \ctrl{1}  & \ctrl{-1}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}  & \ctrl{-1}	& \qw & \rstick{$b_4$} \\		
	\lstick{$z$}   & \qw       & \targ{}   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw 		& \targ{}  	& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \qw 		& \qw & \rstick{$z \oplus s_5$}			
\end{quantikz}
}

\newcommand{\thapliyalThirteenFiveGap}{
\begin{quantikz} [row sep= \rowSep, column sep= \colSep, transparent]
	\lstick{$0$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw & \rstick{$0$} \\
	\lstick{$a_0$} & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw		& \qw 		& \qw      & \targ{}	& \qw & \rstick{$s_0$} \\
	\lstick{$b_0$} & \qw	   & \qw 	   & \qw 		& \qw 		& \qw 		& \ctrl{3}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \qw		& \qw 		& \qw      & \ctrl{-1}	& \qw & \rstick{$b_0$} \\
	\lstick{$0$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw & \rstick{$0$} \\
	\lstick{$a_1$} & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw & \rstick{$s_1$} \\
	\lstick{$b_1$} & \ctrl{-1} & \qw	   & \qw 		& \qw 		& \ctrl{3}	& \targ{}	& \ctrl{3}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \ctrl{3}	& \qw 		& \qw      & \ctrl{-1}	& \qw & \rstick{$b_1$} \\
	\lstick{$0$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw & \rstick{$0$} \\
	\lstick{$a_2$} & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw & \rstick{$s_2$} \\
	\lstick{$b_2$} & \ctrl{-1} & \qw	   & \qw 		& \ctrl{3}	& \targ{}	& \qw 		& \targ{}	& \ctrl{3}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \targ{}	& \ctrl{3}	& \qw      & \ctrl{-1}	& \qw & \rstick{$b_2$} \\
	\lstick{$0$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw & \rstick{$0$} \\
	\lstick{$a_3$} & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw  		& \qw  		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw & \rstick{$s_3$} \\
	\lstick{$b_3$} & \ctrl{-1} & \qw	   & \ctrl{3}  	& \targ{}	& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{3}	& \qw  		& \qw  		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{3} & \ctrl{-1}	& \qw & \rstick{$b_3$} \\
	\lstick{$0$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw & \rstick{$0$} \\
	\lstick{$a_4$} & \targ{}   & \qw	   & \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}  & \targ{}  	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw      & \targ{}	& \qw & \rstick{$s_4$} \\		
	\lstick{$b_4$} & \ctrl{-1} & \ctrl{1}  & \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \ctrl{1}  & \ctrl{-1}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}  & \ctrl{-1}	& \qw & \rstick{$b_4$} \\		
	\lstick{$z$}   & \qw       & \targ{}   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw 		& \targ{}  	& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \qw 		& \qw & \rstick{$z \oplus s_5$}\\
	\lstick{$0$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw & \rstick{$0$}		
\end{quantikz}
}

\newcommand{\thapliyalThirteenFiveNOR}{
\begin{quantikz} [row sep= \rowSep, column sep= \rowSep, transparent]
	\lstick{$0$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw 		& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$0$} \\
	\lstick{$a_0$} & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw		& \qw 		& \qw      & \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$s_0$} \\
	\lstick{$b_0$} & \qw	   & \qw 	   & \qw 		& \qw 		& \qw 		& \ctrl{3}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \qw		& \qw 		& \qw      & \ctrl{-1}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_0$} \\
	\lstick{$0$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$0$} \\
	\lstick{$a_1$} & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$s_1$} \\
	\lstick{$b_1$} & \ctrl{-1} & \qw	   & \qw 		& \qw 		& \ctrl{3}	& \targ{}	& \ctrl{3}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \ctrl{3}	& \qw 		& \qw      & \ctrl{-1}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_1$} \\
	\lstick{$0$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$0$} \\
	\lstick{$a_2$} & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$s_2$} \\
	\lstick{$b_2$} & \ctrl{-1} & \qw	   & \qw 		& \ctrl{3}	& \targ{}	& \qw 		& \targ{}	& \ctrl{3}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \targ{}	& \ctrl{3}	& \qw      & \ctrl{-1}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_2$} \\
	\lstick{$0$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$0$} \\
	\lstick{$a_3$} & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw  		& \qw  		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$s_3$} \\
	\lstick{$b_3$} & \ctrl{-1} & \qw	   & \ctrl{3}  	& \targ{}	& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{3}	& \qw  		& \qw  		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{3} & \ctrl{-1}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_3$} \\
	\lstick{$0$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$0$} \\
	\lstick{$a_4$} & \targ{}   & \qw	   & \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}  & \targ{}  	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw      & \targ{}	& \targ{}	& \ctrl{-13}& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$s_4$} \\		
	\lstick{$b_4$} & \ctrl{-1} & \ctrl{1}  & \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \ctrl{1}  & \ctrl{-1}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}  & \ctrl{-1}	& \qw	 	& \qw		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_4$} \\		
	\lstick{$z$}   & \qw       & \targ{}   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw 		& \targ{}  	& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \qw 		& \targ{}	& \ctrl{-2}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$z \oplus s_5$}\\
	\lstick{$0$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw	 	& \qw		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$0$}		
\end{quantikz}
}

\newcommand{\QMAoneBoxed}{
\begin{quantikz} [row sep= 0.08cm, column sep= 0.04cm, transparent]
	\lstick{$0$}   & \qw	& \qw\gategroup[wires=17,steps=22,style={blue!75!black, thick, dashed, rounded corners, inner xsep=2pt}, background]{{\sc full adder stage generating Sum}} & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw	& \qw 		& \targ{}	& \qw 		& \qw	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw		& \qw 		& \qw 		& \targ{}	& \qw & \rstick{$m_0$} \\
	\lstick{$a_0$} & \qw	& \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw		& \qw 		& \qw      & \targ{}	& \qw	& \qw 		& \qw 		& \qw 		& \qw	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \qw		& \qw 		& \qw 		& \ctrl{-1}	& \qw & \rstick{$s_0$} \\
	\lstick{$b_0$} & \qw	& \qw	   & \qw 	   & \qw 		& \qw 		& \qw 		& \ctrl{3}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \qw		& \qw 		& \qw      & \ctrl{-1}	& \qw	& \qw 		& \qw 		& \qw 		& \qw	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_0$} \\
	\lstick{$0$}   & \qw	& \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw	& \qw 		& \qw 		& \qw 		& \qw	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw		& \qw 		& \targ{}	& \qw & \rstick{$m_1$} \\
	\lstick{$a_1$} & \qw	& \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw	& \qw 		& \qw 		& \qw 		& \qw	& \ctrl{-1}	& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \targ{}	& \ctrl{3}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \ctrl{3}	& \qw		& \qw 		& \ctrl{-1}	& \qw & \rstick{$s_1$} \\
	\lstick{$b_1$} & \qw	& \ctrl{-1} & \qw	   & \qw 		& \qw 		& \ctrl{3}	& \targ{}	& \ctrl{3}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \ctrl{3}	& \qw 		& \qw      & \ctrl{-1}	& \qw	& \qw 		& \qw 		& \qw 		& \qw	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_1$} \\
	\lstick{$0$}   & \qw	& \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw	& \qw 		& \qw 		& \qw 		& \qw	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \qw & \rstick{$m_2$} \\
	\lstick{$a_2$} & \qw	& \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw	& \qw 		& \qw 		& \qw 		& \qw	& \ctrl{-1}	& \qw 		& \qw 		& \ctrl{3}	& \targ{}	& \qw 		& \targ{}	& \ctrl{3}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \targ{}	& \ctrl{3}	& \qw 		& \ctrl{-1}	& \qw & \rstick{$s_2$} \\
	\lstick{$b_2$} & \qw	& \ctrl{-1} & \qw	   & \qw 		& \ctrl{3}	& \targ{}	& \qw 		& \targ{}	& \ctrl{3}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \targ{}	& \ctrl{3}	& \qw      & \ctrl{-1}	& \qw	& \qw 		& \qw 		& \qw 		& \qw	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_2$} \\
	\lstick{$0$}   & \qw	& \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw	& \qw 		& \qw 		& \qw 		& \qw	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \qw & \rstick{$m_3$} \\
	\lstick{$a_3$} & \qw	& \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw  		& \qw  		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw	& \qw 		& \qw 		& \qw 		& \qw	& \ctrl{-1}	& \qw 		& \ctrl{5}	& \targ{}	& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{5}	& \qw		& \qw 		& \ctrl{5}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{5}	& \ctrl{-1}	& \qw & \rstick{$s_3$} \\
	\lstick{$b_3$} & \qw	& \ctrl{-1} & \qw	   & \ctrl{3}  	& \targ{}	& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{3}	& \qw  		& \qw  		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{3} & \ctrl{-1}	& \qw	& \qw 		& \qw 		& \qw 		& \qw	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_3$} \\
	\lstick{$0$}   & \qw	& \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw	& \qw 		& \qw 		& \qw 		& \qw	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \qw & \rstick{$m_4$} \\
	\lstick{$a_4$} & \qw	& \targ{}   & \qw	   & \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}  & \targ{}  	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw      & \targ{}	& \qw	& \targ{}	& \ctrl{-13}& \targ{}	& \qw	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$s_4$} \\		
	\lstick{$b_4$} & \qw	& \ctrl{-1} & \ctrl{1}  & \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \ctrl{1}  & \ctrl{-1}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}  & \ctrl{-1}	& \qw	& \qw	 	& \qw		& \qw		& \qw	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_4$} \\		
	\lstick{$0$}   & \qw	& \qw       & \targ{}   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw 		& \targ{}  	& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \qw 		& \qw	& \targ{}	& \ctrl{-2}	& \targ{}	& \qw	& \ctrl{-3}	& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{1}	& \ctrl{-3}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{-3}	& \qw & \rstick{$s_5$}\\
	\lstick{$0$}   & \qw	& \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw	& \qw	 	& \qw		& \qw		& \qw	& \qw 		& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$s_6$}			
\end{quantikz}
}

\newcommand{\QMAoneSliced}{
\begin{quantikz} [row sep= 0.1cm, column sep= 0.05cm, transparent]
	\lstick{$0$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw\slice[style=blue]{1} & \qw & \qw		& \targ{}	& \qw\slice[style=blue]{2} & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw		& \qw 		& \qw 		& \targ{}	& \qw & \rstick{$m_0$} \\
	\lstick{$a_0$} & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw		& \qw 		& \qw      & \targ{}				  & \qw	& \qw 		& \qw 		& \qw 					   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \qw		& \qw 		& \qw 		& \ctrl{-1}	& \qw & \rstick{$s_0$} \\
	\lstick{$b_0$} & \qw	   & \qw 	   & \qw 		& \qw 		& \qw 		& \ctrl{3}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \qw		& \qw 		& \qw      & \ctrl{-1}				  & \qw	& \qw 		& \qw 		& \qw 					   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_0$} \\
	\lstick{$0$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw					  & \qw	& \qw 		& \qw 		& \qw 					   & \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw		& \qw 		& \targ{}	& \qw & \rstick{$m_1$} \\
	\lstick{$a_1$} & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw      & \targ{}				  & \qw	& \qw 		& \qw 		& \qw 					   & \ctrl{-1}	& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \targ{}	& \ctrl{3}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \ctrl{3}	& \qw		& \qw 		& \ctrl{-1}	& \qw & \rstick{$s_1$} \\
	\lstick{$b_1$} & \ctrl{-1} & \qw	   & \qw 		& \qw 		& \ctrl{3}	& \targ{}	& \ctrl{3}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \ctrl{3}	& \qw 		& \qw      & \ctrl{-1}				  & \qw	& \qw 		& \qw 		& \qw 					   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_1$} \\
	\lstick{$0$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw					  & \qw	& \qw 		& \qw 		& \qw 					   & \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \qw & \rstick{$m_2$} \\
	\lstick{$a_2$} & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}				  & \qw	& \qw 		& \qw 		& \qw 					   & \ctrl{-1}	& \qw 		& \qw 		& \ctrl{3}	& \targ{}	& \qw 		& \targ{}	& \ctrl{3}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \targ{}	& \ctrl{3}	& \qw 		& \ctrl{-1}	& \qw & \rstick{$s_2$} \\
	\lstick{$b_2$} & \ctrl{-1} & \qw	   & \qw 		& \ctrl{3}	& \targ{}	& \qw 		& \targ{}	& \ctrl{3}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \targ{}	& \ctrl{3}	& \qw      & \ctrl{-1}				  & \qw	& \qw 		& \qw 		& \qw 					   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_2$} \\
	\lstick{$0$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw					  & \qw	& \qw 		& \qw 		& \qw 					   & \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \qw & \rstick{$m_3$} \\
	\lstick{$a_3$} & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw  		& \qw  		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}				  & \qw	& \qw 		& \qw 		& \qw 					   & \ctrl{-1}	& \qw 		& \ctrl{5}	& \targ{}	& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{5}	& \qw		& \qw 		& \ctrl{5}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{5}	& \ctrl{-1}	& \qw & \rstick{$s_3$} \\
	\lstick{$b_3$} & \ctrl{-1} & \qw	   & \ctrl{3}  	& \targ{}	& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{3}	& \qw  		& \qw  		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{3} & \ctrl{-1}				  & \qw	& \qw 		& \qw 		& \qw 					   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_3$} \\
	\lstick{$0$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw					  & \qw	& \qw 		& \qw 		& \qw 					   & \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \qw & \rstick{$m_4$} \\
	\lstick{$a_4$} & \targ{}   & \qw	   & \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}  & \targ{}  	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw      & \targ{}				  & \qw	& \targ{}	& \ctrl{-13}& \targ{}				   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$s_4$} \\		
	\lstick{$b_4$} & \ctrl{-1} & \ctrl{1}  & \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \ctrl{1}  & \ctrl{-1}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}  & \ctrl{-1}				  & \qw	& \qw	 	& \qw		& \qw					   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_4$} \\		
	\lstick{$0$}   & \qw       & \targ{}   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw 		& \targ{}  	& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \qw 					  & \qw	& \targ{}	& \ctrl{-2}	& \targ{}				   & \ctrl{-3}	& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{1}	& \ctrl{-3}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{-3}	& \qw & \rstick{$s_5$}\\
	\lstick{$0$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw					  & \qw	& \qw	 	& \qw		& \qw					   & \qw 		& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$s_6$}			
\end{quantikz}
}

\newcommand{\QMAone}{
\begin{quantikz} [row sep= 0.08cm, column sep= 0.03cm, transparent]
	\lstick{$0$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw 		& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw		& \qw 		& \qw 		& \targ{}	& \qw & \rstick{$m_0$} \\
	\lstick{$a_0$} & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw		& \qw 		& \qw      & \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \qw		& \qw 		& \qw 		& \ctrl{-1}	& \qw & \rstick{$s_0$} \\
	\lstick{$b_0$} & \qw	   & \qw 	   & \qw 		& \qw 		& \qw 		& \ctrl{3}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \qw		& \qw 		& \qw      & \ctrl{-1}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_0$} \\
	\lstick{$0$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw 		& \qw 		& \qw 		& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw		& \qw 		& \targ{}	& \qw & \rstick{$m_1$} \\
	\lstick{$a_1$} & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw 		& \qw 		& \qw 		& \ctrl{-1}	& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \targ{}	& \ctrl{3}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \ctrl{3}	& \qw		& \qw 		& \ctrl{-1}	& \qw & \rstick{$s_1$} \\
	\lstick{$b_1$} & \ctrl{-1} & \qw	   & \qw 		& \qw 		& \ctrl{3}	& \targ{}	& \ctrl{3}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \ctrl{3}	& \qw 		& \qw      & \ctrl{-1}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_1$} \\
	\lstick{$0$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw 		& \qw 		& \qw 		& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \qw & \rstick{$m_2$} \\
	\lstick{$a_2$} & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw 		& \qw 		& \qw 		& \ctrl{-1}	& \qw 		& \qw 		& \ctrl{3}	& \targ{}	& \qw 		& \targ{}	& \ctrl{3}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \targ{}	& \ctrl{3}	& \qw 		& \ctrl{-1}	& \qw & \rstick{$s_2$} \\
	\lstick{$b_2$} & \ctrl{-1} & \qw	   & \qw 		& \ctrl{3}	& \targ{}	& \qw 		& \targ{}	& \ctrl{3}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \targ{}	& \ctrl{3}	& \qw      & \ctrl{-1}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_2$} \\
	\lstick{$0$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw 		& \qw 		& \qw 		& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \qw & \rstick{$m_3$} \\
	\lstick{$a_3$} & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw  		& \qw  		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw 		& \qw 		& \qw 		& \ctrl{-1}	& \qw 		& \ctrl{5}	& \targ{}	& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{5}	& \qw		& \qw 		& \ctrl{5}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{5}	& \ctrl{-1}	& \qw & \rstick{$s_3$} \\
	\lstick{$b_3$} & \ctrl{-1} & \qw	   & \ctrl{3}  	& \targ{}	& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{3}	& \qw  		& \qw  		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{3} & \ctrl{-1}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_3$} \\
	\lstick{$0$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw 		& \qw 		& \qw 		& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \qw & \rstick{$m_4$} \\
	\lstick{$a_4$} & \targ{}   & \qw	   & \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}  & \targ{}  	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw      & \targ{}	& \targ{}	& \ctrl{-13}& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$s_4$} \\		
	\lstick{$b_4$} & \ctrl{-1} & \ctrl{1}  & \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \ctrl{1}  & \ctrl{-1}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}  & \ctrl{-1}	& \qw	 	& \qw		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_4$} \\		
	\lstick{$0$}   & \qw       & \targ{}   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw 		& \targ{}  	& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \qw 		& \targ{}	& \ctrl{-2}	& \targ{}	& \ctrl{-3}	& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{1}	& \ctrl{-3}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{-3}	& \qw & \rstick{$s_5$}\\
	\lstick{$0$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw	 	& \qw		& \qw		& \qw 		& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$s_6$}			
\end{quantikz}
}

\newcommand{\QMAtwoBoxed}{
\begin{quantikz} [row sep= 0.1cm, column sep= 0.05cm, transparent]
	\lstick{$0$}   & \qw   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw 		& \targ{}	& \qw  		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$m_0$} \\
	\lstick{$a_0$} & \qw   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw		& \qw 		& \qw      & \targ{}	& \qw 		& \qw 		& \qw  		& \ctrl{2}	& \ctrl{-1}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$s_0$} \\
	\lstick{$b_0$} & \qw   & \qw	   & \qw 	   & \qw 		& \qw 		& \qw 		& \ctrl{3}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \qw		& \qw 		& \qw      & \ctrl{-1}	& \qw 		& \qw 		& \qw  		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_0$} \\
	\lstick{$0$}   & \qw   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw 		& \qw 		& \qw  		& \targ{}	& \ctrl{1}	& \targ{  }	& \qw 		& \qw 		& \qw 		& \qw & \rstick{$m_1$} \\
	\lstick{$a_1$} & \qw   & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw 		& \qw 		& \qw  		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \qw 		& \qw 		& \qw 		& \qw & \rstick{$s_1$} \\
	\lstick{$b_1$} & \qw   & \ctrl{-1} & \qw	   & \qw 		& \qw 		& \ctrl{3}	& \targ{}	& \ctrl{3}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \ctrl{3}	& \qw 		& \qw      & \ctrl{-1}	& \qw 		& \qw 		& \qw  		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_1$} \\
	\lstick{$0$}   & \qw   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw 		& \qw 		& \qw  		& \qw 		& \targ{}	& \ctrl{1}	& \targ{  }	& \qw 		& \qw 		& \qw & \rstick{$m_2$} \\
	\lstick{$a_2$} & \qw   & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw 		& \qw 		& \qw  		& \qw 		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \qw 		& \qw 		& \qw & \rstick{$s_2$} \\
	\lstick{$b_2$} & \qw   & \ctrl{-1} & \qw	   & \qw 		& \ctrl{3}	& \targ{}	& \qw 		& \targ{}	& \ctrl{3}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \targ{}	& \ctrl{3}	& \qw      & \ctrl{-1}	& \qw 		& \qw 		& \qw  		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_2$} \\
	\lstick{$0$}   & \qw   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw 		& \qw 		& \qw  		& \qw 		& \qw 		& \targ{}	& \ctrl{1}	& \targ{  }	& \qw 		& \qw & \rstick{$m_3$} \\
	\lstick{$a_3$} & \qw   & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw  		& \qw  		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw 		& \qw 		& \qw  		& \qw 		& \qw 		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \qw 		& \qw & \rstick{$s_3$} \\
	\lstick{$b_3$} & \qw   & \ctrl{-1} & \qw	   & \ctrl{3}  	& \targ{}	& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{3}	& \qw  		& \qw  		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{3} & \ctrl{-1}	& \qw 		& \qw 		& \qw  		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_3$} \\
	\lstick{$0$}   & \qw   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw 		& \qw 		& \qw  		& \qw 		& \qw 		& \qw 		& \targ{}	& \targ{}	& \qw 		& \qw & \rstick{$m_4$} \\
	\lstick{$a_4$} & \qw   & \targ{}   & \qw	   & \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}  & \targ{}  	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw      & \targ{}	& \targ{}	& \ctrl{-13}& \targ{}	& \qw		& \qw 		& \qw 		& \qw 		& \qw		& \qw 		& \qw & \rstick{$s_4$} \\		
	\lstick{$b_4$} & \qw   & \ctrl{-1} & \ctrl{1}  & \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \ctrl{1}  & \ctrl{-1}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}  & \ctrl{-1}	& \qw	 	& \qw		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_4$} \\		
	\lstick{$0$}   & \qw   & \qw       & \targ{}   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw 		& \targ{}  	& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \qw 		& \targ{}	& \ctrl{-2}	& \targ{}	& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{-3}	& \qw 		& \qw & \rstick{$s_5$}
\end{quantikz}
}

\newcommand{\QMAtwo}{
\begin{quantikz} [row sep= 0.1cm, column sep= 0.05cm, transparent]
	\lstick{$0$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw 		& \targ{}	& \qw  		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$m_0$} \\
	\lstick{$a_0$} & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw		& \qw 		& \qw      & \targ{}	& \qw 		& \qw 		& \qw  		& \ctrl{2}	& \ctrl{-1}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$s_0$} \\
	\lstick{$b_0$} & \qw	   & \qw 	   & \qw 		& \qw 		& \qw 		& \ctrl{3}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \qw		& \qw 		& \qw      & \ctrl{-1}	& \qw 		& \qw 		& \qw  		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_0$} \\
	\lstick{$0$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw 		& \qw 		& \qw  		& \targ{}	& \ctrl{1}	& \targ{  }	& \qw 		& \qw 		& \qw 		& \qw & \rstick{$m_1$} \\
	\lstick{$a_1$} & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw 		& \qw 		& \qw  		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \qw 		& \qw 		& \qw 		& \qw & \rstick{$s_1$} \\
	\lstick{$b_1$} & \ctrl{-1} & \qw	   & \qw 		& \qw 		& \ctrl{3}	& \targ{}	& \ctrl{3}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \ctrl{3}	& \qw 		& \qw      & \ctrl{-1}	& \qw 		& \qw 		& \qw  		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_1$} \\
	\lstick{$0$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw 		& \qw 		& \qw  		& \qw 		& \targ{}	& \ctrl{1}	& \targ{  }	& \qw 		& \qw 		& \qw & \rstick{$m_2$} \\
	\lstick{$a_2$} & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw 		& \qw 		& \qw  		& \qw 		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \qw 		& \qw 		& \qw & \rstick{$s_2$} \\
	\lstick{$b_2$} & \ctrl{-1} & \qw	   & \qw 		& \ctrl{3}	& \targ{}	& \qw 		& \targ{}	& \ctrl{3}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \targ{}	& \ctrl{3}	& \qw      & \ctrl{-1}	& \qw 		& \qw 		& \qw  		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_2$} \\
	\lstick{$0$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw 		& \qw 		& \qw  		& \qw 		& \qw 		& \targ{}	& \ctrl{1}	& \targ{  }	& \qw 		& \qw & \rstick{$m_3$} \\
	\lstick{$a_3$} & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw  		& \qw  		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw 		& \qw 		& \qw  		& \qw 		& \qw 		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \qw 		& \qw & \rstick{$s_3$} \\
	\lstick{$b_3$} & \ctrl{-1} & \qw	   & \ctrl{3}  	& \targ{}	& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{3}	& \qw  		& \qw  		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{3} & \ctrl{-1}	& \qw 		& \qw 		& \qw  		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_3$} \\
	\lstick{$0$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw 		& \qw 		& \qw  		& \qw 		& \qw 		& \qw 		& \targ{}	& \targ{}	& \qw 		& \qw & \rstick{$m_4$} \\
	\lstick{$a_4$} & \targ{}   & \qw	   & \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}  & \targ{}  	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw      & \targ{}	& \targ{}	& \ctrl{-13}& \targ{}	& \qw		& \qw 		& \qw 		& \qw 		& \qw		& \qw 		& \qw & \rstick{$s_4$} \\		
	\lstick{$b_4$} & \ctrl{-1} & \ctrl{1}  & \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \ctrl{1}  & \ctrl{-1}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}  & \ctrl{-1}	& \qw	 	& \qw		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_4$} \\		
	\lstick{$0$}   & \qw       & \targ{}   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw 		& \targ{}  	& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \qw 		& \targ{}	& \ctrl{-2}	& \targ{}	& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{-3}	& \qw 		& \qw & \rstick{$s_5$}
\end{quantikz}
}

\newcommand{\QMAtwoLessQubits}{
\begin{quantikz} [row sep= 0.1cm, column sep= 0.05cm, transparent]
	\lstick{\ket{0}}& \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw 		& \targ{}	& \qw  				& \qw 	& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw & \rstick{$m_0$} \\
	\lstick{$a_0$} & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw		& \qw 		& \qw      & \targ{}	& \qw 		& \qw 		& \qw  				& \qw 	& \ctrl{1}	& \ctrl{-1}	& \qw 		& \qw 		& \qw 		& \qw & \rstick{$s_0$} \\
	\lstick{$b_0$} & \qw	   & \qw 	   & \qw 		& \qw 		& \qw 		& \ctrl{2}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{2}	& \qw		& \qw 		& \qw      & \ctrl{-1}	& \qw 		& \qw 		& \gate{\ket{0}}	& \qw 	& \targ{}	& \ctrl{1}	& \targ{  } & \qw 		& \qw 		& \qw & \rstick{$m_1$} \\
	%\lstick{$0$}  & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw 		& \qw 		& \qw  				& \qw 	& \targ{}	& \ctrl{1}	& \targ{  }	& \qw 		& \qw 		& \qw & \rstick{$0$} \\
	\lstick{$a_1$} & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw 		& \qw 		& \qw  				& \qw 	& \qw 		& \ctrl{1}	& \ctrl{-1}	& \qw 		& \qw 		& \qw & \rstick{$s_1$} \\
	\lstick{$b_1$} & \ctrl{-1} & \qw	   & \qw 		& \qw 		& \ctrl{2}	& \targ{}	& \ctrl{2}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \targ{}	& \ctrl{2}	& \qw 		& \qw      & \ctrl{-1}	& \qw 		& \qw 		& \gate{\ket{0}}	& \qw 	& \qw 		& \targ{}	& \ctrl{1}	& \targ{  }	& \qw 		& \qw & \rstick{$m_2$} \\
	%\lstick{$0$}  & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw 		& \qw 		& \qw  				& \qw 	& \qw 		& \targ{}	& \ctrl{1}	& \targ{  }	& \qw 		& \qw & \rstick{$0$} \\
	\lstick{$a_2$} & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw 		& \qw 		& \qw  				& \qw 	& \qw 		& \qw 		& \ctrl{1}	& \ctrl{-1}	& \qw 		& \qw & \rstick{$s_2$} \\
	\lstick{$b_2$} & \ctrl{-1} & \qw	   & \qw 		& \ctrl{2}	& \targ{}	& \qw 		& \targ{}	& \ctrl{2}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \targ{}	& \ctrl{2}	& \qw      & \ctrl{-1}	& \qw 		& \qw 		& \gate{\ket{0}}	& \qw 	& \qw 		& \qw 		& \targ{}	& \ctrl{1}	& \targ{  }	& \qw & \rstick{$m_3$} \\
	%\lstick{$0$}  & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw 		& \qw 		& \qw  				& \qw 	& \qw 		& \qw 		& \targ{}	& \ctrl{1}	& \targ{  }	& \qw & \rstick{$0$} \\
	\lstick{$a_3$} & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw  		& \qw  		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw 		& \qw 		& \qw  				& \qw 	& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \ctrl{-1}	& \qw & \rstick{$s_3$} \\
	\lstick{$b_3$} & \ctrl{-1} & \qw	   & \ctrl{2}  	& \targ{}	& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{2}	& \qw  		& \qw  		& \ctrl{2}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{2} & \ctrl{-1}	& \qw 		& \qw 		& \gate{\ket{0}}	& \qw 	& \qw 		& \qw 		& \qw 		& \targ{}	& \targ{}	& \qw & \rstick{$m_4$} \\
	%\lstick{$0$}  & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw 		& \qw 		& \qw  				& \qw 	& \qw 		& \qw 		& \qw 		& \targ{}	& \targ{}	& \qw & \rstick{$0$} \\
	\lstick{$a_4$} & \targ{}   & \qw	   & \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}  & \targ{}  	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw      & \targ{}	& \targ{}	& \ctrl{-9}& \targ{}			& \qw 	& \qw		& \qw 		& \qw 		& \qw 		& \qw		& \qw & \rstick{$s_4$} \\		
	\lstick{$b_4$} & \ctrl{-1} & \ctrl{1}  & \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \ctrl{1}  & \ctrl{-1}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}  & \ctrl{-1}	& \qw	 	& \qw		& \gate{\ket{0}}	& \qw 	& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{\ket{0}} \\		
	\lstick{\ket{0}}& \qw      & \targ{}   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw 		& \targ{}  	& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \qw 		& \targ{}	& \ctrl{-2}	& \targ{}			& \qw 	& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{-3}	& \qw & \rstick{$s_5$}
\end{quantikz}
}

\newcommand{\QMAsingleZero}{
\begin{quantikz} [row sep= 0.1cm, column sep= 0.05cm, transparent]
	\lstick{\ket{0}}& \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw       & \qw		& \qw 		& \targ{}	& \qw  				& \qw 	& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw & \rstick{$m_0$} \\
	\lstick{$a_0$} & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \targ{  }	& \qw 		& \qw       & \qw		& \qw 		& \qw 		& \qw  				& \qw 	& \ctrl{1}	& \ctrl{-1}	& \qw 		& \qw 		& \qw 		& \qw & \rstick{$s_0$} \\
	\lstick{$b_0$} & \qw	   & \qw 	   & \qw 		& \qw 		& \qw 		& \ctrl{2}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \qw 		& \qw       & \qw		& \qw 		& \qw 		& \gate{\ket{0}}	& \qw 	& \targ{}	& \ctrl{1}	& \targ{  } & \qw 		& \qw 		& \qw & \rstick{$m_1$} \\
	\lstick{$a_1$} & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \targ{  }	& \qw       & \qw		& \qw 		& \qw 		& \qw  				& \qw 	& \qw 		& \ctrl{1}	& \ctrl{-1}	& \qw 		& \qw 		& \qw & \rstick{$s_1$} \\
	\lstick{$b_1$} & \ctrl{-1} & \qw	   & \qw 		& \qw 		& \ctrl{2}	& \targ{}	& \ctrl{2}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \targ{}	& \ctrl{2}	& \ctrl{-1}	& \qw       & \qw		& \qw 		& \qw 		& \gate{\ket{0}}	& \qw 	& \qw 		& \targ{}	& \ctrl{1}	& \targ{  }	& \qw 		& \qw & \rstick{$m_2$} \\
	\lstick{$a_2$} & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{  } & \qw		& \qw 		& \qw 		& \qw  				& \qw 	& \qw 		& \qw 		& \ctrl{1}	& \ctrl{-1}	& \qw 		& \qw & \rstick{$s_2$} \\
	\lstick{$b_2$} & \ctrl{-1} & \qw	   & \qw 		& \ctrl{2}	& \targ{}	& \qw 		& \targ{}	& \ctrl{2}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \targ{}	& \ctrl{2}	& \ctrl{-1} & \qw		& \qw 		& \qw 		& \gate{\ket{0}}	& \qw 	& \qw 		& \qw 		& \targ{}	& \ctrl{1}	& \targ{  }	& \qw & \rstick{$m_3$} \\
	\lstick{$a_3$} & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw  		& \qw  		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw       & \targ{}	& \qw 		& \qw 		& \qw  				& \qw 	& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \ctrl{-1}	& \qw & \rstick{$s_3$} \\
	\lstick{$b_3$} & \ctrl{-1} & \qw	   & \ctrl{2}  	& \targ{}	& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{2}	& \qw  		& \qw  		& \ctrl{2}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{2}  & \ctrl{-1}	& \qw 		& \qw 		& \gate{\ket{0}}	& \qw 	& \qw 		& \qw 		& \qw 		& \targ{}	& \targ{}	& \qw & \rstick{$m_4$} \\
	\lstick{$a_4$} & \targ{}   & \qw	   & \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}  & \targ{}  	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw       & \targ{}	& \targ{}	& \ctrl{-9} & \targ{}			& \qw 	& \qw		& \qw 		& \qw 		& \qw 		& \qw		& \qw & \rstick{$s_4$} \\		
	\lstick{$b_4$} & \ctrl{-1} & \ctrl{1}  & \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \ctrl{1}  & \ctrl{-1}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}   & \ctrl{-1}	& \qw	 	& \qw		& \gate{\ket{0}}	& \qw 	& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{\ket{0}} \\		
	\lstick{\ket{0}}& \qw      & \targ{}   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw 		& \targ{}  	& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw       & \qw 		& \targ{}	& \ctrl{-2}	& \targ{}			& \qw 	& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{-3}	& \qw & \rstick{$s_5$}
\end{quantikz}
}

\newcommand{\QMAdoubleZero}{
\begin{quantikz} [row sep= 0.1cm, column sep= 0.05cm, transparent]
	\lstick{\ket{0}}& \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 			& \qw       	& \qw			& \qw 			& \targ{}	& \qw  				& \qw 	& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw & \rstick{$m_0$} \\
	\lstick{$a_0$} & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \targ{  }	& \qw 			& \qw       	& \qw			& \qw 			& \qw 		& \qw  				& \qw 	& \ctrl{1}	& \ctrl{-1}	& \qw 		& \qw 		& \qw 		& \qw & \rstick{$s_0$} \\
	\lstick{$b_0$} & \qw	   & \qw 	   & \qw 		& \qw 		& \qw 		& \ctrl{2}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \gate{\ket{0}}& \qw       	& \qw			& \qw 			& \qw 		& \gate{\ket{0}}	& \qw 	& \targ{}	& \ctrl{1}	& \targ{  } & \qw 		& \qw 		& \qw & \rstick{$m_1$} \\
	\lstick{$a_1$} & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \targ{  }		& \qw       	& \qw			& \qw 			& \qw 		& \qw  				& \qw 	& \qw 		& \ctrl{1}	& \ctrl{-1}	& \qw 		& \qw 		& \qw & \rstick{$s_1$} \\
	\lstick{$b_1$} & \ctrl{-1} & \qw	   & \qw 		& \qw 		& \ctrl{2}	& \targ{}	& \ctrl{2}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \targ{}	& \ctrl{2}	& \ctrl{-1}		& \gate{\ket{0}}& \qw			& \qw 			& \qw 		& \gate{\ket{0}}	& \qw 	& \qw 		& \targ{}	& \ctrl{1}	& \targ{  }	& \qw 		& \qw & \rstick{$m_2$} \\
	\lstick{$a_2$} & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 			& \targ{  } 	& \qw			& \qw 			& \qw 		& \qw  				& \qw 	& \qw 		& \qw 		& \ctrl{1}	& \ctrl{-1}	& \qw 		& \qw & \rstick{$s_2$} \\
	\lstick{$b_2$} & \ctrl{-1} & \qw	   & \qw 		& \ctrl{2}	& \targ{}	& \qw 		& \targ{}	& \ctrl{2}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \targ{}	& \ctrl{2}		& \ctrl{-1} 	& \gate{\ket{0}}& \qw 			& \qw 		& \gate{\ket{0}}	& \qw 	& \qw 		& \qw 		& \targ{}	& \ctrl{1}	& \targ{  }	& \qw & \rstick{$m_3$} \\
	\lstick{$a_3$} & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw  		& \qw  		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 			& \qw       	& \targ{}		& \qw 			& \qw 		& \qw  				& \qw 	& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \ctrl{-1}	& \qw & \rstick{$s_3$} \\
	\lstick{$b_3$} & \ctrl{-1} & \qw	   & \ctrl{2}  	& \targ{}	& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{2}	& \qw  		& \qw  		& \ctrl{2}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}		& \ctrl{2}  	& \ctrl{-1}		& \gate{\ket{0}}& \qw 		& \gate{\ket{0}}	& \qw 	& \qw 		& \qw 		& \qw 		& \targ{}	& \targ{}	& \qw & \rstick{$m_4$} \\
	\lstick{$a_4$} & \targ{}   & \qw	   & \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}  & \targ{}  	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw			& \qw       	& \targ{}		& \targ{}		& \ctrl{-9} & \targ{}			& \qw 	& \qw		& \qw 		& \qw 		& \qw 		& \qw		& \qw & \rstick{$s_4$} \\		
	\lstick{$b_4$} & \ctrl{-1} & \ctrl{1}  & \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \ctrl{1}  & \ctrl{-1}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw			& \targ{}   	& \ctrl{-1}		& \qw	 		& \qw		& \gate{\ket{0}}	& \qw 	& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{\ket{0}} \\		
	\lstick{\ket{0}}& \qw      & \targ{}   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw 		& \targ{}  	& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 			& \qw       	& \qw 			& \targ{}		& \ctrl{-2}	& \targ{}			& \qw 	& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{-3}	& \qw & \rstick{$s_5$}
\end{quantikz}
}

==> ISCAS2024_Xtalk_attack_RNS_distributed_quantum/latex_images/xtalk_attacks.tex <==
\usepackage{tikz}
\usepackage{quantikz}
\usepackage{amsmath}

\newcommand{\rowSep}{0.25cm}
\newcommand{\colSep}{0.2cm}
\tikzset{slice/.append style={draw=blue}}
%\tikzset{slice/.append label style={blue}}

\newcommand{\myCnot}{
\begin{quantikz} [row sep= \rowSep, column sep= \colSep]
	\lstick{$a$} & \ctrl{1} & \qw & \rstick{$a$}\\
	\lstick{$b$} & \targ{}  & \qw & \rstick{$a \oplus b$}
\end{quantikz}
}

\newcommand{\mySwap}{
\begin{quantikz}
	\qw & \swap{1} & \qw \\
	\qw & \targX{} & \qw
\end{quantikz} = \begin{quantikz}
	\qw & \ctrl{1} & \targ{} 	& \ctrl{1} & \qw \\
	\qw & \targ{}  & \ctrl{-1} 	& \targ{}  & \qw
\end{quantikz}
}

\newcommand{\myToffoli}{
\begin{quantikz} [row sep= \rowSep, column sep= \colSep]
	\lstick{$a$} & \ctrl{1} & \qw & \rstick{$a$} \\
	\lstick{$b$} & \ctrl{1} & \qw & \rstick{$b$} \\
	\lstick{$c$} & \targ{}  & \qw & \rstick{$a \cdot b \oplus c$}
\end{quantikz}
}

\newcommand{\attackCNOT}{
	\begin{quantikz} [row sep= \rowSep, column sep= \colSep, transparent]
		\lstick{\ket{1}} & \ctrl{1} 	& \qw	\slice{n=1}   & \qw & \ctrl{1} 	& \qw	\slice{n=2}   & \qw & \ctrl{1} 	& \qw	\slice{n=3}   & \qw & \ctrl{1} 	& \qw	\slice{n=4}   & \qw & \ctrl{1} 	& \qw	\slice{n=5}   & \qw & \ctrl{1} 	& \qw	\slice{n=6}   & \qw & \ctrl{1} & \rstick{} \\
		\lstick{\ket{x}} & \targ{ } 	& \qw	              & \qw & \targ{ } 	& \qw	              & \qw & \targ{ } 	& \qw	              & \qw & \targ{ } 	& \qw	              & \qw & \targ{ } 	& \qw	              & \qw & \targ{ } 	& \qw	              & \qw & \targ{ } & \rstick{}
	\end{quantikz}
}

\newcommand{\attackCNOTtwo}{
	\begin{quantikz} [row sep= \rowSep, column sep= \colSep, transparent]
		\lstick{\ket{1}} & \ctrl{1} 	& \qw & \qw	\slice{n=1}   & \qw & \qw & \ctrl{1} 	& \qw & \qw	\slice{n=2}   & \qw & \ctrl{1} 	& \qw & \qw	\slice{n=3}   & \qw & \qw & \ctrl{1} 	& \qw & \qw	\slice{n=4} 	& \qw & \rstick{} \\
		\lstick{\ket{x}} & \targ{ } 	& \qw & \qw	              & \qw & \qw & \targ{ } 	& \qw & \qw	              & \qw & \targ{ } 	& \qw & \qw	              & \qw & \qw & \targ{ } 	& \qw & \qw	            	& \qw & \rstick{}
	\end{quantikz}
}


\newcommand{\attackAltCNOT}{
	\begin{quantikz} [row sep= \rowSep, column sep= \colSep, transparent]
		\lstick{\ket{1}} & \ctrl{1} 	& \targ{  } 	& \targ{} 	& \ctrl{1} 	& \qw	\slice{n=1}   & \qw & \qw{} 	& \targ{  }		& \qw	\slice{n=2}   & \qw & \targ{} 	& \ctrl{1} 	& \qw	\slice{n=3}   & \qw & \qw{} 	& \targ{  }  	& \qw	\slice{n=4}   & \qw & \rstick{} \\
		\lstick{\ket{x}} & \targ{ } 	& \ctrl{-1} 	& \qw    	& \targ{ } 	& \qw	              & \qw & \targ{} 	& \ctrl{-1}		& \qw	              & \qw & \qw    	& \targ{ } 	& \qw	              & \qw & \targ{} 	& \ctrl{-1} 	& \qw	              & \qw & \rstick{}
	\end{quantikz}
}

\newcommand{\attackSAC}{
	\begin{quantikz} [row sep= \rowSep, column sep= \colSep, transparent]
		\lstick{\ket{1}} & \gate{H} 	& \ctrl{1} 	& \targ{  } 	& \qw	\slice{n=1}   & \qw & \ctrl{1} 	& \targ{  } & \qw	\slice{n=2}   & \qw & \ctrl{1} 	& \targ{  } 	& \qw	\slice{n=3}   & \qw & \ctrl{1} 	& \targ{  } & \qw	\slice{n=4}   & \qw & \ctrl{1} 	& \targ{  }  & \qw	\slice{n=5}   & \qw 	 & \rstick{} \\
		\lstick{\ket{x}} & \gate{H} 	& \targ{ } 	& \ctrl{-1} 	& \qw	              & \qw & \targ{ } 	& \ctrl{-1} & \qw	              & \qw & \targ{ } 	& \ctrl{-1} 	& \qw	              & \qw & \targ{ } 	& \ctrl{-1} & \qw	              & \qw & \targ{ } 	& \ctrl{-1}  & \qw	              & \qw 	 & \rstick{}
	\end{quantikz}
}

\newcommand{\attackSACtwo}{
	\begin{quantikz} [row sep= \rowSep, column sep= \colSep, transparent]
		\lstick{\ket{1}} & \gate{H} 	& \ctrl{1} 	& \targ{  } 	& \qw	\slice{n=1}   & \qw & \ctrl{1} 	& \targ{  } & \qw	\slice{n=2}   & \qw & \ctrl{1} 	& \targ{  } 	& \qw	\slice{n=3}   & \qw & \ctrl{1} 	& \targ{  } & \qw	\slice{n=4} & \qw 	 & \rstick{} \\
		\lstick{\ket{x}} & \gate{H} 	& \targ{ } 	& \ctrl{-1} 	& \qw	              & \qw & \targ{ } 	& \ctrl{-1} & \qw	              & \qw & \targ{ } 	& \ctrl{-1} 	& \qw	              & \qw & \targ{ } 	& \ctrl{-1} & \qw	            & \qw 	 & \rstick{}
	\end{quantikz}
}

\newcommand{\attackAPC}{
	\begin{quantikz} [row sep= \rowSep, column sep= \colSep, transparent]
		\lstick{\ket{1}} & \gate{H} & \ctrl{1} 	& \gate{R\textsubscript{Y}(\pi)} 	& \ctrl{1} 						 & \qw	\slice{n=1}   & \qw & \targ{  } & \ctrl{1} 								& \gate{R\textsubscript{Z}(\pi)} 	& \qw	\slice{n = 2} & \qw & \ctrl{1} 	& \gate{R\textsubscript{Y}(\pi)}	& \ctrl{1} 						 & \qw	\slice{n = 3} & \qw 	& \rstick{} \\
		\lstick{\ket{x}} & \gate{H} & \targ{ } 	& \ctrl{-1} 						& \gate{R\textsubscript{Z}(\pi)} & \qw	              & \qw & \ctrl{-1} & \gate{R\textsubscript{Y}(\pi)} 	    & \ctrl{-1} 						& \qw	              & \qw & \targ{ } 	& \ctrl{-1} 						& \gate{R\textsubscript{Z}(\pi)} & \qw	              & \qw  	& \rstick{}
	\end{quantikz}
}

\newcommand{\attackAPCtwo}{
	\begin{quantikz} [row sep= \rowSep, column sep= \colSep, transparent]
		\lstick{\ket{1}} & \gate{H} & \ctrl{1} 	& \gate{R\textsubscript{Y}(\pi)} 	& \ctrl{1} 						 & \qw	\slice{n=1}   & \qw & \targ{  } & \ctrl{1} 								& \gate{R\textsubscript{Z}(\pi)} 	& \qw	\slice{n = 2} & \qw & \rstick{} \\
		\lstick{\ket{x}} & \gate{H} & \targ{ } 	& \ctrl{-1} 						& \gate{R\textsubscript{Z}(\pi)} & \qw	              & \qw & \ctrl{-1} & \gate{R\textsubscript{Y}(\pi)} 	    & \ctrl{-1} 						& \qw	              & \qw	& \rstick{}
	\end{quantikz}
}

==> ISCAS2024_Xtalk_attack_RNS_distributed_quantum/xtalk_attacks.tex <==
\usepackage{tikz}
\usepackage{quantikz}
\usepackage{amsmath}

\newcommand{\rowSep}{0.25cm}
\newcommand{\rowSepT}{0.4cm}
\newcommand{\colSep}{0.2cm}
\newcommand{\colSepT}{0.16cm}
\tikzset{slice/.append style={draw=blue}}
%\tikzset{slice/.append label style={blue}}

\newcommand{\myCnot}{
\begin{quantikz} [row sep= \rowSep, column sep= \colSep]
	\lstick{$a$} & \ctrl{1} & \qw & \rstick{$a$}\\
	\lstick{$b$} & \targ{}  & \qw & \rstick{$a \oplus b$}
\end{quantikz}
}

\newcommand{\mySwap}{
\begin{quantikz}
	\qw & \swap{1} & \qw \\
	\qw & \targX{} & \qw
\end{quantikz} = \begin{quantikz}
	\qw & \ctrl{1} & \targ{} 	& \ctrl{1} & \qw \\
	\qw & \targ{}  & \ctrl{-1} 	& \targ{}  & \qw
\end{quantikz}
}

\newcommand{\myToffoli}{
\begin{quantikz} [row sep= \rowSep, column sep= \colSep]
	\lstick{$a$} & \ctrl{1} & \qw & \rstick{$a$} \\
	\lstick{$b$} & \ctrl{1} & \qw & \rstick{$b$} \\
	\lstick{$c$} & \targ{}  & \qw & \rstick{$a \cdot b \oplus c$}
\end{quantikz}
}

\newcommand{\attackCNOT}{
\begin{quantikz} [row sep= \rowSep, column sep= \colSep, transparent]
	\lstick{$\ket{1}$} & \ctrl{1} 	& \qw	\slice{n=1}   & \qw & \ctrl{1} 	& \qw	\slice{n=2}   & \qw & \ctrl{1} 	& \qw	\slice{n=3}   & \qw & \ctrl{1} 	& \qw	\slice{n=4}   & \qw & \ctrl{1} 	& \qw	\slice{n=5}   & \qw & \ctrl{1} 	& \qw	\slice{n=6}   & \qw & \ctrl{1} & \rstick{} \\
	\lstick{$\ket{x}$} & \targ{ } 	& \qw	              & \qw & \targ{ } 	& \qw	              & \qw & \targ{ } 	& \qw	              & \qw & \targ{ } 	& \qw	              & \qw & \targ{ } 	& \qw	              & \qw & \targ{ } 	& \qw	              & \qw & \targ{ } & \rstick{}
\end{quantikz}
}

\newcommand{\attackCNOTtwo}{
	\begin{quantikz} [row sep= \rowSepT, column sep= 0.215cm, transparent]
		\lstick{$\ket{1}$}  & \ctrl{1} 	& \qw & \qw	\slice{n=1}   & \qw & \qw & \ctrl{1} 	& \qw & \qw	\slice{n=2}   & \qw & \qw & \ctrl{1} 	& \qw & \qw	\slice{n=3}   & \qw & \qw & \ctrl{1} 	& \qw & \qw	\slice{n=4} 	& \qw & \qw & \ctrl{1} 	& \qw & \qw	\slice{n=5} 	& \qw & \rstick{} \\
		\lstick{$\ket{x}$}  & \targ{ } 	& \qw & \qw	              & \qw & \qw & \targ{ } 	& \qw & \qw	              & \qw & \qw & \targ{ } 	& \qw & \qw	              & \qw & \qw & \targ{ } 	& \qw & \qw	            	& \qw & \qw & \targ{ } 	& \qw & \qw	            	& \qw & \rstick{}
	\end{quantikz}
}


\newcommand{\attackAltCNOT}{
	\begin{quantikz} [row sep= \rowSepT, column sep= \colSep, transparent]
		\lstick{$\ket{1}$} & \ctrl{1} 	& \targ{  } 	& \targ{} 	& \ctrl{1} 	& \qw	\slice{n=1}   & \qw & \qw{} 	& \targ{  }		& \qw	\slice{n=2}   & \qw & \targ{} 	& \ctrl{1} 	& \qw	\slice{n=3}   & \qw & \qw{} 	& \targ{  }  	& \qw	\slice{n=4}   & \qw & \rstick{} \\
		\lstick{$\ket{x}$} & \targ{ } 	& \ctrl{-1} 	& \qw    	& \targ{ } 	& \qw	              & \qw & \targ{} 	& \ctrl{-1}		& \qw	              & \qw & \qw    	& \targ{ } 	& \qw	              & \qw & \targ{} 	& \ctrl{-1} 	& \qw	              & \qw & \rstick{}
	\end{quantikz}
}

\newcommand{\attackSAC}{
	\begin{quantikz} [row sep= \rowSep, column sep= \colSep, transparent]
		\lstick{$\ket{1}$} & \gate{H} 	& \ctrl{1} 	& \targ{  } 	& \qw	\slice{n=1}   & \qw & \ctrl{1} 	& \targ{  } & \qw	\slice{n=2}   & \qw & \ctrl{1} 	& \targ{  } 	& \qw	\slice{n=3}   & \qw & \ctrl{1} 	& \targ{  } & \qw	\slice{n=4}   & \qw & \ctrl{1} 	& \targ{  }  & \qw	\slice{n=5}   & \qw 	 & \rstick{} \\
		\lstick{$\ket{x}$} & \gate{H} 	& \targ{ } 	& \ctrl{-1} 	& \qw	              & \qw & \targ{ } 	& \ctrl{-1} & \qw	              & \qw & \targ{ } 	& \ctrl{-1} 	& \qw	              & \qw & \targ{ } 	& \ctrl{-1} & \qw	              & \qw & \targ{ } 	& \ctrl{-1}  & \qw	              & \qw 	 & \rstick{}
	\end{quantikz}
}

\newcommand{\attackSACtwo}{
	\begin{quantikz} [row sep= \rowSep, column sep= \colSep, transparent]
		\lstick{$\ket{1}$} & \qw  & \gate{H} 	& \ctrl{1} 	& \targ{  } 	& \qw	\slice{n=1}   & \qw & \ctrl{1} 	& \targ{  } & \qw	\slice{n=2}   & \qw & \ctrl{1} 	& \targ{  } 	& \qw	\slice{n=3}   & \qw & \ctrl{1} 	& \targ{  } & \qw	\slice{n=4} & \qw 	 & \rstick{} \\
		\lstick{$\ket{x}$} & \qw  & \gate{H} 	& \targ{ } 	& \ctrl{-1} 	& \qw	              & \qw & \targ{ } 	& \ctrl{-1} & \qw	              & \qw & \targ{ } 	& \ctrl{-1} 	& \qw	              & \qw & \targ{ } 	& \ctrl{-1} & \qw	            & \qw 	 & \rstick{}
	\end{quantikz}
}

\newcommand{\attackAPC}{
	\begin{quantikz} [row sep= \rowSep, column sep= \colSep, transparent]
		\lstick{$\ket{1}$} & \gate{H} & \ctrl{1} 	& \gate{R\textsubscript{Y}(\pi)} 	& \ctrl{1} 						 & \qw	\slice{n=1}   & \qw & \targ{  } & \ctrl{1} 								& \gate{R\textsubscript{Z}(\pi)} 	& \qw	\slice{n = 2} & \qw & \ctrl{1} 	& \gate{R\textsubscript{Y}(\pi)}	& \ctrl{1} 						 & \qw	\slice{n = 3} & \qw 	& \rstick{} \\
		\lstick{$\ket{x}$} & \gate{H} & \targ{ } 	& \ctrl{-1} 						& \gate{R\textsubscript{Z}(\pi)} & \qw	              & \qw & \ctrl{-1} & \gate{R\textsubscript{Y}(\pi)} 	    & \ctrl{-1} 						& \qw	              & \qw & \targ{ } 	& \ctrl{-1} 						& \gate{R\textsubscript{Z}(\pi)} & \qw	              & \qw  	& \rstick{}
	\end{quantikz}
}

\newcommand{\attackAPCtwo}{
	\begin{quantikz} [row sep= \rowSep, column sep= \colSepT, transparent]
		\lstick{$\ket{1}$} & \qw & \gate{H} & \ctrl{1} 	& \gate{R\textsubscript{Y}(\pi)} 	& \ctrl{1} 						 & \qw	\slice{n=1}   & \qw & \targ{  } & \ctrl{1} 								& \gate{R\textsubscript{Z}(\pi)} 	& \qw	\slice{n = 2} & \qw & \rstick{} \\
		\lstick{$\ket{x}$} & \qw & \gate{H} & \targ{ } 	& \ctrl{-1} 						& \gate{R\textsubscript{Z}(\pi)} & \qw	              & \qw & \ctrl{-1} & \gate{R\textsubscript{Y}(\pi)} 	    & \ctrl{-1} 						& \qw	              & \qw	& \rstick{}
	\end{quantikz}
}

==> latex_images/quantikz_figures1.tex <==
\usepackage{tikz}
\usepackage{quantikz}
\usepackage{amsmath}


\newcommand{\rowSep}{0.6cm}
\newcommand{\colSep}{0.2cm}

\newcommand{\myCnot}{
\begin{quantikz} [row sep= \rowSep, column sep= \colSep]
	\lstick{$a$} & \qw	& \ctrl{1} & \qw & \rstick{$a$}\\
	\lstick{$b$} & \qw	& \targ{}  & \qw & \rstick{$a \oplus b$}
\end{quantikz}
}

\newcommand{\myToffoli}{
\begin{quantikz} [row sep= \rowSep, column sep= \colSep]
	\lstick{$a$} & \ctrl{1} & \qw & \rstick{$a$} \\
	\lstick{$b$} & \ctrl{1} & \qw & \rstick{$b$} \\
	\lstick{$c$} & \targ{}  & \qw & \rstick{$a \cdot b \oplus c$}
\end{quantikz}
}

\newcommand{\QMAone}{
%\begin{quantikz} [row sep= 0.06cm, column sep= 0.025cm, transparent]
	%\gategroup[17,steps=22,style={blue!75!black, ultra thick, dashed, rounded corners, inner xsep=2pt}, background]{{\sc Quantum Full Adder}}
\begin{quantikz} [row sep= {0.5cm, between origins}, column sep= {0.05cm}, transparent]
	\lstick{$\ket{0}$}   & \qw	& \qw\gategroup[17,steps=22,style={blue!75!black, ultra thick, dashed, rounded corners, inner xsep=-2pt}, background]{{\sc Quantum Full Adder}}		& \qw		& \qw	    & \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw	& \qw		& \qw	& \qw	& \qw	& \qw\gategroup[17,steps=3,style={green!50!black, ultra thick, dashed, rounded corners, inner xsep=-3pt}, background]{{\sc NOR}} 		& \targ{}	& \qw 		& \qw	& \qw	& \qw	& \qw	& \qw\gategroup[17,steps=22,style={blue!75!black, ultra thick, dashed, rounded corners, inner xsep=-2pt}, background]{{\sc Quantum Full Adder}} 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw		& \qw 		& \qw 		& \targ{}	& \qw & \rstick{$m_0$} \\
	\lstick{$a_0$} 		 & \qw	& \qw	    & \qw	   	& \qw		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw		& \qw 		& \qw      & \targ{}	& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw 		& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \qw		& \qw 		& \qw 		& \ctrl{-1}	& \qw & \rstick{$s_0$} \\
	\lstick{$b_0$} 		 & \qw	& \qw	    & \qw 	   	& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \qw		& \qw 		& \qw      & \ctrl{-1}	& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw 		& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_0$} \\
	\lstick{$\ket{0}$}   & \qw	& \qw	    & \qw	   	& \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw 		& \qw	& \qw	& \qw	& \qw	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw		& \qw 		& \targ{}	& \qw & \rstick{$m_1$} \\
	\lstick{$a_1$} 		 & \qw	& \targ{} 	& \qw	   	& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw 		& \qw	& \qw	& \qw	& \qw	& \ctrl{-1}	& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \targ{}	& \ctrl{3}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \ctrl{3}	& \qw		& \qw 		& \ctrl{-1}	& \qw & \rstick{$s_1$} \\
	\lstick{$b_1$} 		 & \qw	& \ctrl{-1} & \qw	   	& \qw 		& \qw 		& \ctrl{3}	& \targ{}	& \ctrl{3}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \ctrl{3}	& \qw 		& \qw      & \ctrl{-1}	& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw 		& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_1$} \\
	\lstick{$\ket{0}$}   & \qw	& \qw	   	& \qw	   	& \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw 		& \qw	& \qw	& \qw	& \qw	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \qw & \rstick{$m_2$} \\
	\lstick{$a_2$} 		 & \qw	& \targ{} 	& \qw	   	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw 		& \qw	& \qw	& \qw	& \qw	& \ctrl{-1}	& \qw 		& \qw 		& \ctrl{3}	& \targ{}	& \qw 		& \targ{}	& \ctrl{3}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \targ{}	& \ctrl{3}	& \qw 		& \ctrl{-1}	& \qw & \rstick{$s_2$} \\
	\lstick{$b_2$} 		 & \qw	& \ctrl{-1} & \qw	   	& \qw 		& \ctrl{3}	& \targ{}	& \qw 		& \targ{}	& \ctrl{3}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \targ{}	& \ctrl{3}	& \qw      & \ctrl{-1}	& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw 		& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_2$} \\
	\lstick{$\ket{0}$}   & \qw	& \qw	   	& \qw	   	& \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw 		& \qw	& \qw	& \qw	& \qw	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \qw & \rstick{$m_3$} \\
	\lstick{$a_3$} 		 & \qw	& \targ{} 	& \qw	   	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw  		& \qw  		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw 		& \qw	& \qw	& \qw	& \qw	& \ctrl{-1}	& \qw 		& \ctrl{5}	& \targ{}	& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{5}	& \qw		& \qw 		& \ctrl{5}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{5}	& \ctrl{-1}	& \qw & \rstick{$s_3$} \\
	\lstick{$b_3$} 		 & \qw	& \ctrl{-1} & \qw	   	& \ctrl{3}  & \targ{}	& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{3}	& \qw  		& \qw  		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{3} & \ctrl{-1}	& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw 		& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_3$} \\
	\lstick{$\ket{0}$}   & \qw	& \qw	   	& \qw	   	& \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw 		& \qw	& \qw	& \qw	& \qw	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \qw & \rstick{$m_4$} \\
	\lstick{$a_4$} 		 & \qw	& \targ{} 	& \qw	   	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}  & \targ{}  	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw      & \targ{}	& \qw	& \qw	& \qw	& \qw	& \targ{}	& \ctrl{-13}& \targ{}	& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$s_4$} \\		
	\lstick{$b_4$} 		 & \qw	& \ctrl{-1} & \ctrl{1}  & \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \ctrl{1}  & \ctrl{-1}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}  & \ctrl{-1}	& \qw	& \qw	& \qw	& \qw	& \qw	 	& \qw		& \qw		& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_4$} \\		
	\lstick{$\ket{0}$}   & \qw	& \qw     	& \targ{}   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw 		& \targ{}  	& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \qw 		& \qw	& \qw	& \qw	& \qw	& \targ{}	& \ctrl{-2}	& \targ{}	& \qw	& \qw	& \qw	& \qw	& \ctrl{-3}	& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{1}	& \ctrl{-3}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{-3}	& \qw & \rstick{$s_5$} \\
	\lstick{$\ket{0}$}   & \qw	& \qw	   	& \qw	   	& \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw	& \qw	& \qw	& \qw	& \qw	 	& \qw		& \qw		& \qw	& \qw	& \qw	& \qw	& \qw 		& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$s_6$}			
\end{quantikz}
}

\newcommand{\QMAtwo}{
%\begin{quantikz} [row sep= 0.02cm, column sep= 0.01cm, transparent]
\begin{quantikz} [row sep= {0.5cm, between origins}, column sep= {0.05cm}, transparent]
	\lstick{$\ket{0}$}  & \qw	 & \qw\gategroup[16,steps=22,style={blue!75!black, ultra thick, dashed, rounded corners, inner xsep=-2pt}, background]{{\sc Quantum Full Adder}}	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw	& \qw	& \qw	& \qw	& \qw\gategroup[16,steps=3,style={green!50!black, ultra thick, dashed, rounded corners, inner xsep=-3pt}, background]{{\sc NOR}} 		& \targ{}	& \qw  		& \qw	& \qw	& \qw	& \qw\gategroup[16,steps=6,style={red!70!green!40!blue!80, ultra thick, dashed, rounded corners, inner xsep=-3pt}, background]{{\sc Half Adder}}	& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$m_0$} \\
	\lstick{$a_0$} 		& \qw	 & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw		& \qw 		& \qw      & \targ{}	& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw  		& \qw	& \qw	& \qw	& \qw	& \ctrl{2}	& \ctrl{-1}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$s_0$} \\
	\lstick{$b_0$} 		& \qw	 & \qw	   & \qw 	   & \qw 		& \qw 		& \qw 		& \ctrl{3}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \qw		& \qw 		& \qw      & \ctrl{-1}	& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw  		& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_0$} \\
	\lstick{$\ket{0}$}  & \qw	 & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw  		& \qw	& \qw	& \qw	& \qw	& \targ{}	& \ctrl{1}	& \targ{  }	& \qw 		& \qw 		& \qw 		& \qw & \rstick{$m_1$} \\
	\lstick{$a_1$} 		& \qw	 & \targ{} & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw  		& \qw	& \qw	& \qw	& \qw	& \qw 		& \ctrl{2}	& \ctrl{-1}	& \qw 		& \qw 		& \qw 		& \qw & \rstick{$s_1$} \\
	\lstick{$b_1$} 		& \qw	& \ctrl{-1}& \qw	   & \qw 		& \qw 		& \ctrl{3}	& \targ{}	& \ctrl{3}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \ctrl{3}	& \qw 		& \qw      & \ctrl{-1}	& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw  		& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_1$} \\
	\lstick{$\ket{0}$}  & \qw	 & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw  		& \qw	& \qw	& \qw	& \qw	& \qw 		& \targ{}	& \ctrl{1}	& \targ{  }	& \qw 		& \qw 		& \qw & \rstick{$m_2$} \\
	\lstick{$a_2$} 		& \qw	& \targ{}  & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw  		& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \qw 		& \qw 		& \qw & \rstick{$s_2$} \\
	\lstick{$b_2$} 		& \qw	& \ctrl{-1}& \qw	   & \qw 		& \ctrl{3}	& \targ{}	& \qw 		& \targ{}	& \ctrl{3}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \targ{}	& \ctrl{3}	& \qw      & \ctrl{-1}	& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw  		& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_2$} \\
	\lstick{$\ket{0}$}  & \qw	 & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw  		& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \targ{}	& \ctrl{1}	& \targ{  }	& \qw 		& \qw & \rstick{$m_3$} \\
	\lstick{$a_3$} 		& \qw	 & \targ{} & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw  		& \qw  		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw  		& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \qw 		& \qw & \rstick{$s_3$} \\
	\lstick{$b_3$} 		& \qw	& \ctrl{-1}& \qw	   & \ctrl{3}  	& \targ{}	& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{3}	& \qw  		& \qw  		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{3} & \ctrl{-1}	& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw  		& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_3$} \\
	\lstick{$\ket{0}$}  & \qw	 & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw  		& \qw	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw 		& \targ{}	& \targ{}	& \qw 		& \qw & \rstick{$m_4$} \\
	\lstick{$a_4$} 		& \qw	 & \targ{} & \qw	   & \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}  & \targ{}  	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw      & \targ{}	& \qw	& \qw	& \qw	& \qw	& \targ{}	& \ctrl{-13}& \targ{}	& \qw	& \qw	& \qw	& \qw	& \qw		& \qw 		& \qw 		& \qw 		& \qw		& \qw 		& \qw & \rstick{$s_4$} \\		
	\lstick{$b_4$} 		& \qw	& \ctrl{-1}& \ctrl{1}  & \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \ctrl{1}  & \ctrl{-1}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}  & \ctrl{-1}	& \qw	& \qw	& \qw	& \qw	& \qw	 	& \qw		& \qw  		& \qw	& \qw	& \qw	& \qw	& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_4$} \\		
	\lstick{$\ket{0}$}  & \qw	 & \qw     & \targ{}   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw 		& \targ{}  	& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \qw 		& \qw	& \qw	& \qw	& \qw	& \targ{}	& \ctrl{-2}	& \targ{}	& \qw	& \qw	& \qw	& \qw	& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{-3}	& \qw 		& \qw & \rstick{$s_5$}
\end{quantikz}
}

\newcommand{\QMAtwobk}{
%\begin{quantikz} [row sep= 0.02cm, column sep= 0.01cm, transparent]
\begin{quantikz} [row sep= {0.5cm, between origins}, column sep= {0.05cm}, transparent]
	\lstick{$\ket{0}$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw 		& \targ{}	& \qw  		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$m_0$} \\
	\lstick{$a_0$} & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw		& \qw 		& \qw      & \targ{}	& \qw 		& \qw 		& \qw  		& \ctrl{2}	& \ctrl{-1}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$s_0$} \\
	\lstick{$b_0$} & \qw	   & \qw 	   & \qw 		& \qw 		& \qw 		& \ctrl{3}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \qw		& \qw 		& \qw      & \ctrl{-1}	& \qw 		& \qw 		& \qw  		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_0$} \\
	\lstick{$\ket{0}$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw 		& \qw 		& \qw  		& \targ{}	& \ctrl{1}	& \targ{  }	& \qw 		& \qw 		& \qw 		& \qw & \rstick{$m_1$} \\
	\lstick{$a_1$} & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw 		& \qw 		& \qw  		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \qw 		& \qw 		& \qw 		& \qw & \rstick{$s_1$} \\
	\lstick{$b_1$} & \ctrl{-1} & \qw	   & \qw 		& \qw 		& \ctrl{3}	& \targ{}	& \ctrl{3}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \ctrl{3}	& \qw 		& \qw      & \ctrl{-1}	& \qw 		& \qw 		& \qw  		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_1$} \\
	\lstick{$\ket{0}$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw 		& \qw 		& \qw  		& \qw 		& \targ{}	& \ctrl{1}	& \targ{  }	& \qw 		& \qw 		& \qw & \rstick{$m_2$} \\
	\lstick{$a_2$} & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw 		& \qw 		& \qw  		& \qw 		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \qw 		& \qw 		& \qw & \rstick{$s_2$} \\
	\lstick{$b_2$} & \ctrl{-1} & \qw	   & \qw 		& \ctrl{3}	& \targ{}	& \qw 		& \targ{}	& \ctrl{3}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \targ{}	& \ctrl{3}	& \qw      & \ctrl{-1}	& \qw 		& \qw 		& \qw  		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_2$} \\
	\lstick{$\ket{0}$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw 		& \qw 		& \qw  		& \qw 		& \qw 		& \targ{}	& \ctrl{1}	& \targ{  }	& \qw 		& \qw & \rstick{$m_3$} \\
	\lstick{$a_3$} & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw  		& \qw  		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw 		& \qw 		& \qw  		& \qw 		& \qw 		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \qw 		& \qw & \rstick{$s_3$} \\
	\lstick{$b_3$} & \ctrl{-1} & \qw	   & \ctrl{3}  	& \targ{}	& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{3}	& \qw  		& \qw  		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{3} & \ctrl{-1}	& \qw 		& \qw 		& \qw  		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_3$} \\
	\lstick{$\ket{0}$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw 		& \qw 		& \qw  		& \qw 		& \qw 		& \qw 		& \targ{}	& \targ{}	& \qw 		& \qw & \rstick{$m_4$} \\
	\lstick{$a_4$} & \targ{}   & \qw	   & \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}  & \targ{}  	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw      & \targ{}	& \targ{}	& \ctrl{-13}& \targ{}	& \qw		& \qw 		& \qw 		& \qw 		& \qw		& \qw 		& \qw & \rstick{$s_4$} \\		
	\lstick{$b_4$} & \ctrl{-1} & \ctrl{1}  & \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \ctrl{1}  & \ctrl{-1}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}  & \ctrl{-1}	& \qw	 	& \qw		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_4$} \\		
	\lstick{$\ket{0}$}   & \qw       & \targ{}   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw 		& \targ{}  	& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \qw 		& \targ{}	& \ctrl{-2}	& \targ{}	& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{-3}	& \qw 		& \qw & \rstick{$s_5$}
\end{quantikz}
}


\newcommand{\QMAthree}{
\begin{quantikz} [row sep= {0.5cm, between origins}, column sep= {0.05cm}, transparent]
	\lstick{$\ket{0}$}   	& \qw	    & \qw	   	& \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw	& \qw 		& \targ{}	& \qw  		& \qw				& \ctrl{1}		& \targ{}		& \qw 			& \qw 			& \qw 		& \qw 		& \qw & \rstick{$m_0$} \\
	\lstick{$a_0$} 			& \qw	    & \qw	   	& \qw		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw		& \qw 		& \qw      & \targ{}	& \qw	& \qw 		& \qw 		& \qw  		& \qw				& \ctrl{1}		& \ctrl{-1}		& \qw 			& \qw 			& \qw 		& \qw 		& \qw & \rstick{$s_0$} \\
	\lstick{$b_0$} 			& \qw	    & \qw 	   	& \qw 		& \qw 		& \qw 		& \ctrl{2}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{2}	& \qw		& \qw 		& \qw      & \ctrl{-1}	& \qw	& \qw 		& \qw 		& \qw  		& \gate{\ket{0}}	& \targ{}		& \ctrl{1}		& \targ{  }		& \qw 			& \qw 		& \qw 		& \qw & \rstick{$m_1$} \\
	\lstick{$a_1$} 			& \targ{}   & \qw	   	& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw	& \qw 		& \qw 		& \qw  		& \qw				& \qw 			& \ctrl{1}		& \ctrl{-1}		& \qw 			& \qw 		& \qw 		& \qw & \rstick{$s_1$} \\
	\lstick{$b_1$} 			& \ctrl{-1} & \qw	   	& \qw 		& \qw 		& \ctrl{2}	& \targ{}	& \ctrl{2}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \targ{}	& \ctrl{2}	& \qw 		& \qw      & \ctrl{-1}	& \qw	& \qw 		& \qw 		& \qw  		& \qw				& \gate{\ket{0}}& \targ{}		& \ctrl{1}		& \targ{  }		& \qw 		& \qw 		& \qw & \rstick{$m_2$} \\
	\lstick{$a_2$} 			& \targ{}   & \qw	   	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw	& \qw 		& \qw 		& \qw  		& \qw				& \qw 			& \qw 			& \ctrl{1}		& \ctrl{-1}		& \qw 		& \qw 		& \qw & \rstick{$s_2$} \\
	\lstick{$b_2$} 			& \ctrl{-1} & \qw	   	& \qw 		& \ctrl{2}	& \targ{}	& \qw 		& \targ{}	& \ctrl{2}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \targ{}	& \ctrl{2}	& \qw      & \ctrl{-1}	& \qw	& \qw 		& \qw 		& \qw  		& \qw				& \qw 			& \gate{\ket{0}}& \targ{}		& \ctrl{1}		& \targ{  }	& \qw 		& \qw & \rstick{$m_3$} \\
	\lstick{$a_3$} 			& \targ{}   & \qw	   	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw  		& \qw  		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw	& \qw 		& \qw 		& \qw  		& \qw				& \qw 			& \qw 			& \qw 			& \ctrl{1}		& \ctrl{-1}	& \qw 		& \qw & \rstick{$s_3$} \\
	\lstick{$b_3$} 			& \ctrl{-1} & \qw	   	& \ctrl{2}  & \targ{}	& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{2}	& \qw  		& \qw  		& \ctrl{2}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{2} & \ctrl{-1}	& \qw	& \qw 		& \qw 		& \qw  		& \qw				& \qw 			& \qw 			& \gate{\ket{0}}& \targ{}		& \targ{}	& \qw 		& \qw & \rstick{$m_4$} \\
	\lstick{$a_4$} 			& \targ{}   & \qw	   	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}  & \targ{}  	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw      & \targ{}	& \qw	& \targ{}	& \ctrl{-9} & \targ{}	& \qw				& \qw			& \qw 			& \qw 			& \qw 			& \qw		& \qw 		& \qw & \rstick{$s_4$} \\		
	\lstick{$b_4$} 			& \ctrl{-1} & \ctrl{1}  & \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \ctrl{1}  & \ctrl{-1}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}  & \ctrl{-1}	& \qw	& \qw	 	& \qw		& \qw  		& \qw				& \qw			& \qw 			& \qw 			& \gate{\ket{0}}& \qw 		& \qw 		& \qw & \rstick{$\ket{0}$} \\		
	\lstick{$\ket{0}$}   	& \qw       & \targ{}   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw 		& \targ{}  	& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \qw 		& \qw	& \targ{}	& \ctrl{-2}	& \targ{}	& \qw				& \qw			& \qw 			& \qw 			& \qw 			& \ctrl{-3}	& \qw 		& \qw & \rstick{$s_5$}
\end{quantikz}
}

\newcommand{\QMAfour}{
\begin{quantikz} [row sep= {0.5cm, between origins}, column sep= {0.05cm}, transparent]
	\lstick{$\ket{0}$}   	& \qw	    & \qw	   	& \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw	& \qw				& \qw	& \qw 		& \targ{}	& \qw  		& \qw				& \ctrl{1}		& \targ{}		& \qw 			& \qw 			& \qw 		& \qw 		& \qw & \rstick{$m_0$} \\
	\lstick{$a_0$} 			& \qw	    & \qw	   	& \qw		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw		& \qw 		& \qw      & \targ{}	& \qw	& \qw				& \qw	& \qw 		& \qw 		& \qw  		& \qw				& \ctrl{1}		& \ctrl{-1}		& \qw 			& \qw 			& \qw 		& \qw 		& \qw & \rstick{$s_0$} \\
	\lstick{$b_0$} 			& \qw	    & \qw 	   	& \qw 		& \qw 		& \qw 		& \ctrl{2}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{2}	& \qw		& \qw 		& \qw      & \ctrl{-1}	& \qw	& \gate{\ket{0}}	& \qw	& \qw 		& \qw 		& \qw  		& \gate{\ket{0}}	& \targ{}		& \ctrl{1}		& \targ{  }		& \qw 			& \qw 		& \qw 		& \qw & \rstick{$m_1$} \\
	\lstick{$a_1$} 			& \targ{}   & \qw	   	& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw	& \qw				& \qw	& \qw 		& \qw 		& \qw  		& \qw				& \qw 			& \ctrl{1}		& \ctrl{-1}		& \qw 			& \qw 		& \qw 		& \qw & \rstick{$s_1$} \\
	\lstick{$b_1$} 			& \ctrl{-1} & \qw	   	& \qw 		& \qw 		& \ctrl{2}	& \targ{}	& \ctrl{2}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \targ{}	& \ctrl{2}	& \qw 		& \qw      & \ctrl{-1}	& \qw	& \gate{\ket{0}}	& \qw	& \qw 		& \qw 		& \qw  		& \qw				& \gate{\ket{0}}& \targ{}		& \ctrl{1}		& \targ{  }		& \qw 		& \qw 		& \qw & \rstick{$m_2$} \\
	\lstick{$a_2$} 			& \targ{}   & \qw	   	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw	& \qw				& \qw	& \qw 		& \qw 		& \qw  		& \qw				& \qw 			& \qw 			& \ctrl{1}		& \ctrl{-1}		& \qw 		& \qw 		& \qw & \rstick{$s_2$} \\
	\lstick{$b_2$} 			& \ctrl{-1} & \qw	   	& \qw 		& \ctrl{2}	& \targ{}	& \qw 		& \targ{}	& \ctrl{2}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \targ{}	& \ctrl{2}	& \qw      & \ctrl{-1}	& \qw	& \gate{\ket{0}}	& \qw	& \qw 		& \qw 		& \qw  		& \qw				& \qw 			& \gate{\ket{0}}& \targ{}		& \ctrl{1}		& \targ{  }	& \qw 		& \qw & \rstick{$m_3$} \\
	\lstick{$a_3$} 			& \targ{}   & \qw	   	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw  		& \qw  		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw	& \qw				& \qw	& \qw 		& \qw 		& \qw  		& \qw				& \qw 			& \qw 			& \qw 			& \ctrl{1}		& \ctrl{-1}	& \qw 		& \qw & \rstick{$s_3$} \\
	\lstick{$b_3$} 			& \ctrl{-1} & \qw	   	& \ctrl{2}  & \targ{}	& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{2}	& \qw  		& \qw  		& \ctrl{2}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{2} & \ctrl{-1}	& \qw	& \gate{\ket{0}}	& \qw	& \qw 		& \qw 		& \qw  		& \qw				& \qw 			& \qw 			& \gate{\ket{0}}& \targ{}		& \targ{}	& \qw 		& \qw & \rstick{$m_4$} \\
	\lstick{$a_4$} 			& \targ{}   & \qw	   	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}  & \targ{}  	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw      & \targ{}	& \qw	& \qw				& \qw	& \targ{}	& \ctrl{-9} & \targ{}	& \qw				& \qw			& \qw 			& \qw 			& \qw 			& \qw		& \qw 		& \qw & \rstick{$s_4$} \\		
	\lstick{$b_4$} 			& \ctrl{-1} & \ctrl{1}  & \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \ctrl{1}  & \ctrl{-1}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}  & \ctrl{-1}	& \qw	& \gate{\ket{0}}	& \qw	& \qw	 	& \qw		& \qw  		& \qw				& \qw			& \qw 			& \qw 			& \gate{\ket{0}}& \qw 		& \qw 		& \qw & \rstick{$\ket{0}$} \\		
	\lstick{$\ket{0}$}   	& \qw       & \targ{}   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw 		& \targ{}  	& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \qw 		& \qw	& \qw				& \qw	& \targ{}	& \ctrl{-2}	& \targ{}	& \qw				& \qw			& \qw 			& \qw 			& \qw 			& \ctrl{-3}	& \qw 		& \qw & \rstick{$s_5$}
\end{quantikz}
}

\newcommand{\QMAfourNEW}{
\begin{quantikz} [row sep= {0.5cm, between origins}, column sep= {0.05cm}, transparent]
	\lstick{$\ket{0}$}   	& \qw	    & \qw	   	& \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw	& \qw\gategroup[12,steps=5,style={blue!75!black, ultra thick, dashed, rounded corners, inner xsep=-3pt}, background]{{\sc QMA4 Zero Resets}}	& \qw	& \qw				& \qw	& \qw	& \qw	& \qw 		& \targ{}	& \qw  		& \qw				& \ctrl{1}		& \targ{}		& \qw 			& \qw 			& \qw 		& \qw 		& \qw & \rstick{$m_0$} \\
	\lstick{$a_0$} 			& \qw	    & \qw	   	& \qw		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw		& \qw 		& \qw      & \targ{}	& \qw	& \qw	& \qw	& \qw				& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw  		& \qw				& \ctrl{1}		& \ctrl{-1}		& \qw 			& \qw 			& \qw 		& \qw 		& \qw & \rstick{$s_0$} \\
	\lstick{$b_0$} 			& \qw	    & \qw 	   	& \qw 		& \qw 		& \qw 		& \ctrl{2}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{2}	& \qw		& \qw 		& \qw      & \ctrl{-1}	& \qw	& \qw	& \qw	& \gate{\ket{0}}	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw  		& \gate{\ket{0}}	& \targ{}		& \ctrl{1}		& \targ{  }		& \qw 			& \qw 		& \qw 		& \qw & \rstick{$m_1$} \\
	\lstick{$a_1$} 			& \targ{}   & \qw	   	& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw	& \qw	& \qw	& \qw				& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw  		& \qw				& \qw 			& \ctrl{1}		& \ctrl{-1}		& \qw 			& \qw 		& \qw 		& \qw & \rstick{$s_1$} \\
	\lstick{$b_1$} 			& \ctrl{-1} & \qw	   	& \qw 		& \qw 		& \ctrl{2}	& \targ{}	& \ctrl{2}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \targ{}	& \ctrl{2}	& \qw 		& \qw      & \ctrl{-1}	& \qw	& \qw	& \qw	& \gate{\ket{0}}	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw  		& \qw				& \gate{\ket{0}}& \targ{}		& \ctrl{1}		& \targ{  }		& \qw 		& \qw 		& \qw & \rstick{$m_2$} \\
	\lstick{$a_2$} 			& \targ{}   & \qw	   	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw	& \qw	& \qw	& \qw				& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw  		& \qw				& \qw 			& \qw 			& \ctrl{1}		& \ctrl{-1}		& \qw 		& \qw 		& \qw & \rstick{$s_2$} \\
	\lstick{$b_2$} 			& \ctrl{-1} & \qw	   	& \qw 		& \ctrl{2}	& \targ{}	& \qw 		& \targ{}	& \ctrl{2}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \targ{}	& \ctrl{2}	& \qw      & \ctrl{-1}	& \qw	& \qw	& \qw	& \gate{\ket{0}}	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw  		& \qw				& \qw 			& \gate{\ket{0}}& \targ{}		& \ctrl{1}		& \targ{  }	& \qw 		& \qw & \rstick{$m_3$} \\
	\lstick{$a_3$} 			& \targ{}   & \qw	   	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw  		& \qw  		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw	& \qw	& \qw	& \qw				& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw  		& \qw				& \qw 			& \qw 			& \qw 			& \ctrl{1}		& \ctrl{-1}	& \qw 		& \qw & \rstick{$s_3$} \\
	\lstick{$b_3$} 			& \ctrl{-1} & \qw	   	& \ctrl{2}  & \targ{}	& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{2}	& \qw  		& \qw  		& \ctrl{2}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{2} & \ctrl{-1}	& \qw	& \qw	& \qw	& \gate{\ket{0}}	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw  		& \qw				& \qw 			& \qw 			& \gate{\ket{0}}& \targ{}		& \targ{}	& \qw 		& \qw & \rstick{$m_4$} \\
	\lstick{$a_4$} 			& \targ{}   & \qw	   	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}  & \targ{}  	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw      & \targ{}	& \qw	& \qw	& \qw	& \qw				& \qw	& \qw	& \qw	& \targ{}	& \ctrl{-9} & \targ{}	& \qw				& \qw			& \qw 			& \qw 			& \qw 			& \qw		& \qw 		& \qw & \rstick{$s_4$} \\		
	\lstick{$b_4$} 			& \ctrl{-1} & \ctrl{1}  & \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \ctrl{1}  & \ctrl{-1}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}  & \ctrl{-1}	& \qw	& \qw	& \qw	& \gate{\ket{0}}	& \qw	& \qw	& \qw	& \qw	 	& \qw		& \qw  		& \qw				& \qw			& \qw 			& \qw 			& \gate{\ket{0}}& \qw 		& \qw 		& \qw & \rstick{$\ket{0}$} \\		
	\lstick{$\ket{0}$}   	& \qw       & \targ{}   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw 		& \targ{}  	& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \qw 		& \qw	& \qw	& \qw	& \qw				& \qw	& \qw	& \qw	& \targ{}	& \ctrl{-2}	& \targ{}	& \qw				& \qw			& \qw 			& \qw 			& \qw 			& \ctrl{-3}	& \qw 		& \qw & \rstick{$s_5$}
\end{quantikz}
}

\newcommand{\QMAfourCombined}{
\begin{quantikz} [row sep= {0.5cm, between origins}, column sep= {0.05cm}, transparent]
	\lstick{$\ket{0}$}   	& \qw	    & \qw	   	& \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw	& \qw\gategroup[12,steps=5,style={blue!75!black, ultra thick, dashed, rounded corners, inner xsep=-3pt}, background]{{\sc QMA4 Zero Resets}}	& \qw	& \qw				& \qw	& \qw	& \qw	& \qw 		& \targ{}	& \qw  		& \qw				& \ctrl{1}		& \targ{}		& \qw 			& \qw 			& \qw 		& \qw 		& \qw & \rstick{$m_0$} \\
	\lstick{$a_0$} 			& \qw	    & \qw	   	& \qw		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw		& \qw 		& \qw      & \targ{}	& \qw	& \qw	& \qw	& \qw				& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw  		& \qw				& \ctrl{1}		& \ctrl{-1}		& \qw 			& \qw 			& \qw 		& \qw 		& \qw & \rstick{$s_0$} \\
	\lstick{$b_0$} 			& \qw	    & \qw 	   	& \qw 		& \qw 		& \qw 		& \ctrl{2}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{2}	& \qw		& \qw 		& \qw      & \ctrl{-1}	& \qw	& \qw	& \qw	& \gate{\ket{0}}	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw  		& \gate{\ket{0}}	& \targ{}		& \ctrl{1}		& \targ{  }		& \qw 			& \qw 		& \qw 		& \qw & \rstick{$m_1$} \\
	\lstick{$a_1$} 			& \targ{}   & \qw	   	& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw	& \qw	& \qw	& \qw				& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw  		& \qw				& \qw 			& \ctrl{1}		& \ctrl{-1}		& \qw 			& \qw 		& \qw 		& \qw & \rstick{$s_1$} \\
	\lstick{$b_1$} 			& \ctrl{-1} & \qw	   	& \qw 		& \qw 		& \ctrl{2}	& \targ{}	& \ctrl{2}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \targ{}	& \ctrl{2}	& \qw 		& \qw      & \ctrl{-1}	& \qw	& \qw	& \qw	& \gate{\ket{0}}	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw  		& \qw				& \gate{\ket{0}}& \targ{}		& \ctrl{1}		& \targ{  }		& \qw 		& \qw 		& \qw & \rstick{$m_2$} \\
	\lstick{$a_2$} 			& \targ{}   & \qw	   	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw	& \qw	& \qw	& \qw				& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw  		& \qw				& \qw 			& \qw 			& \ctrl{1}		& \ctrl{-1}		& \qw 		& \qw 		& \qw & \rstick{$s_2$} \\
	\lstick{$b_2$} 			& \ctrl{-1} & \qw	   	& \qw 		& \ctrl{2}	& \targ{}	& \qw 		& \targ{}	& \ctrl{2}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \targ{}	& \ctrl{2}	& \qw      & \ctrl{-1}	& \qw	& \qw	& \qw	& \gate{\ket{0}}	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw  		& \qw				& \qw 			& \gate{\ket{0}}& \targ{}		& \ctrl{1}		& \targ{  }	& \qw 		& \qw & \rstick{$m_3$} \\
	\lstick{$a_3$} 			& \targ{}   & \qw	   	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw  		& \qw  		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw	& \qw	& \qw	& \qw				& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw  		& \qw				& \qw 			& \qw 			& \qw 			& \ctrl{1}		& \ctrl{-1}	& \qw 		& \qw & \rstick{$s_3$} \\
	\lstick{$b_3$} 			& \ctrl{-1} & \qw	   	& \ctrl{2}  & \targ{}	& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{2}	& \qw  		& \qw  		& \ctrl{2}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{2} & \ctrl{-1}	& \qw	& \qw	& \qw	& \gate{\ket{0}}	& \qw	& \qw	& \qw	& \qw 		& \qw 		& \qw  		& \qw				& \qw 			& \qw 			& \gate{\ket{0}}& \targ{}		& \targ{}	& \qw 		& \qw & \rstick{$m_4$} \\
	\lstick{$a_4$} 			& \targ{}   & \qw	   	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}  & \targ{}  	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw      & \targ{}	& \qw	& \qw	& \qw	& \qw				& \qw	& \qw	& \qw	& \targ{}	& \ctrl{-9} & \targ{}	& \qw				& \qw			& \qw 			& \qw 			& \qw 			& \qw		& \qw 		& \qw & \rstick{$s_4$} \\		
	\lstick{$b_4$} 			& \ctrl{-1} & \ctrl{1}  & \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \ctrl{1}  & \ctrl{-1}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}  & \ctrl{-1}	& \qw	& \qw	& \qw	& \gate{\ket{0}}	& \qw	& \qw	& \qw	& \qw	 	& \qw		& \qw  		& \qw				& \qw			& \qw 			& \qw 			& \gate{\ket{0}}& \qw 		& \qw 		& \qw & \rstick{$\ket{0}$} \\		
	\lstick{$\ket{0}$}   	& \qw       & \targ{}   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw 		& \targ{}  	& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \qw 		& \qw	& \qw	& \qw	& \qw				& \qw	& \qw	& \qw	& \targ{}	& \ctrl{-2}	& \targ{}	& \qw				& \qw			& \qw 			& \qw 			& \qw 			& \ctrl{-3}	& \qw 		& \qw & \rstick{$s_5$}
\end{quantikz}
}

==> latex_images/quantikz_figures2.tex <==
\usepackage{tikz}
\usepackage{quantikz}
\usepackage{amsmath}

\newcommand{\rowSep}{0.25cm}
\newcommand{\colSep}{0.2cm}


\newcommand{\myCnot}{
\begin{quantikz} [row sep= \rowSep, column sep= \colSep]
	\lstick{$a$} & \ctrl{1} & \qw & \rstick{$a$}\\
	\lstick{$b$} & \targ{}  & \qw & \rstick{$a \oplus b$}
\end{quantikz}
}

\newcommand{\mySwap}{
\begin{quantikz}
	\qw & \swap{1} & \qw \\
	\qw & \targX{} & \qw
\end{quantikz} = \begin{quantikz}
	\qw & \ctrl{1} & \targ{} 	& \ctrl{1} & \qw \\
	\qw & \targ{}  & \ctrl{-1} 	& \targ{}  & \qw
\end{quantikz}
}

\newcommand{\myToffoli}{
\begin{quantikz} [row sep= \rowSep, column sep= \colSep]
	\lstick{$a$} & \ctrl{1} & \qw & \rstick{$a$} \\
	\lstick{$b$} & \ctrl{1} & \qw & \rstick{$b$} \\
	\lstick{$c$} & \targ{}  & \qw & \rstick{$a \cdot b \oplus c$}
\end{quantikz}
}

\newcommand{\ModFour}{
	\begin{quantikz} [row sep= \rowSep, column sep= \colSep, transparent]
		\lstick{$A_0$} & \ctrl{1} 	& \targ{}	&	\rstick{$M_0$} \\
		\lstick{$B_0$} & \ctrl{1} 	& \ctrl{-1}	&	\rstick{$B_0$} \\
		\lstick{$A_1$} & \targ{}  	& \targ{}	&	\rstick{$M_1$} \\
		\lstick{$B_1$} & \qw		& \ctrl{-1}	&	\rstick{$B_1$} 
	\end{quantikz}
}

\newcommand{\ModEight}{
\begin{quantikz} [row sep= \rowSep, column sep= \colSep, transparent]
	\lstick{$A_0$} & \qw	    & \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw		& \targ{}	& \rstick{$M_0$} \\
	\lstick{$B_0$} & \qw 	   	& \qw 		& \ctrl{2}	& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{2}	& \qw		& \ctrl{-1}	& \rstick{$B_0$} \\
	\lstick{$A_1$} & \targ{}   	& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \targ{}	& \rstick{$M_1$} \\
	\lstick{$B_1$} & \ctrl{-1} 	& \ctrl{2}	& \targ{}	& \ctrl{2}	& \qw 		& \ctrl{2}	& \ctrl{-1}	& \targ{}	& \ctrl{2}	& \ctrl{-1}	& \rstick{$B_1$} \\
	\lstick{$A_2$} & \targ{}   	& \qw 		& \qw 		& \qw 		& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \rstick{$M_2$} \\
	\lstick{$B_2$} & \ctrl{-1} 	& \targ{}	& \qw 		& \targ{}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \targ{}	& \ctrl{-1}	& \rstick{$B_2$} 
\end{quantikz}
}

\newcommand{\KimModuloAdder}{
	\begin{quantikz} [row sep= \rowSep, column sep= \colSep, transparent]
		\lstick{$0$}   & \targ{}	& \qw		& \ctrl{2}	& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{2}	& \targ{}	& \targ{}	& \ctrl{2}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{2}	& \qw		& \qw		& \qw		& \ctrl{2}		& \targ{}	& \qw  & \rstick{$0$} \\
		\lstick{$a_0$} & \ctrl{1} 	& \ctrl{1} 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		&  \qw 	 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 	 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		&  \qw 	  	& \ctrl{1} 	& \ctrl{2} 	& \ctrl{1} 	& \qw 		 	& \qw 		& \qw  & \rstick{$a_0$} \\
		\lstick{$b_0$} & \ctrl{1}	& \targ{}	& \ctrl{1}	& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}	& \qw		& \qw		& \ctrl{1}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1} 	& \targ{} 	& \ctrl{1} 	& \targ{} 	& \targ{} 		& \qw		& \qw  & \rstick{$s_0$} \\
		\lstick{$0$}   & \targ{}	& \qw		& \targ{}	& \ctrl{2}	& \qw		& \qw		& \qw		& \ctrl{2}	& \targ{}	& \qw		& \qw		& \targ{}	& \ctrl{2}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{2}	& \qw		& \qw		& \qw		& \ctrl{2}	& \targ{}	& \qw		& \targ{}	& \qw		& \qw			& \qw		& \qw  & \rstick{$c_1$} \\
		\lstick{$a_1$} & \ctrl{1} 	& \ctrl{1} 	& \qw 		&  \qw 	 	& \qw 		& \qw 		& \qw 		&  \qw 	 	& \qw 		& \qw 		& \qw 		& \qw 		&  \qw 	 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 	 	& \qw 		& \qw 		&  \qw 	  	& \ctrl{1} 	& \ctrl{2} 	& \ctrl{1} 	& \qw 		& \qw 		& \qw	 	& \qw		& \qw		& \qw 			& \qw 		& \qw  & \rstick{$a_1$} \\
		\lstick{$b_1$} & \ctrl{1} 	& \targ{} 	& \qw 		& \ctrl{1} 	& \qw 		& \qw 		& \qw 		& \ctrl{1} 	& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1} 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 	 	& \qw 		& \qw 		& \ctrl{1} 	& \targ{} 	& \ctrl{1} 	& \targ{} 	& \targ{} 	& \qw 		& \qw	 	& \qw		& \qw		& \qw 			& \qw 		& \qw  & \rstick{$s_1$} \\
		\lstick{$0$}   & \targ{}	& \qw		& \qw		& \targ{}	& \ctrl{2}	& \qw		& \ctrl{2}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \targ{}	& \ctrl{2}	& \qw		& \ctrl{2}	& \qw		& \qw		& \qw		& \ctrl{2}	& \targ{}	& \qw		& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw			& \qw		& \qw  & \rstick{$c_2$} \\
		\lstick{$a_2$} & \ctrl{1} 	& \ctrl{1} 	& \qw 		& \qw 		&  \qw 	 	& \qw 		&  \qw 	 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		&  \qw 	 	& \qw 		&  \qw 	  	& \ctrl{1} 	& \ctrl{2} 	& \ctrl{1} 	& \qw 		& \qw 		& \qw	 	& \qw 		& \qw	 	& \qw 		& \qw 		& \qw	 	& \qw 		& \qw	 	& \qw 			& \qw 		& \qw  & \rstick{$a_2$} \\
		\lstick{$b_2$} & \ctrl{1} 	& \targ{} 	& \qw 		& \qw 		& \ctrl{1} 	& \qw 		& \ctrl{1} 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1} 	& \qw 		& \ctrl{1} 	& \targ{} 	& \ctrl{1} 	& \targ{} 	& \targ{} 	& \qw 		& \qw	 	& \qw 		& \qw	 	& \qw 		& \qw 		& \qw	 	& \qw 		& \qw	 	& \qw 			& \qw 		& \qw  & \rstick{$s_2$} \\
		\lstick{$0$}   & \targ{}	& \qw		& \qw		& \qw		& \targ{}	& \ctrl{2}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \ctrl{2}	& \targ{}	& \qw		& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw			& \qw		& \qw  & \rstick{$c_3$} \\
		\lstick{$a_3$} & \ctrl{1} 	& \ctrl{1} 	& \qw 		& \qw 		& \qw 		&  \qw 	 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 	 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw	 	& \qw 		& \qw	 	& \qw 		& \qw 		& \qw	 	& \qw 		& \qw	 	& \qw 			& \qw 		& \qw  & \rstick{$a_3$} \\
		\lstick{$b_3$} & \ctrl{1} 	& \targ{} 	& \qw 		& \qw 		& \qw 		& \ctrl{1} 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{} 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw	 	& \qw 		& \qw	 	& \qw 		& \qw 		& \qw	 	& \qw 		& \qw	 	& \qw 			& \qw 		& \qw  & \rstick{$s_3$} \\
		\lstick{$0$}   & \targ{} 	& \qw 		& \qw 		& \qw 		& \qw 		& \targ{} 	& \qw 		& \qw 		& \qw 		& \ctrl{-12}& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw	 	& \qw 		& \qw	 	& \qw 		& \qw 		& \qw	 	& \qw 		& \qw	 	& \qw 			& \ctrl{-12}& \qw  & \rstick{$c_4$}
	\end{quantikz}
}

\newcommand{\KimModuloAdderThree}{
	\begin{quantikz} [row sep= \rowSep, column sep= \colSep, transparent]
		\lstick{$0$}   & \targ{}	& \qw		& \ctrl{2}	& \qw		& \ctrl{2}	& \targ{}	& \targ{}	& \ctrl{2}	& \qw		& \ctrl{2}	& \qw		& \qw		& \qw		& \ctrl{2}	& \targ{}	& \qw		& \rstick{$0$} \\
		\lstick{$A_0$} & \ctrl{1} 	& \ctrl{1} 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		&  \qw 	 	& \ctrl{1}	& \ctrl{1}	& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \rstick{$A_0$} \\
		\lstick{$B_0$} & \ctrl{1}	& \targ{}	& \ctrl{1}	& \qw		& \ctrl{1}	& \qw		& \qw		& \ctrl{1}	& \qw		& \ctrl{1}	& \targ{}	& \ctrl{1}	& \targ{}	& \targ{}	& \qw		& \qw		& \rstick{$M_0$} \\
		\lstick{$0$}   & \targ{}	& \qw		& \targ{}	& \ctrl{2}	& \targ{}	& \qw		& \qw		& \targ{}	& \ctrl{2}	& \targ{}	& \qw		& \targ{}	& \qw		& \qw		& \qw		& \qw		& \rstick{$Carry_0$} \\
		\lstick{$A_1$} & \ctrl{1} 	& \ctrl{1} 	& \qw 		&  \qw 	 	& \qw 		& \qw 		& \qw		& \qw 		& \qw 	 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 	 	& \qw 		& \qw 		& \rstick{$A_1$} \\
		\lstick{$B_1$} & \ctrl{1} 	& \targ{} 	& \qw 		& \ctrl{1} 	& \qw 		& \qw 		& \qw		& \qw 		& \targ{} 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw	 	& \qw 		& \qw 		& \rstick{$M_1$} \\
		\lstick{$0$}   & \targ{}	& \qw		& \qw		& \targ{}	& \qw		& \ctrl{-6}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{-6}	& \qw		& \rstick{$Carry_1$}
	\end{quantikz}
}

\newcommand{\ProposedModuloAdderThree}{
	\begin{quantikz} [row sep= \rowSep, column sep= \colSep, transparent]
		\lstick{$0$}   & \qw		& \qw		& \targ{}	& \qw		& \ctrl{2}	& \targ{}	&\rstick{$M_0$}   \\
		\lstick{$A_0$} & \ctrl{1}	& \ctrl{1}	& \qw		& \qw		& \qw		& \qw		&\rstick{$A_0$} \\
		\lstick{$B_0$} & \ctrl{2}	& \targ{}	& \qw		& \qw		& \ctrl{1}	& \ctrl{-2}	&\rstick{$S_0$} \\
		\lstick{$0$}   & \qw		& \qw		& \qw		& \targ{}	& \targ{}	& \qw		&\rstick{$M_1$} \\
		\lstick{$0$}   & \targ{}	& \targ{}	& \ctrl{-4}	& \qw		& \targ{}	& \qw		&\rstick{$Carry_1$} \\
		\lstick{$0$}   & \qw		& \targ{}	& \ctrl{-1}	& \qw		& \qw		& \qw		&\rstick{$\overline{A_1}.\overline{B_1}$} \\
		\lstick{$A_1$} & \targ{}	& \ctrl{-1}	& \targ{}	& \ctrl{-3}	& \qw		& \qw		&\rstick{$A_1$} \\
		\lstick{$B_1$} & \targ{}	& \ctrl{-1}	& \targ{}	& \ctrl{-1}	& \qw		& \qw		&\rstick{$B_1$}
	\end{quantikz}
}

\newcommand{\ProposedModuloAdderNine}{
	\begin{quantikz} [row sep= \rowSep, column sep= \colSep, transparent]
		\lstick{$0$}   & \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \qw		& \ctrl{1}	& \qw		& \qw		& \targ{}	& \rstick{$M_0$} \\
		\lstick{$A_0$} & \qw		& \qw		& \qw		& \ctrl{1}	& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}	& \qw		& \targ{}	& \qw		& \qw		& \ctrl{2}	& \qw		& \qw		& \ctrl{-1}	& \rstick{$S_0$} \\
		\lstick{$B_0$} & \qw		& \qw		& \qw		& \ctrl{3}	& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{3}	& \qw		& \ctrl{-1}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \rstick{$B_0$} \\
		\lstick{$0$}   & \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \ctrl{1}	& \qw		& \targ{}	& \rstick{$M_1$} \\
		\lstick{$A_1$} & \targ{}	& \qw		& \qw		& \qw		& \ctrl{1}	& \qw		& \qw		& \ctrl{1}	& \targ{}	& \qw		& \qw		& \targ{}	& \qw		& \qw		& \qw		& \ctrl{2}	& \qw		& \ctrl{-1}	& \rstick{$S_1$} \\
		\lstick{$B_1$} & \ctrl{-1}	& \qw		& \ctrl{3}	& \targ{}	& \ctrl{3}	& \qw		& \qw		& \ctrl{3}	& \ctrl{-1} & \targ{}	& \ctrl{3}	& \ctrl{-1}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \rstick{$B_1$} \\
		\lstick{$0$}   & \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \ctrl{1}	& \targ{}	& \rstick{$M_2$} \\
		\lstick{$A_2$} & \targ{}	& \qw		& \qw		& \qw		& \qw		& \ctrl{1}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \targ{}	& \qw		& \qw		& \qw		& \qw		& \ctrl{2}	& \ctrl{-1}	& \rstick{$S_2$} \\
		\lstick{$B_2$} & \ctrl{-1}	& \ctrl{2}	& \targ{}	& \qw		& \targ{}	& \ctrl{2}	& \ctrl{-1}	& \targ{}	& \qw		& \qw		& \targ{}	& \ctrl{-1}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \rstick{$B_2$} \\
		\lstick{$0$}   & \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \qw		& \targ{}	& \qw		& \rstick{$M_3$} \\
		\lstick{$0$}   & \qw		& \targ{}	& \qw		& \qw		& \qw		& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \ctrl{-10}& \targ{}	& \qw		& \qw		& \qw		& \qw		& \rstick{$Carry_3$} \\
		\lstick{$0$}   & \qw		& \qw		& \qw		& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \ctrl{-1}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \rstick{$\overline{A_3}.\overline{B_3}$} \\
		\lstick{$A_3$} & \qw		& \qw		& \targ{}	& \ctrl{-1}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{-3}	& \qw		& \qw		& \qw		& \rstick{$A_3$} \\
		\lstick{$B_3$} & \qw		& \qw		& \targ{}	& \ctrl{-1}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{-1}	& \qw		& \qw		& \qw		& \rstick{$B_3$} \\
	\end{quantikz}
}


==> latex_images/quantikz_figures_bk.tex <==
\usepackage{tikz}
\usepackage{quantikz}
\usepackage{amsmath}

\newcommand{\rowSep}{0.25cm}
\newcommand{\colSep}{0.2cm}


\newcommand{\myCnot}{
\begin{quantikz} [row sep= \rowSep, column sep= \colSep]
	\lstick{$a$} & \ctrl{1} & \qw & \rstick{$a$}\\
	\lstick{$b$} & \targ{}  & \qw & \rstick{$a \oplus b$}
\end{quantikz}
}

\newcommand{\mySwap}{
\begin{quantikz}
	\qw & \swap{1} & \qw \\
	\qw & \targX{} & \qw
\end{quantikz} = \begin{quantikz}
	\qw & \ctrl{1} & \targ{} 	& \ctrl{1} & \qw \\
	\qw & \targ{}  & \ctrl{-1} 	& \targ{}  & \qw
\end{quantikz}
}

\newcommand{\myToffoli}{
\begin{quantikz} [row sep= \rowSep, column sep= \colSep]
	\lstick{$a$} & \ctrl{1} & \qw & \rstick{$a$} \\
	\lstick{$b$} & \ctrl{1} & \qw & \rstick{$b$} \\
	\lstick{$c$} & \targ{}  & \qw & \rstick{$a \cdot b \oplus c$}
\end{quantikz}
}

\newcommand{\KimModuloAdderBoxed}{
\begin{quantikz} [row sep= 0.2cm, column sep= 0.17cm, transparent]
	\lstick{$0$}   & \targ{} &\qw	& \qw\gategroup[13,steps=9,style={blue!75!black, ultra thick, dashed, rounded corners, inner xsep=2pt}, background]{{\sc QRCA based Carry Generation Logic}}
												& \qw		& \ctrl{2}	& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{2}	& \qw  & \targ{}	& \targ{}	& \qw	& \ctrl{2}\gategroup[13,steps=19,style={green!50!black, ultra thick, dashed, rounded corners, inner xsep=2pt}, background]{{\sc QRCA based Carryout Truncated Full Adder}}		
																																																	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{2}	& \qw		& \qw		& \qw		& \ctrl{2}		& \qw  & \targ{}	& \qw  & \rstick{$0$} \\
	\lstick{$a_0$} & \qw  	 &\qw	& \ctrl{1} 	& \ctrl{1} 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		&  \qw 	 	& \qw  & \qw 		& \qw 		& \qw	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 	 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		&  \qw 	  	& \ctrl{1} 	& \ctrl{2} 	& \ctrl{1} 	& \qw 		 	& \qw  & \qw 		& \qw  & \rstick{$a_0$} \\
	\lstick{$b_0$} & \qw  	 &\qw	& \ctrl{1}	& \targ{}	& \ctrl{1}	& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}	& \qw  & \qw		& \qw		& \qw	& \ctrl{1}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1} 	& \targ{} 	& \ctrl{1} 	& \targ{} 	& \targ{} 		& \qw  & \qw		& \qw  & \rstick{$s_0$} \\
	\lstick{$0$}   & \qw  	 &\qw	& \targ{}	& \qw		& \targ{}	& \ctrl{2}	& \qw		& \qw		& \qw		& \ctrl{2}	& \targ{}	& \qw  & \qw		& \qw		& \qw	& \targ{}	& \ctrl{2}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{2}	& \qw		& \qw		& \qw		& \ctrl{2}	& \targ{}	& \qw		& \targ{}	& \qw		& \qw			& \qw  & \qw		& \qw  & \rstick{$c_1$} \\
	\lstick{$a_1$} & \qw  	 &\qw	& \ctrl{1} 	& \ctrl{1} 	& \qw 		&  \qw 	 	& \qw 		& \qw 		& \qw 		&  \qw 	 	& \qw 		& \qw  & \qw 		& \qw 		& \qw	& \qw 		&  \qw 	 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 	 	& \qw 		& \qw 		&  \qw 	  	& \ctrl{1} 	& \ctrl{2} 	& \ctrl{1} 	& \qw 		& \qw 		& \qw	 	& \qw		& \qw		& \qw 			& \qw  & \qw 		& \qw  & \rstick{$a_1$} \\
	\lstick{$b_1$} & \qw  	 &\qw	& \ctrl{1} 	& \targ{} 	& \qw 		& \ctrl{1} 	& \qw 		& \qw 		& \qw 		& \ctrl{1} 	& \qw 		& \qw  & \qw 		& \qw 		& \qw	& \qw 		& \ctrl{1} 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 	 	& \qw 		& \qw 		& \ctrl{1} 	& \targ{} 	& \ctrl{1} 	& \targ{} 	& \targ{} 	& \qw 		& \qw	 	& \qw		& \qw		& \qw 			& \qw  & \qw 		& \qw  & \rstick{$s_1$} \\
	\lstick{$0$}   & \qw  	 &\qw	& \targ{}	& \qw		& \qw		& \targ{}	& \ctrl{2}	& \qw		& \ctrl{2}	& \targ{}	& \qw		& \qw  & \qw		& \qw		& \qw	& \qw		& \targ{}	& \ctrl{2}	& \qw		& \ctrl{2}	& \qw		& \qw		& \qw		& \ctrl{2}	& \targ{}	& \qw		& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw			& \qw  & \qw		& \qw  & \rstick{$c_2$} \\
	\lstick{$a_2$} & \qw  	 &\qw	& \ctrl{1} 	& \ctrl{1} 	& \qw 		& \qw 		&  \qw 	 	& \qw 		&  \qw 	 	& \qw 		& \qw 		& \qw  & \qw 		& \qw 		& \qw	& \qw 		& \qw 		&  \qw 	 	& \qw 		&  \qw 	  	& \ctrl{1} 	& \ctrl{2} 	& \ctrl{1} 	& \qw 		& \qw 		& \qw	 	& \qw 		& \qw	 	& \qw 		& \qw 		& \qw	 	& \qw 		& \qw	 	& \qw 			& \qw  & \qw 		& \qw  & \rstick{$a_2$} \\
	\lstick{$b_2$} & \qw  	 &\qw	& \ctrl{1} 	& \targ{} 	& \qw 		& \qw 		& \ctrl{1} 	& \qw 		& \ctrl{1} 	& \qw 		& \qw 		& \qw  & \qw 		& \qw 		& \qw	& \qw 		& \qw 		& \ctrl{1} 	& \qw 		& \ctrl{1} 	& \targ{} 	& \ctrl{1} 	& \targ{} 	& \targ{} 	& \qw 		& \qw	 	& \qw 		& \qw	 	& \qw 		& \qw 		& \qw	 	& \qw 		& \qw	 	& \qw 			& \qw  & \qw 		& \qw  & \rstick{$s_2$} \\
	\lstick{$0$}   & \qw  	 &\qw	& \targ{}	& \qw		& \qw		& \qw		& \targ{}	& \ctrl{2}	& \targ{}	& \qw		& \qw		& \qw  & \qw		& \qw		& \qw	& \qw		& \qw		& \targ{}	& \ctrl{2}	& \targ{}	& \qw		& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw			& \qw  & \qw		& \qw  & \rstick{$c_3$} \\
	\lstick{$a_3$} & \qw  	 &\qw	& \ctrl{1} 	& \ctrl{1} 	& \qw 		& \qw 		& \qw 		&  \qw 	 	& \qw 		& \qw 		& \qw 		& \qw  & \qw 		& \qw 		& \qw	& \qw 		& \qw 		& \qw 		& \qw 	 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw	 	& \qw 		& \qw	 	& \qw 		& \qw 		& \qw	 	& \qw 		& \qw	 	& \qw 			& \qw  & \qw 		& \qw  & \rstick{$a_3$} \\
	\lstick{$b_3$} & \qw  	 &\qw	& \ctrl{1} 	& \targ{} 	& \qw 		& \qw 		& \qw 		& \ctrl{1} 	& \qw 		& \qw 		& \qw 		& \qw  & \qw 		& \qw 		& \qw	& \qw 		& \qw 		& \qw 		& \targ{} 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw	 	& \qw 		& \qw	 	& \qw 		& \qw 		& \qw	 	& \qw 		& \qw	 	& \qw 			& \qw  & \qw 		& \qw  & \rstick{$s_3$} \\
	\lstick{$0$}   & \qw  	 &\qw	& \targ{} 	& \qw 		& \qw 		& \qw 		& \qw 		& \targ{} 	& \qw 		& \qw 		& \qw 		& \qw  & \ctrl{-12}& \qw 		& \qw	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw	 	& \qw 		& \qw	 	& \qw 		& \qw 		& \qw	 	& \qw 		& \qw	 	& \qw 			& \qw  & \ctrl{-12}& \qw  & \rstick{$c_4$}
\end{quantikz}
}

\newcommand{\KimModuloAdder}{
\begin{quantikz} [row sep= \rowSep, column sep= \colSep, transparent]
	\lstick{$0$}   & \targ{}	& \qw		& \ctrl{2}	& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{2}	& \targ{}	& \targ{}	& \ctrl{2}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{2}	& \qw		& \qw		& \qw		& \ctrl{2}		& \targ{}	& \qw  & \rstick{$0$} \\
	\lstick{$a_0$} & \ctrl{1} 	& \ctrl{1} 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		&  \qw 	 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 	 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		&  \qw 	  	& \ctrl{1} 	& \ctrl{2} 	& \ctrl{1} 	& \qw 		 	& \qw 		& \qw  & \rstick{$a_0$} \\
	\lstick{$b_0$} & \ctrl{1}	& \targ{}	& \ctrl{1}	& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}	& \qw		& \qw		& \ctrl{1}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1} 	& \targ{} 	& \ctrl{1} 	& \targ{} 	& \targ{} 		& \qw		& \qw  & \rstick{$s_0$} \\
	\lstick{$0$}   & \targ{}	& \qw		& \targ{}	& \ctrl{2}	& \qw		& \qw		& \qw		& \ctrl{2}	& \targ{}	& \qw		& \qw		& \targ{}	& \ctrl{2}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{2}	& \qw		& \qw		& \qw		& \ctrl{2}	& \targ{}	& \qw		& \targ{}	& \qw		& \qw			& \qw		& \qw  & \rstick{$c_1$} \\
	\lstick{$a_1$} & \ctrl{1} 	& \ctrl{1} 	& \qw 		&  \qw 	 	& \qw 		& \qw 		& \qw 		&  \qw 	 	& \qw 		& \qw 		& \qw 		& \qw 		&  \qw 	 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 	 	& \qw 		& \qw 		&  \qw 	  	& \ctrl{1} 	& \ctrl{2} 	& \ctrl{1} 	& \qw 		& \qw 		& \qw	 	& \qw		& \qw		& \qw 			& \qw 		& \qw  & \rstick{$a_1$} \\
	\lstick{$b_1$} & \ctrl{1} 	& \targ{} 	& \qw 		& \ctrl{1} 	& \qw 		& \qw 		& \qw 		& \ctrl{1} 	& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1} 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 	 	& \qw 		& \qw 		& \ctrl{1} 	& \targ{} 	& \ctrl{1} 	& \targ{} 	& \targ{} 	& \qw 		& \qw	 	& \qw		& \qw		& \qw 			& \qw 		& \qw  & \rstick{$s_1$} \\
	\lstick{$0$}   & \targ{}	& \qw		& \qw		& \targ{}	& \ctrl{2}	& \qw		& \ctrl{2}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \targ{}	& \ctrl{2}	& \qw		& \ctrl{2}	& \qw		& \qw		& \qw		& \ctrl{2}	& \targ{}	& \qw		& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw			& \qw		& \qw  & \rstick{$c_2$} \\
	\lstick{$a_2$} & \ctrl{1} 	& \ctrl{1} 	& \qw 		& \qw 		&  \qw 	 	& \qw 		&  \qw 	 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		&  \qw 	 	& \qw 		&  \qw 	  	& \ctrl{1} 	& \ctrl{2} 	& \ctrl{1} 	& \qw 		& \qw 		& \qw	 	& \qw 		& \qw	 	& \qw 		& \qw 		& \qw	 	& \qw 		& \qw	 	& \qw 			& \qw 		& \qw  & \rstick{$a_2$} \\
	\lstick{$b_2$} & \ctrl{1} 	& \targ{} 	& \qw 		& \qw 		& \ctrl{1} 	& \qw 		& \ctrl{1} 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1} 	& \qw 		& \ctrl{1} 	& \targ{} 	& \ctrl{1} 	& \targ{} 	& \targ{} 	& \qw 		& \qw	 	& \qw 		& \qw	 	& \qw 		& \qw 		& \qw	 	& \qw 		& \qw	 	& \qw 			& \qw 		& \qw  & \rstick{$s_2$} \\
	\lstick{$0$}   & \targ{}	& \qw		& \qw		& \qw		& \targ{}	& \ctrl{2}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \ctrl{2}	& \targ{}	& \qw		& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw			& \qw		& \qw  & \rstick{$c_3$} \\
	\lstick{$a_3$} & \ctrl{1} 	& \ctrl{1} 	& \qw 		& \qw 		& \qw 		&  \qw 	 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 	 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw	 	& \qw 		& \qw	 	& \qw 		& \qw 		& \qw	 	& \qw 		& \qw	 	& \qw 			& \qw 		& \qw  & \rstick{$a_3$} \\
	\lstick{$b_3$} & \ctrl{1} 	& \targ{} 	& \qw 		& \qw 		& \qw 		& \ctrl{1} 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{} 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw	 	& \qw 		& \qw	 	& \qw 		& \qw 		& \qw	 	& \qw 		& \qw	 	& \qw 			& \qw 		& \qw  & \rstick{$s_3$} \\
	\lstick{$0$}   & \targ{} 	& \qw 		& \qw 		& \qw 		& \qw 		& \targ{} 	& \qw 		& \qw 		& \qw 		& \ctrl{-12}& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw	 	& \qw 		& \qw	 	& \qw 		& \qw 		& \qw	 	& \qw 		& \qw	 	& \qw 			& \ctrl{-12}& \qw  & \rstick{$c_4$}
\end{quantikz}
}

\newcommand{\ProposedModuloAdderBoxed}{
\begin{quantikz} [row sep= \rowSep, column sep= \colSep, transparent]
	\lstick{$1$}   & \qw		& \qw\gategroup[16,steps=7,style={blue!75!black, ultra thick, dashed, rounded corners, inner xsep=2pt}, background]{{\sc Carry-lookahead Generation Logic}}		
											& \qw		& \ctrl{3}	& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \targ{}	& \qw		& \qw\gategroup[16,steps=14,style={green!50!black, ultra thick, dashed, rounded corners, inner xsep=2pt}, background]{{\sc Carry-lookahead Truncated Full Adder}}
																																												& \qw		& \ctrl{4}	& \qw		& \qw		& \ctrl{2}	& \qw		& \qw		& \qw		& \qw		& \ctrl{4}	& \qw		& \qw		& \qw		& \qw		& \targ{}	& \qw		& \rstick{$0$} \\
	%\lstick{$0$}   & \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \rstick{$0$} \\
	\lstick{$a_0$} & \qw		& \ctrl{2}	& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}	& \qw		& \qw		& \qw		& \qw		& \ctrl{3}	& \ctrl{1}	& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}	& \qw		& \qw		& \qw		& \ctrl{1}	& \ctrl{3}	& \qw		& \qw		& \qw		& \qw		& \rstick{$a_0$} \\
	\lstick{$b_0$} & \qw		& \ctrl{1}	& \ctrl{1}	& \ctrl{1}	& \qw		& \qw		& \qw		& \targ{}	& \qw		& \qw		& \qw		& \qw		& \ctrl{2}	& \targ{}	& \ctrl{2}	& \qw		& \qw		& \targ{}	& \targ{}	& \targ{}	& \qw		& \qw		& \ctrl{2}	& \targ{}	& \ctrl{2}	& \targ{}	& \qw		& \qw		& \qw		& \rstick{$s_0$} \\
	\lstick{$0$}   & \qw		& \targ{}	& \targ{}	& \targ{}	& \ctrl{4}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \rstick{$c_1$} \\
	\lstick{$0$}   & \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \qw		& \targ{}	& \ctrl{4}	& \qw		& \ctrl{2}	& \qw		& \qw		& \qw		& \ctrl{4}	& \targ{}	& \qw		& \targ{}	& \qw		& \qw		& \qw		& \qw		& \rstick{$0$} \\
	\lstick{$a_1$} & \qw		& \ctrl{2}	& \ctrl{1}	& \qw		& \qw		& \qw		& \qw		& \ctrl{1}	& \qw		& \qw		& \qw		& \qw		& \ctrl{3}	& \ctrl{1}	& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}	& \qw		& \qw		& \qw		& \ctrl{1}	& \ctrl{3}	& \qw		& \qw		& \qw		& \qw		& \rstick{$a_1$} \\
	\lstick{$b_1$} & \qw		& \ctrl{1}	& \targ{}	& \qw		& \ctrl{1}	& \qw		& \qw		& \targ{}	& \qw		& \qw		& \qw		& \qw		& \ctrl{2}	& \targ{}	& \qw		& \ctrl{2}	& \qw		& \targ{}	& \targ{}	& \targ{}	& \qw		& \ctrl{2}	& \qw		& \targ{}	& \ctrl{2}	& \targ{}	& \qw		& \qw		& \qw		& \rstick{$s_1$} \\
	\lstick{$0$}   & \qw		& \targ{}	& \qw		& \qw		& \targ{}	& \ctrl{8}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \rstick{$c_2$} \\
	\lstick{$0$}   & \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \qw		& \qw		& \targ{}	& \ctrl{3}	& \ctrl{2}	& \qw		& \qw		& \ctrl{3}	& \targ{}	& \qw		& \qw		& \targ{}	& \qw		& \qw		& \qw		& \qw		& \rstick{$0$} \\
	\lstick{$a_2$} & \qw		& \ctrl{3}	& \ctrl{1}	& \qw		& \qw		& \qw		& \qw		& \ctrl{1}	& \qw		& \qw		& \qw		& \qw		& \ctrl{2}	& \ctrl{1}	& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}	& \qw		& \qw		& \qw		& \ctrl{1}	& \ctrl{2}	& \qw		& \qw		& \qw		& \qw		& \rstick{$a_2$} \\
	\lstick{$b_2$} & \qw		& \ctrl{2}	& \targ{}	& \ctrl{1}	& \qw		& \qw		& \ctrl{1}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \ctrl{1}	& \targ{}	& \qw		& \qw		& \ctrl{1}	& \targ{}	& \targ{}	& \targ{}	& \ctrl{1}	& \qw		& \qw		& \targ{}	& \ctrl{1}	& \targ{}	& \qw		& \qw		& \qw		& \rstick{$s_2$} \\
	\lstick{$0$}   & \qw		& \qw		& \qw		& \targ{}	& \qw		& \ctrl{4}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \qw		& \qw		& \qw		& \targ{}	& \ctrl{3}	& \qw		& \qw		& \targ{}	& \qw		& \qw		& \qw		& \targ{}	& \qw		& \qw		& \qw		& \qw		& \rstick{$0$} \\
	\lstick{$0$}   & \qw		& \targ{}	& \qw		& \qw		& \ctrl{3}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \rstick{$c_3$} \\
	\lstick{$a_3$} & \qw		& \ctrl{2}	& \ctrl{1}	& \qw		& \qw		& \qw		& \qw		& \ctrl{1}	& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}	& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}	& \qw		& \qw		& \qw		& \ctrl{1}	& \qw		& \qw		& \qw		& \qw		& \qw		& \rstick{$a_3$} \\
	\lstick{$b_3$} & \qw		& \ctrl{1}	& \targ{}	& \ctrl{-3}	& \ctrl{1}	& \qw		& \ctrl{-3}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \qw		& \qw		& \qw		& \targ{}	& \targ{}	& \targ{}	& \qw		& \qw		& \qw		& \targ{}	& \qw		& \targ{}	& \qw		& \qw		& \qw		& \rstick{$s_3$} \\
	\lstick{$0$}   & \qw		& \targ{}	& \qw		& \qw		& \targ{}	& \targ{}	& \qw		& \qw		& \qw		& \ctrl{-15}& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{-15}& \qw		& \rstick{$c_4$}
\end{quantikz}
}

\newcommand{\ProposedModuloAdder}{
\begin{quantikz} [row sep= \rowSep, column sep= \colSep, transparent]
	\lstick{$1$}   & \qw		& \qw		& \qw		& \ctrl{3}	& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \targ{}	& \qw		& \qw		& \qw		& \ctrl{4}	& \qw		& \qw		& \ctrl{2}	& \qw		& \qw		& \qw		& \qw		& \ctrl{4}	& \qw		& \qw		& \qw		& \qw		& \targ{}	& \qw		& \rstick{$1$} \\
	%\lstick{$0$}   & \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \rstick{$0$} \\
	\lstick{$a_0$} & \qw		& \ctrl{2}	& \qw		& \qw		& \ctrl{1}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{3}	& \ctrl{1}	& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}	& \qw		& \qw		& \qw		& \ctrl{1}	& \ctrl{3}	& \qw		& \qw		& \qw		& \qw		& \rstick{$a_0$} \\
	\lstick{$b_0$} & \qw		& \ctrl{1}	& \ctrl{1}	& \ctrl{1}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{2}	& \targ{}	& \ctrl{2}	& \qw		& \qw		& \targ{}	& \targ{}	& \targ{}	& \qw		& \qw		& \ctrl{2}	& \targ{}	& \ctrl{2}	& \targ{}	& \qw		& \qw		& \qw		& \rstick{$s_0$} \\
	\lstick{$0$}   & \qw		& \targ{}	& \targ{}	& \targ{}	& \ctrl{4}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \rstick{$c_1$} \\
	\lstick{$0$}   & \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \qw		& \targ{}	& \ctrl{4}	& \qw		& \ctrl{2}	& \qw		& \qw		& \qw		& \ctrl{4}	& \targ{}	& \qw		& \targ{}	& \qw		& \qw		& \qw		& \qw		& \rstick{$0$} \\
	\lstick{$a_1$} & \qw		& \ctrl{2}	& \ctrl{1}	& \qw		& \qw		& \ctrl{1}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{3}	& \ctrl{1}	& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}	& \qw		& \qw		& \qw		& \ctrl{1}	& \ctrl{3}	& \qw		& \qw		& \qw		& \qw		& \rstick{$a_1$} \\
	\lstick{$b_1$} & \qw		& \ctrl{1}	& \targ{}	& \qw		& \ctrl{1}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{2}	& \targ{}	& \qw		& \ctrl{2}	& \qw		& \targ{}	& \targ{}	& \targ{}	& \qw		& \ctrl{2}	& \qw		& \targ{}	& \ctrl{2}	& \targ{}	& \qw		& \qw		& \qw		& \rstick{$s_1$} \\
	\lstick{$0$}   & \qw		& \targ{}	& \qw		& \qw		& \targ{}	& \ctrl{8}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \rstick{$c_2$} \\
	\lstick{$0$}   & \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \qw		& \qw		& \targ{}	& \ctrl{3}	& \ctrl{2}	& \qw		& \qw		& \ctrl{3}	& \targ{}	& \qw		& \qw		& \targ{}	& \qw		& \qw		& \qw		& \qw		& \rstick{$0$} \\
	\lstick{$a_2$} & \qw		& \ctrl{3}	& \ctrl{1}	& \qw		& \qw		& \qw		& \qw		& \ctrl{1}	& \qw		& \qw		& \qw		& \qw		& \ctrl{2}	& \ctrl{1}	& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}	& \qw		& \qw		& \qw		& \ctrl{1}	& \ctrl{2}	& \qw		& \qw		& \qw		& \qw		& \rstick{$a_2$} \\
	\lstick{$b_2$} & \qw		& \ctrl{2}	& \targ{}	& \ctrl{1}	& \qw		& \qw		& \ctrl{1}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \ctrl{1}	& \targ{}	& \qw		& \qw		& \ctrl{1}	& \targ{}	& \targ{}	& \targ{}	& \ctrl{1}	& \qw		& \qw		& \targ{}	& \ctrl{1}	& \targ{}	& \qw		& \qw		& \qw		& \rstick{$s_2$} \\
	\lstick{$0$}   & \qw		& \qw		& \qw		& \targ{}	& \qw		& \ctrl{4}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \qw		& \qw		& \qw		& \targ{}	& \ctrl{3}	& \qw		& \qw		& \targ{}	& \qw		& \qw		& \qw		& \targ{}	& \qw		& \qw		& \qw		& \qw		& \rstick{$0$} \\
	\lstick{$0$}   & \qw		& \targ{}	& \qw		& \qw		& \ctrl{3}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \rstick{$c_3$} \\
	\lstick{$a_3$} & \qw		& \ctrl{2}	& \ctrl{1}	& \qw		& \qw		& \qw		& \qw		& \ctrl{1}	& \qw		& \qw		& \qw		& \qw		& \ctrl{1}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}	& \qw		& \qw		& \qw		& \ctrl{1}	& \qw		& \qw		& \qw		& \qw		& \qw		& \rstick{$a_3$} \\
	\lstick{$b_3$} & \qw		& \ctrl{1}	& \targ{}	& \ctrl{-3}	& \ctrl{1}	& \qw		& \ctrl{-3}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \targ{}	& \qw		& \qw		& \qw		& \qw		& \targ{}	& \targ{}	& \targ{}	& \qw		& \qw		& \qw		& \targ{}	& \qw		& \targ{}	& \qw		& \qw		& \qw		& \rstick{$s_3$} \\
	\lstick{$0$}   & \qw		& \targ{}	& \qw		& \qw		& \targ{}	& \targ{}	& \qw		& \qw		& \qw		& \ctrl{-15}& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{-15}& \qw		& \rstick{$c_4$}
\end{quantikz}
}


\newcommand{\thapliyalThirteen}{
\begin{quantikz} [row sep= \rowSep, column sep= \colSep, transparent]
	\lstick{$a_0$} & \qw	   & \qw		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw & \rstick{$s_0$} \\
	\lstick{$b_0$} & \qw 	   & \qw 		& \qw 		& \qw 		& \ctrl{2}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \qw 		& \qw		& \qw & \rstick{$b_0$} \\
	\lstick{$a_1$} & \targ{}   & \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \targ{}	& \qw & \rstick{$s_1$} \\
	\lstick{$b_1$} & \ctrl{-1} & \qw 		& \qw 		& \ctrl{2}	& \targ{}	& \ctrl{2}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \targ{}	& \ctrl{2}	& \qw 		& \ctrl{-1}	& \qw & \rstick{$b_1$} \\
	\lstick{$a_2$} & \targ{}   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \qw & \rstick{$s_2$} \\
	\lstick{$b_2$} & \ctrl{-1} & \qw 		& \ctrl{2}	& \targ{}	& \qw 		& \targ{}	& \ctrl{2}	& \qw 		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \targ{}	& \ctrl{2}	& \ctrl{-1}	& \qw & \rstick{$b_2$} \\
	\lstick{$a_3$} & \targ{}   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \qw & \rstick{$s_3$} \\
	\lstick{$b_3$} & \ctrl{-1} & \ctrl{1} 	& \targ{}	& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{1}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{-1}	& \qw & \rstick{$b_3$} \\
	\lstick{$z$}   & \qw       & \targ{} 	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$z \oplus s_4$}			
\end{quantikz}
}

\newcommand{\thapliyalThirteenFive}{
\begin{quantikz} [row sep= \rowSep, column sep= \colSep, transparent]
	\lstick{$a_0$} & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw		& \qw 		& \qw      & \targ{}	& \qw & \rstick{$s_0$} \\
	\lstick{$b_0$} & \qw	   & \qw 	   & \qw 		& \qw 		& \qw 		& \ctrl{2}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{2}	& \qw		& \qw 		& \qw      & \ctrl{-1}	& \qw & \rstick{$b_0$} \\
	\lstick{$a_1$} & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw & \rstick{$s_1$} \\
	\lstick{$b_1$} & \ctrl{-1} & \qw	   & \qw 		& \qw 		& \ctrl{2}	& \targ{}	& \ctrl{2}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \targ{}	& \ctrl{2}	& \qw 		& \qw      & \ctrl{-1}	& \qw & \rstick{$b_1$} \\
	\lstick{$a_2$} & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw & \rstick{$s_2$} \\
	\lstick{$b_2$} & \ctrl{-1} & \qw	   & \qw 		& \ctrl{2}	& \targ{}	& \qw 		& \targ{}	& \ctrl{2}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \targ{}	& \ctrl{2}	& \qw      & \ctrl{-1}	& \qw & \rstick{$b_2$} \\
	\lstick{$a_3$} & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw  		& \qw  		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw & \rstick{$s_3$} \\
	\lstick{$b_3$} & \ctrl{-1} & \qw	   & \ctrl{2}  	& \targ{}	& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{2}	& \qw  		& \qw  		& \ctrl{2}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{2} & \ctrl{-1}	& \qw & \rstick{$b_3$} \\
	\lstick{$a_4$} & \targ{}   & \qw	   & \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}  & \targ{}  	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw      & \targ{}	& \qw & \rstick{$s_4$} \\		
	\lstick{$b_4$} & \ctrl{-1} & \ctrl{1}  & \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \ctrl{1}  & \ctrl{-1}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}  & \ctrl{-1}	& \qw & \rstick{$b_4$} \\		
	\lstick{$z$}   & \qw       & \targ{}   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw 		& \targ{}  	& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \qw 		& \qw & \rstick{$z \oplus s_5$}			
\end{quantikz}
}

\newcommand{\thapliyalThirteenFiveGap}{
\begin{quantikz} [row sep= \rowSep, column sep= \colSep, transparent]
	\lstick{$0$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw & \rstick{$0$} \\
	\lstick{$a_0$} & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw		& \qw 		& \qw      & \targ{}	& \qw & \rstick{$s_0$} \\
	\lstick{$b_0$} & \qw	   & \qw 	   & \qw 		& \qw 		& \qw 		& \ctrl{3}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \qw		& \qw 		& \qw      & \ctrl{-1}	& \qw & \rstick{$b_0$} \\
	\lstick{$0$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw & \rstick{$0$} \\
	\lstick{$a_1$} & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw & \rstick{$s_1$} \\
	\lstick{$b_1$} & \ctrl{-1} & \qw	   & \qw 		& \qw 		& \ctrl{3}	& \targ{}	& \ctrl{3}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \ctrl{3}	& \qw 		& \qw      & \ctrl{-1}	& \qw & \rstick{$b_1$} \\
	\lstick{$0$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw & \rstick{$0$} \\
	\lstick{$a_2$} & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw & \rstick{$s_2$} \\
	\lstick{$b_2$} & \ctrl{-1} & \qw	   & \qw 		& \ctrl{3}	& \targ{}	& \qw 		& \targ{}	& \ctrl{3}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \targ{}	& \ctrl{3}	& \qw      & \ctrl{-1}	& \qw & \rstick{$b_2$} \\
	\lstick{$0$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw & \rstick{$0$} \\
	\lstick{$a_3$} & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw  		& \qw  		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw & \rstick{$s_3$} \\
	\lstick{$b_3$} & \ctrl{-1} & \qw	   & \ctrl{3}  	& \targ{}	& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{3}	& \qw  		& \qw  		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{3} & \ctrl{-1}	& \qw & \rstick{$b_3$} \\
	\lstick{$0$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw & \rstick{$0$} \\
	\lstick{$a_4$} & \targ{}   & \qw	   & \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}  & \targ{}  	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw      & \targ{}	& \qw & \rstick{$s_4$} \\		
	\lstick{$b_4$} & \ctrl{-1} & \ctrl{1}  & \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \ctrl{1}  & \ctrl{-1}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}  & \ctrl{-1}	& \qw & \rstick{$b_4$} \\		
	\lstick{$z$}   & \qw       & \targ{}   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw 		& \targ{}  	& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \qw 		& \qw & \rstick{$z \oplus s_5$}\\
	\lstick{$0$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw & \rstick{$0$}		
\end{quantikz}
}

\newcommand{\thapliyalThirteenFiveNOR}{
\begin{quantikz} [row sep= \rowSep, column sep= \rowSep, transparent]
	\lstick{$0$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw 		& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$0$} \\
	\lstick{$a_0$} & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw		& \qw 		& \qw      & \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$s_0$} \\
	\lstick{$b_0$} & \qw	   & \qw 	   & \qw 		& \qw 		& \qw 		& \ctrl{3}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \qw		& \qw 		& \qw      & \ctrl{-1}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_0$} \\
	\lstick{$0$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$0$} \\
	\lstick{$a_1$} & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$s_1$} \\
	\lstick{$b_1$} & \ctrl{-1} & \qw	   & \qw 		& \qw 		& \ctrl{3}	& \targ{}	& \ctrl{3}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \ctrl{3}	& \qw 		& \qw      & \ctrl{-1}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_1$} \\
	\lstick{$0$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$0$} \\
	\lstick{$a_2$} & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$s_2$} \\
	\lstick{$b_2$} & \ctrl{-1} & \qw	   & \qw 		& \ctrl{3}	& \targ{}	& \qw 		& \targ{}	& \ctrl{3}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \targ{}	& \ctrl{3}	& \qw      & \ctrl{-1}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_2$} \\
	\lstick{$0$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$0$} \\
	\lstick{$a_3$} & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw  		& \qw  		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$s_3$} \\
	\lstick{$b_3$} & \ctrl{-1} & \qw	   & \ctrl{3}  	& \targ{}	& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{3}	& \qw  		& \qw  		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{3} & \ctrl{-1}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_3$} \\
	\lstick{$0$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$0$} \\
	\lstick{$a_4$} & \targ{}   & \qw	   & \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}  & \targ{}  	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw      & \targ{}	& \targ{}	& \ctrl{-13}& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$s_4$} \\		
	\lstick{$b_4$} & \ctrl{-1} & \ctrl{1}  & \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \ctrl{1}  & \ctrl{-1}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}  & \ctrl{-1}	& \qw	 	& \qw		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_4$} \\		
	\lstick{$z$}   & \qw       & \targ{}   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw 		& \targ{}  	& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \qw 		& \targ{}	& \ctrl{-2}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$z \oplus s_5$}\\
	\lstick{$0$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw	 	& \qw		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$0$}		
\end{quantikz}
}

\newcommand{\QMAoneBoxed}{
\begin{quantikz} [row sep= 0.08cm, column sep= 0.04cm, transparent]
	\lstick{$0$}   & \qw	& \qw\gategroup[wires=17,steps=22,style={blue!75!black, thick, dashed, rounded corners, inner xsep=2pt}, background]{{\sc full adder stage generating Sum}} & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw	& \qw 		& \targ{}	& \qw 		& \qw	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw		& \qw 		& \qw 		& \targ{}	& \qw & \rstick{$m_0$} \\
	\lstick{$a_0$} & \qw	& \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw		& \qw 		& \qw      & \targ{}	& \qw	& \qw 		& \qw 		& \qw 		& \qw	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \qw		& \qw 		& \qw 		& \ctrl{-1}	& \qw & \rstick{$s_0$} \\
	\lstick{$b_0$} & \qw	& \qw	   & \qw 	   & \qw 		& \qw 		& \qw 		& \ctrl{3}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \qw		& \qw 		& \qw      & \ctrl{-1}	& \qw	& \qw 		& \qw 		& \qw 		& \qw	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_0$} \\
	\lstick{$0$}   & \qw	& \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw	& \qw 		& \qw 		& \qw 		& \qw	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw		& \qw 		& \targ{}	& \qw & \rstick{$m_1$} \\
	\lstick{$a_1$} & \qw	& \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw	& \qw 		& \qw 		& \qw 		& \qw	& \ctrl{-1}	& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \targ{}	& \ctrl{3}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \ctrl{3}	& \qw		& \qw 		& \ctrl{-1}	& \qw & \rstick{$s_1$} \\
	\lstick{$b_1$} & \qw	& \ctrl{-1} & \qw	   & \qw 		& \qw 		& \ctrl{3}	& \targ{}	& \ctrl{3}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \ctrl{3}	& \qw 		& \qw      & \ctrl{-1}	& \qw	& \qw 		& \qw 		& \qw 		& \qw	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_1$} \\
	\lstick{$0$}   & \qw	& \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw	& \qw 		& \qw 		& \qw 		& \qw	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \qw & \rstick{$m_2$} \\
	\lstick{$a_2$} & \qw	& \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw	& \qw 		& \qw 		& \qw 		& \qw	& \ctrl{-1}	& \qw 		& \qw 		& \ctrl{3}	& \targ{}	& \qw 		& \targ{}	& \ctrl{3}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \targ{}	& \ctrl{3}	& \qw 		& \ctrl{-1}	& \qw & \rstick{$s_2$} \\
	\lstick{$b_2$} & \qw	& \ctrl{-1} & \qw	   & \qw 		& \ctrl{3}	& \targ{}	& \qw 		& \targ{}	& \ctrl{3}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \targ{}	& \ctrl{3}	& \qw      & \ctrl{-1}	& \qw	& \qw 		& \qw 		& \qw 		& \qw	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_2$} \\
	\lstick{$0$}   & \qw	& \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw	& \qw 		& \qw 		& \qw 		& \qw	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \qw & \rstick{$m_3$} \\
	\lstick{$a_3$} & \qw	& \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw  		& \qw  		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw	& \qw 		& \qw 		& \qw 		& \qw	& \ctrl{-1}	& \qw 		& \ctrl{5}	& \targ{}	& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{5}	& \qw		& \qw 		& \ctrl{5}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{5}	& \ctrl{-1}	& \qw & \rstick{$s_3$} \\
	\lstick{$b_3$} & \qw	& \ctrl{-1} & \qw	   & \ctrl{3}  	& \targ{}	& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{3}	& \qw  		& \qw  		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{3} & \ctrl{-1}	& \qw	& \qw 		& \qw 		& \qw 		& \qw	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_3$} \\
	\lstick{$0$}   & \qw	& \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw	& \qw 		& \qw 		& \qw 		& \qw	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \qw & \rstick{$m_4$} \\
	\lstick{$a_4$} & \qw	& \targ{}   & \qw	   & \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}  & \targ{}  	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw      & \targ{}	& \qw	& \targ{}	& \ctrl{-13}& \targ{}	& \qw	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$s_4$} \\		
	\lstick{$b_4$} & \qw	& \ctrl{-1} & \ctrl{1}  & \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \ctrl{1}  & \ctrl{-1}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}  & \ctrl{-1}	& \qw	& \qw	 	& \qw		& \qw		& \qw	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_4$} \\		
	\lstick{$0$}   & \qw	& \qw       & \targ{}   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw 		& \targ{}  	& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \qw 		& \qw	& \targ{}	& \ctrl{-2}	& \targ{}	& \qw	& \ctrl{-3}	& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{1}	& \ctrl{-3}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{-3}	& \qw & \rstick{$s_5$}\\
	\lstick{$0$}   & \qw	& \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw	& \qw	 	& \qw		& \qw		& \qw	& \qw 		& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$s_6$}			
\end{quantikz}
}

\newcommand{\QMAoneSliced}{
\begin{quantikz} [row sep= 0.1cm, column sep= 0.05cm, transparent]
	\lstick{$0$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw\slice[style=blue]{1} & \qw & \qw		& \targ{}	& \qw\slice[style=blue]{2} & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw		& \qw 		& \qw 		& \targ{}	& \qw & \rstick{$m_0$} \\
	\lstick{$a_0$} & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw		& \qw 		& \qw      & \targ{}				  & \qw	& \qw 		& \qw 		& \qw 					   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \qw		& \qw 		& \qw 		& \ctrl{-1}	& \qw & \rstick{$s_0$} \\
	\lstick{$b_0$} & \qw	   & \qw 	   & \qw 		& \qw 		& \qw 		& \ctrl{3}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \qw		& \qw 		& \qw      & \ctrl{-1}				  & \qw	& \qw 		& \qw 		& \qw 					   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_0$} \\
	\lstick{$0$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw					  & \qw	& \qw 		& \qw 		& \qw 					   & \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw		& \qw 		& \targ{}	& \qw & \rstick{$m_1$} \\
	\lstick{$a_1$} & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw      & \targ{}				  & \qw	& \qw 		& \qw 		& \qw 					   & \ctrl{-1}	& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \targ{}	& \ctrl{3}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \ctrl{3}	& \qw		& \qw 		& \ctrl{-1}	& \qw & \rstick{$s_1$} \\
	\lstick{$b_1$} & \ctrl{-1} & \qw	   & \qw 		& \qw 		& \ctrl{3}	& \targ{}	& \ctrl{3}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \ctrl{3}	& \qw 		& \qw      & \ctrl{-1}				  & \qw	& \qw 		& \qw 		& \qw 					   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_1$} \\
	\lstick{$0$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw					  & \qw	& \qw 		& \qw 		& \qw 					   & \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \qw & \rstick{$m_2$} \\
	\lstick{$a_2$} & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}				  & \qw	& \qw 		& \qw 		& \qw 					   & \ctrl{-1}	& \qw 		& \qw 		& \ctrl{3}	& \targ{}	& \qw 		& \targ{}	& \ctrl{3}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \targ{}	& \ctrl{3}	& \qw 		& \ctrl{-1}	& \qw & \rstick{$s_2$} \\
	\lstick{$b_2$} & \ctrl{-1} & \qw	   & \qw 		& \ctrl{3}	& \targ{}	& \qw 		& \targ{}	& \ctrl{3}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \targ{}	& \ctrl{3}	& \qw      & \ctrl{-1}				  & \qw	& \qw 		& \qw 		& \qw 					   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_2$} \\
	\lstick{$0$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw					  & \qw	& \qw 		& \qw 		& \qw 					   & \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \qw & \rstick{$m_3$} \\
	\lstick{$a_3$} & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw  		& \qw  		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}				  & \qw	& \qw 		& \qw 		& \qw 					   & \ctrl{-1}	& \qw 		& \ctrl{5}	& \targ{}	& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{5}	& \qw		& \qw 		& \ctrl{5}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{5}	& \ctrl{-1}	& \qw & \rstick{$s_3$} \\
	\lstick{$b_3$} & \ctrl{-1} & \qw	   & \ctrl{3}  	& \targ{}	& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{3}	& \qw  		& \qw  		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{3} & \ctrl{-1}				  & \qw	& \qw 		& \qw 		& \qw 					   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_3$} \\
	\lstick{$0$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw					  & \qw	& \qw 		& \qw 		& \qw 					   & \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \qw & \rstick{$m_4$} \\
	\lstick{$a_4$} & \targ{}   & \qw	   & \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}  & \targ{}  	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw      & \targ{}				  & \qw	& \targ{}	& \ctrl{-13}& \targ{}				   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$s_4$} \\		
	\lstick{$b_4$} & \ctrl{-1} & \ctrl{1}  & \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \ctrl{1}  & \ctrl{-1}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}  & \ctrl{-1}				  & \qw	& \qw	 	& \qw		& \qw					   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_4$} \\		
	\lstick{$0$}   & \qw       & \targ{}   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw 		& \targ{}  	& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \qw 					  & \qw	& \targ{}	& \ctrl{-2}	& \targ{}				   & \ctrl{-3}	& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{1}	& \ctrl{-3}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{-3}	& \qw & \rstick{$s_5$}\\
	\lstick{$0$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw					  & \qw	& \qw	 	& \qw		& \qw					   & \qw 		& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$s_6$}			
\end{quantikz}
}

\newcommand{\QMAone}{
\begin{quantikz} [row sep= 0.08cm, column sep= 0.03cm, transparent]
	\lstick{$0$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw 		& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw		& \qw 		& \qw 		& \targ{}	& \qw & \rstick{$m_0$} \\
	\lstick{$a_0$} & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw		& \qw 		& \qw      & \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \qw		& \qw 		& \qw 		& \ctrl{-1}	& \qw & \rstick{$s_0$} \\
	\lstick{$b_0$} & \qw	   & \qw 	   & \qw 		& \qw 		& \qw 		& \ctrl{3}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \qw		& \qw 		& \qw      & \ctrl{-1}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_0$} \\
	\lstick{$0$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw 		& \qw 		& \qw 		& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw		& \qw 		& \targ{}	& \qw & \rstick{$m_1$} \\
	\lstick{$a_1$} & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw 		& \qw 		& \qw 		& \ctrl{-1}	& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \targ{}	& \ctrl{3}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \ctrl{3}	& \qw		& \qw 		& \ctrl{-1}	& \qw & \rstick{$s_1$} \\
	\lstick{$b_1$} & \ctrl{-1} & \qw	   & \qw 		& \qw 		& \ctrl{3}	& \targ{}	& \ctrl{3}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \ctrl{3}	& \qw 		& \qw      & \ctrl{-1}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_1$} \\
	\lstick{$0$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw 		& \qw 		& \qw 		& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \qw & \rstick{$m_2$} \\
	\lstick{$a_2$} & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw 		& \qw 		& \qw 		& \ctrl{-1}	& \qw 		& \qw 		& \ctrl{3}	& \targ{}	& \qw 		& \targ{}	& \ctrl{3}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \targ{}	& \ctrl{3}	& \qw 		& \ctrl{-1}	& \qw & \rstick{$s_2$} \\
	\lstick{$b_2$} & \ctrl{-1} & \qw	   & \qw 		& \ctrl{3}	& \targ{}	& \qw 		& \targ{}	& \ctrl{3}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \targ{}	& \ctrl{3}	& \qw      & \ctrl{-1}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_2$} \\
	\lstick{$0$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw 		& \qw 		& \qw 		& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \qw & \rstick{$m_3$} \\
	\lstick{$a_3$} & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw  		& \qw  		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw 		& \qw 		& \qw 		& \ctrl{-1}	& \qw 		& \ctrl{5}	& \targ{}	& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{5}	& \qw		& \qw 		& \ctrl{5}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{5}	& \ctrl{-1}	& \qw & \rstick{$s_3$} \\
	\lstick{$b_3$} & \ctrl{-1} & \qw	   & \ctrl{3}  	& \targ{}	& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{3}	& \qw  		& \qw  		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{3} & \ctrl{-1}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_3$} \\
	\lstick{$0$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw 		& \qw 		& \qw 		& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \qw & \rstick{$m_4$} \\
	\lstick{$a_4$} & \targ{}   & \qw	   & \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}  & \targ{}  	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw      & \targ{}	& \targ{}	& \ctrl{-13}& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$s_4$} \\		
	\lstick{$b_4$} & \ctrl{-1} & \ctrl{1}  & \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \ctrl{1}  & \ctrl{-1}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}  & \ctrl{-1}	& \qw	 	& \qw		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_4$} \\		
	\lstick{$0$}   & \qw       & \targ{}   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw 		& \targ{}  	& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \qw 		& \targ{}	& \ctrl{-2}	& \targ{}	& \ctrl{-3}	& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{1}	& \ctrl{-3}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{-3}	& \qw & \rstick{$s_5$}\\
	\lstick{$0$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw	 	& \qw		& \qw		& \qw 		& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$s_6$}			
\end{quantikz}
}

\newcommand{\QMAtwoBoxed}{
\begin{quantikz} [row sep= 0.1cm, column sep= 0.05cm, transparent]
	\lstick{$0$}   & \qw   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw 		& \targ{}	& \qw  		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$m_0$} \\
	\lstick{$a_0$} & \qw   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw		& \qw 		& \qw      & \targ{}	& \qw 		& \qw 		& \qw  		& \ctrl{2}	& \ctrl{-1}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$s_0$} \\
	\lstick{$b_0$} & \qw   & \qw	   & \qw 	   & \qw 		& \qw 		& \qw 		& \ctrl{3}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \qw		& \qw 		& \qw      & \ctrl{-1}	& \qw 		& \qw 		& \qw  		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_0$} \\
	\lstick{$0$}   & \qw   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw 		& \qw 		& \qw  		& \targ{}	& \ctrl{1}	& \targ{  }	& \qw 		& \qw 		& \qw 		& \qw & \rstick{$m_1$} \\
	\lstick{$a_1$} & \qw   & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw 		& \qw 		& \qw  		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \qw 		& \qw 		& \qw 		& \qw & \rstick{$s_1$} \\
	\lstick{$b_1$} & \qw   & \ctrl{-1} & \qw	   & \qw 		& \qw 		& \ctrl{3}	& \targ{}	& \ctrl{3}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \ctrl{3}	& \qw 		& \qw      & \ctrl{-1}	& \qw 		& \qw 		& \qw  		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_1$} \\
	\lstick{$0$}   & \qw   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw 		& \qw 		& \qw  		& \qw 		& \targ{}	& \ctrl{1}	& \targ{  }	& \qw 		& \qw 		& \qw & \rstick{$m_2$} \\
	\lstick{$a_2$} & \qw   & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw 		& \qw 		& \qw  		& \qw 		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \qw 		& \qw 		& \qw & \rstick{$s_2$} \\
	\lstick{$b_2$} & \qw   & \ctrl{-1} & \qw	   & \qw 		& \ctrl{3}	& \targ{}	& \qw 		& \targ{}	& \ctrl{3}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \targ{}	& \ctrl{3}	& \qw      & \ctrl{-1}	& \qw 		& \qw 		& \qw  		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_2$} \\
	\lstick{$0$}   & \qw   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw 		& \qw 		& \qw  		& \qw 		& \qw 		& \targ{}	& \ctrl{1}	& \targ{  }	& \qw 		& \qw & \rstick{$m_3$} \\
	\lstick{$a_3$} & \qw   & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw  		& \qw  		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw 		& \qw 		& \qw  		& \qw 		& \qw 		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \qw 		& \qw & \rstick{$s_3$} \\
	\lstick{$b_3$} & \qw   & \ctrl{-1} & \qw	   & \ctrl{3}  	& \targ{}	& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{3}	& \qw  		& \qw  		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{3} & \ctrl{-1}	& \qw 		& \qw 		& \qw  		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_3$} \\
	\lstick{$0$}   & \qw   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw 		& \qw 		& \qw  		& \qw 		& \qw 		& \qw 		& \targ{}	& \targ{}	& \qw 		& \qw & \rstick{$m_4$} \\
	\lstick{$a_4$} & \qw   & \targ{}   & \qw	   & \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}  & \targ{}  	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw      & \targ{}	& \targ{}	& \ctrl{-13}& \targ{}	& \qw		& \qw 		& \qw 		& \qw 		& \qw		& \qw 		& \qw & \rstick{$s_4$} \\		
	\lstick{$b_4$} & \qw   & \ctrl{-1} & \ctrl{1}  & \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \ctrl{1}  & \ctrl{-1}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}  & \ctrl{-1}	& \qw	 	& \qw		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_4$} \\		
	\lstick{$0$}   & \qw   & \qw       & \targ{}   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw 		& \targ{}  	& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \qw 		& \targ{}	& \ctrl{-2}	& \targ{}	& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{-3}	& \qw 		& \qw & \rstick{$s_5$}
\end{quantikz}
}

\newcommand{\QMAtwo}{
\begin{quantikz} [row sep= 0.1cm, column sep= 0.05cm, transparent]
	\lstick{$0$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw 		& \targ{}	& \qw  		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$m_0$} \\
	\lstick{$a_0$} & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw		& \qw 		& \qw      & \targ{}	& \qw 		& \qw 		& \qw  		& \ctrl{2}	& \ctrl{-1}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$s_0$} \\
	\lstick{$b_0$} & \qw	   & \qw 	   & \qw 		& \qw 		& \qw 		& \ctrl{3}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \qw		& \qw 		& \qw      & \ctrl{-1}	& \qw 		& \qw 		& \qw  		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_0$} \\
	\lstick{$0$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw 		& \qw 		& \qw  		& \targ{}	& \ctrl{1}	& \targ{  }	& \qw 		& \qw 		& \qw 		& \qw & \rstick{$m_1$} \\
	\lstick{$a_1$} & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw 		& \qw 		& \qw  		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \qw 		& \qw 		& \qw 		& \qw & \rstick{$s_1$} \\
	\lstick{$b_1$} & \ctrl{-1} & \qw	   & \qw 		& \qw 		& \ctrl{3}	& \targ{}	& \ctrl{3}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \ctrl{3}	& \qw 		& \qw      & \ctrl{-1}	& \qw 		& \qw 		& \qw  		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_1$} \\
	\lstick{$0$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw 		& \qw 		& \qw  		& \qw 		& \targ{}	& \ctrl{1}	& \targ{  }	& \qw 		& \qw 		& \qw & \rstick{$m_2$} \\
	\lstick{$a_2$} & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw 		& \qw 		& \qw  		& \qw 		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \qw 		& \qw 		& \qw & \rstick{$s_2$} \\
	\lstick{$b_2$} & \ctrl{-1} & \qw	   & \qw 		& \ctrl{3}	& \targ{}	& \qw 		& \targ{}	& \ctrl{3}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \targ{}	& \ctrl{3}	& \qw      & \ctrl{-1}	& \qw 		& \qw 		& \qw  		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_2$} \\
	\lstick{$0$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw 		& \qw 		& \qw  		& \qw 		& \qw 		& \targ{}	& \ctrl{1}	& \targ{  }	& \qw 		& \qw & \rstick{$m_3$} \\
	\lstick{$a_3$} & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw  		& \qw  		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw 		& \qw 		& \qw  		& \qw 		& \qw 		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \qw 		& \qw & \rstick{$s_3$} \\
	\lstick{$b_3$} & \ctrl{-1} & \qw	   & \ctrl{3}  	& \targ{}	& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{3}	& \qw  		& \qw  		& \ctrl{3}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{3} & \ctrl{-1}	& \qw 		& \qw 		& \qw  		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_3$} \\
	\lstick{$0$}   & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw 		& \qw 		& \qw  		& \qw 		& \qw 		& \qw 		& \targ{}	& \targ{}	& \qw 		& \qw & \rstick{$m_4$} \\
	\lstick{$a_4$} & \targ{}   & \qw	   & \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}  & \targ{}  	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw      & \targ{}	& \targ{}	& \ctrl{-13}& \targ{}	& \qw		& \qw 		& \qw 		& \qw 		& \qw		& \qw 		& \qw & \rstick{$s_4$} \\		
	\lstick{$b_4$} & \ctrl{-1} & \ctrl{1}  & \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \ctrl{1}  & \ctrl{-1}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}  & \ctrl{-1}	& \qw	 	& \qw		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{$b_4$} \\		
	\lstick{$0$}   & \qw       & \targ{}   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw 		& \targ{}  	& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \qw 		& \targ{}	& \ctrl{-2}	& \targ{}	& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{-3}	& \qw 		& \qw & \rstick{$s_5$}
\end{quantikz}
}

\newcommand{\QMAtwoLessQubits}{
\begin{quantikz} [row sep= 0.1cm, column sep= 0.05cm, transparent]
	\lstick{\ket{0}}& \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw 		& \targ{}	& \qw  				& \qw 	& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw & \rstick{$m_0$} \\
	\lstick{$a_0$} & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw		& \qw 		& \qw      & \targ{}	& \qw 		& \qw 		& \qw  				& \qw 	& \ctrl{1}	& \ctrl{-1}	& \qw 		& \qw 		& \qw 		& \qw & \rstick{$s_0$} \\
	\lstick{$b_0$} & \qw	   & \qw 	   & \qw 		& \qw 		& \qw 		& \ctrl{2}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{2}	& \qw		& \qw 		& \qw      & \ctrl{-1}	& \qw 		& \qw 		& \gate{\ket{0}}	& \qw 	& \targ{}	& \ctrl{1}	& \targ{  } & \qw 		& \qw 		& \qw & \rstick{$m_1$} \\
	%\lstick{$0$}  & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw 		& \qw 		& \qw  				& \qw 	& \targ{}	& \ctrl{1}	& \targ{  }	& \qw 		& \qw 		& \qw & \rstick{$0$} \\
	\lstick{$a_1$} & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw 		& \qw 		& \qw  				& \qw 	& \qw 		& \ctrl{1}	& \ctrl{-1}	& \qw 		& \qw 		& \qw & \rstick{$s_1$} \\
	\lstick{$b_1$} & \ctrl{-1} & \qw	   & \qw 		& \qw 		& \ctrl{2}	& \targ{}	& \ctrl{2}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \targ{}	& \ctrl{2}	& \qw 		& \qw      & \ctrl{-1}	& \qw 		& \qw 		& \gate{\ket{0}}	& \qw 	& \qw 		& \targ{}	& \ctrl{1}	& \targ{  }	& \qw 		& \qw & \rstick{$m_2$} \\
	%\lstick{$0$}  & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw 		& \qw 		& \qw  				& \qw 	& \qw 		& \targ{}	& \ctrl{1}	& \targ{  }	& \qw 		& \qw & \rstick{$0$} \\
	\lstick{$a_2$} & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw 		& \qw 		& \qw  				& \qw 	& \qw 		& \qw 		& \ctrl{1}	& \ctrl{-1}	& \qw 		& \qw & \rstick{$s_2$} \\
	\lstick{$b_2$} & \ctrl{-1} & \qw	   & \qw 		& \ctrl{2}	& \targ{}	& \qw 		& \targ{}	& \ctrl{2}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \targ{}	& \ctrl{2}	& \qw      & \ctrl{-1}	& \qw 		& \qw 		& \gate{\ket{0}}	& \qw 	& \qw 		& \qw 		& \targ{}	& \ctrl{1}	& \targ{  }	& \qw & \rstick{$m_3$} \\
	%\lstick{$0$}  & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw 		& \qw 		& \qw  				& \qw 	& \qw 		& \qw 		& \targ{}	& \ctrl{1}	& \targ{  }	& \qw & \rstick{$0$} \\
	\lstick{$a_3$} & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw  		& \qw  		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \targ{}	& \qw 		& \qw 		& \qw  				& \qw 	& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \ctrl{-1}	& \qw & \rstick{$s_3$} \\
	\lstick{$b_3$} & \ctrl{-1} & \qw	   & \ctrl{2}  	& \targ{}	& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{2}	& \qw  		& \qw  		& \ctrl{2}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{2} & \ctrl{-1}	& \qw 		& \qw 		& \gate{\ket{0}}	& \qw 	& \qw 		& \qw 		& \qw 		& \targ{}	& \targ{}	& \qw & \rstick{$m_4$} \\
	%\lstick{$0$}  & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw      & \qw		& \qw 		& \qw 		& \qw  				& \qw 	& \qw 		& \qw 		& \qw 		& \targ{}	& \targ{}	& \qw & \rstick{$0$} \\
	\lstick{$a_4$} & \targ{}   & \qw	   & \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}  & \targ{}  	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw      & \targ{}	& \targ{}	& \ctrl{-9}& \targ{}			& \qw 	& \qw		& \qw 		& \qw 		& \qw 		& \qw		& \qw & \rstick{$s_4$} \\		
	\lstick{$b_4$} & \ctrl{-1} & \ctrl{1}  & \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \ctrl{1}  & \ctrl{-1}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}  & \ctrl{-1}	& \qw	 	& \qw		& \gate{\ket{0}}	& \qw 	& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{\ket{0}} \\		
	\lstick{\ket{0}}& \qw      & \targ{}   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw 		& \targ{}  	& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw      & \qw 		& \targ{}	& \ctrl{-2}	& \targ{}			& \qw 	& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{-3}	& \qw & \rstick{$s_5$}
\end{quantikz}
}

\newcommand{\QMAsingleZero}{
\begin{quantikz} [row sep= 0.1cm, column sep= 0.05cm, transparent]
	\lstick{\ket{0}}& \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 		& \qw       & \qw		& \qw 		& \targ{}	& \qw  				& \qw 	& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw & \rstick{$m_0$} \\
	\lstick{$a_0$} & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \targ{  }	& \qw 		& \qw       & \qw		& \qw 		& \qw 		& \qw  				& \qw 	& \ctrl{1}	& \ctrl{-1}	& \qw 		& \qw 		& \qw 		& \qw & \rstick{$s_0$} \\
	\lstick{$b_0$} & \qw	   & \qw 	   & \qw 		& \qw 		& \qw 		& \ctrl{2}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \qw 		& \qw       & \qw		& \qw 		& \qw 		& \gate{\ket{0}}	& \qw 	& \targ{}	& \ctrl{1}	& \targ{  } & \qw 		& \qw 		& \qw & \rstick{$m_1$} \\
	\lstick{$a_1$} & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \targ{  }	& \qw       & \qw		& \qw 		& \qw 		& \qw  				& \qw 	& \qw 		& \ctrl{1}	& \ctrl{-1}	& \qw 		& \qw 		& \qw & \rstick{$s_1$} \\
	\lstick{$b_1$} & \ctrl{-1} & \qw	   & \qw 		& \qw 		& \ctrl{2}	& \targ{}	& \ctrl{2}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \targ{}	& \ctrl{2}	& \ctrl{-1}	& \qw       & \qw		& \qw 		& \qw 		& \gate{\ket{0}}	& \qw 	& \qw 		& \targ{}	& \ctrl{1}	& \targ{  }	& \qw 		& \qw & \rstick{$m_2$} \\
	\lstick{$a_2$} & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{  } & \qw		& \qw 		& \qw 		& \qw  				& \qw 	& \qw 		& \qw 		& \ctrl{1}	& \ctrl{-1}	& \qw 		& \qw & \rstick{$s_2$} \\
	\lstick{$b_2$} & \ctrl{-1} & \qw	   & \qw 		& \ctrl{2}	& \targ{}	& \qw 		& \targ{}	& \ctrl{2}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \targ{}	& \ctrl{2}	& \ctrl{-1} & \qw		& \qw 		& \qw 		& \gate{\ket{0}}	& \qw 	& \qw 		& \qw 		& \targ{}	& \ctrl{1}	& \targ{  }	& \qw & \rstick{$m_3$} \\
	\lstick{$a_3$} & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw  		& \qw  		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw       & \targ{}	& \qw 		& \qw 		& \qw  				& \qw 	& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \ctrl{-1}	& \qw & \rstick{$s_3$} \\
	\lstick{$b_3$} & \ctrl{-1} & \qw	   & \ctrl{2}  	& \targ{}	& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{2}	& \qw  		& \qw  		& \ctrl{2}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{2}  & \ctrl{-1}	& \qw 		& \qw 		& \gate{\ket{0}}	& \qw 	& \qw 		& \qw 		& \qw 		& \targ{}	& \targ{}	& \qw & \rstick{$m_4$} \\
	\lstick{$a_4$} & \targ{}   & \qw	   & \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}  & \targ{}  	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw       & \targ{}	& \targ{}	& \ctrl{-9} & \targ{}			& \qw 	& \qw		& \qw 		& \qw 		& \qw 		& \qw		& \qw & \rstick{$s_4$} \\		
	\lstick{$b_4$} & \ctrl{-1} & \ctrl{1}  & \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \ctrl{1}  & \ctrl{-1}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}   & \ctrl{-1}	& \qw	 	& \qw		& \gate{\ket{0}}	& \qw 	& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{\ket{0}} \\		
	\lstick{\ket{0}}& \qw      & \targ{}   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw 		& \targ{}  	& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw       & \qw 		& \targ{}	& \ctrl{-2}	& \targ{}			& \qw 	& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{-3}	& \qw & \rstick{$s_5$}
\end{quantikz}
}

\newcommand{\QMAdoubleZero}{
\begin{quantikz} [row sep= 0.1cm, column sep= 0.05cm, transparent]
	\lstick{\ket{0}}& \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \qw		& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw		& \qw 			& \qw       	& \qw			& \qw 			& \targ{}	& \qw  				& \qw 	& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw & \rstick{$m_0$} \\
	\lstick{$a_0$} & \qw	   & \qw	   & \qw		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \targ{  }	& \qw 			& \qw       	& \qw			& \qw 			& \qw 		& \qw  				& \qw 	& \ctrl{1}	& \ctrl{-1}	& \qw 		& \qw 		& \qw 		& \qw & \rstick{$s_0$} \\
	\lstick{$b_0$} & \qw	   & \qw 	   & \qw 		& \qw 		& \qw 		& \ctrl{2}	& \qw 		& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \gate{\ket{0}}& \qw       	& \qw			& \qw 			& \qw 		& \gate{\ket{0}}	& \qw 	& \targ{}	& \ctrl{1}	& \targ{  } & \qw 		& \qw 		& \qw & \rstick{$m_1$} \\
	\lstick{$a_1$} & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \targ{  }		& \qw       	& \qw			& \qw 			& \qw 		& \qw  				& \qw 	& \qw 		& \ctrl{1}	& \ctrl{-1}	& \qw 		& \qw 		& \qw & \rstick{$s_1$} \\
	\lstick{$b_1$} & \ctrl{-1} & \qw	   & \qw 		& \qw 		& \ctrl{2}	& \targ{}	& \ctrl{2}	& \qw 		& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \targ{}	& \ctrl{2}	& \ctrl{-1}		& \gate{\ket{0}}& \qw			& \qw 			& \qw 		& \gate{\ket{0}}	& \qw 	& \qw 		& \targ{}	& \ctrl{1}	& \targ{  }	& \qw 		& \qw & \rstick{$m_2$} \\
	\lstick{$a_2$} & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 			& \targ{  } 	& \qw			& \qw 			& \qw 		& \qw  				& \qw 	& \qw 		& \qw 		& \ctrl{1}	& \ctrl{-1}	& \qw 		& \qw & \rstick{$s_2$} \\
	\lstick{$b_2$} & \ctrl{-1} & \qw	   & \qw 		& \ctrl{2}	& \targ{}	& \qw 		& \targ{}	& \ctrl{2}	& \qw 		& \qw  		& \qw  		& \qw		& \qw 		& \ctrl{2}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \targ{}	& \ctrl{2}		& \ctrl{-1} 	& \gate{\ket{0}}& \qw 			& \qw 		& \gate{\ket{0}}	& \qw 	& \qw 		& \qw 		& \targ{}	& \ctrl{1}	& \targ{  }	& \qw & \rstick{$m_3$} \\
	\lstick{$a_3$} & \targ{}   & \qw	   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \qw  		& \qw  		& \ctrl{1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 			& \qw       	& \targ{}		& \qw 			& \qw 		& \qw  				& \qw 	& \qw 		& \qw 		& \qw 		& \ctrl{1}	& \ctrl{-1}	& \qw & \rstick{$s_3$} \\
	\lstick{$b_3$} & \ctrl{-1} & \qw	   & \ctrl{2}  	& \targ{}	& \qw 		& \qw 		& \qw 		& \targ{}	& \ctrl{2}	& \qw  		& \qw  		& \ctrl{2}	& \ctrl{-1}	& \targ{}	& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \targ{}		& \ctrl{2}  	& \ctrl{-1}		& \gate{\ket{0}}& \qw 		& \gate{\ket{0}}	& \qw 	& \qw 		& \qw 		& \qw 		& \targ{}	& \targ{}	& \qw & \rstick{$m_4$} \\
	\lstick{$a_4$} & \targ{}   & \qw	   & \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \ctrl{1}  & \targ{}  	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw			& \qw       	& \targ{}		& \targ{}		& \ctrl{-9} & \targ{}			& \qw 	& \qw		& \qw 		& \qw 		& \qw 		& \qw		& \qw & \rstick{$s_4$} \\		
	\lstick{$b_4$} & \ctrl{-1} & \ctrl{1}  & \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \targ{}	& \ctrl{1}  & \ctrl{-1}	& \targ{}	& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw		& \qw			& \targ{}   	& \ctrl{-1}		& \qw	 		& \qw		& \gate{\ket{0}}	& \qw 	& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw & \rstick{\ket{0}} \\		
	\lstick{\ket{0}}& \qw      & \targ{}   & \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw		& \qw 		& \targ{}  	& \qw  		& \qw		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 		& \qw 			& \qw       	& \qw 			& \targ{}		& \ctrl{-2}	& \targ{}			& \qw 	& \qw		& \qw 		& \qw 		& \qw 		& \ctrl{-3}	& \qw & \rstick{$s_5$}
\end{quantikz}
}

==> latex_images/xtalk_attacks.tex <==
\usepackage{tikz}
\usepackage{quantikz}
\usepackage{amsmath}

\newcommand{\rowSep}{0.25cm}
\newcommand{\colSep}{0.2cm}
\tikzset{slice/.append style={draw=blue}}
%\tikzset{slice/.append label style={blue}}

\newcommand{\myCnot}{
\begin{quantikz} [row sep= \rowSep, column sep= \colSep]
	\lstick{$a$} & \ctrl{1} & \qw & \rstick{$a$}\\
	\lstick{$b$} & \targ{}  & \qw & \rstick{$a \oplus b$}
\end{quantikz}
}

\newcommand{\mySwap}{
\begin{quantikz}
	\qw & \swap{1} & \qw \\
	\qw & \targX{} & \qw
\end{quantikz} = \begin{quantikz}
	\qw & \ctrl{1} & \targ{} 	& \ctrl{1} & \qw \\
	\qw & \targ{}  & \ctrl{-1} 	& \targ{}  & \qw
\end{quantikz}
}

\newcommand{\myToffoli}{
\begin{quantikz} [row sep= \rowSep, column sep= \colSep]
	\lstick{$a$} & \ctrl{1} & \qw & \rstick{$a$} \\
	\lstick{$b$} & \ctrl{1} & \qw & \rstick{$b$} \\
	\lstick{$c$} & \targ{}  & \qw & \rstick{$a \cdot b \oplus c$}
\end{quantikz}
}

\newcommand{\attackCNOT}{
	\begin{quantikz} [row sep= \rowSep, column sep= \colSep, transparent]
		\lstick{\ket{1}} & \ctrl{1} 	& \qw	\slice{n=1}   & \qw & \ctrl{1} 	& \qw	\slice{n=2}   & \qw & \ctrl{1} 	& \qw	\slice{n=3}   & \qw & \ctrl{1} 	& \qw	\slice{n=4}   & \qw & \ctrl{1} 	& \qw	\slice{n=5}   & \qw & \ctrl{1} 	& \qw	\slice{n=6}   & \qw & \ctrl{1} & \rstick{} \\
		\lstick{\ket{x}} & \targ{ } 	& \qw	              & \qw & \targ{ } 	& \qw	              & \qw & \targ{ } 	& \qw	              & \qw & \targ{ } 	& \qw	              & \qw & \targ{ } 	& \qw	              & \qw & \targ{ } 	& \qw	              & \qw & \targ{ } & \rstick{}
	\end{quantikz}
}

\newcommand{\attackCNOTtwo}{
	\begin{quantikz} [row sep= \rowSep, column sep= \colSep, transparent]
		\lstick{\ket{1}} & \ctrl{1} 	& \qw & \qw	\slice{n=1}   & \qw & \qw & \ctrl{1} 	& \qw & \qw	\slice{n=2}   & \qw & \ctrl{1} 	& \qw & \qw	\slice{n=3}   & \qw & \qw & \ctrl{1} 	& \qw & \qw	\slice{n=4} 	& \qw & \rstick{} \\
		\lstick{\ket{x}} & \targ{ } 	& \qw & \qw	              & \qw & \qw & \targ{ } 	& \qw & \qw	              & \qw & \targ{ } 	& \qw & \qw	              & \qw & \qw & \targ{ } 	& \qw & \qw	            	& \qw & \rstick{}
	\end{quantikz}
}


\newcommand{\attackAltCNOT}{
	\begin{quantikz} [row sep= \rowSep, column sep= \colSep, transparent]
		\lstick{\ket{1}} & \ctrl{1} 	& \targ{  } 	& \targ{} 	& \ctrl{1} 	& \qw	\slice{n=1}   & \qw & \qw{} 	& \targ{  }		& \qw	\slice{n=2}   & \qw & \targ{} 	& \ctrl{1} 	& \qw	\slice{n=3}   & \qw & \qw{} 	& \targ{  }  	& \qw	\slice{n=4}   & \qw & \rstick{} \\
		\lstick{\ket{x}} & \targ{ } 	& \ctrl{-1} 	& \qw    	& \targ{ } 	& \qw	              & \qw & \targ{} 	& \ctrl{-1}		& \qw	              & \qw & \qw    	& \targ{ } 	& \qw	              & \qw & \targ{} 	& \ctrl{-1} 	& \qw	              & \qw & \rstick{}
	\end{quantikz}
}

\newcommand{\attackSAC}{
	\begin{quantikz} [row sep= \rowSep, column sep= \colSep, transparent]
		\lstick{\ket{1}} & \gate{H} 	& \ctrl{1} 	& \targ{  } 	& \qw	\slice{n=1}   & \qw & \ctrl{1} 	& \targ{  } & \qw	\slice{n=2}   & \qw & \ctrl{1} 	& \targ{  } 	& \qw	\slice{n=3}   & \qw & \ctrl{1} 	& \targ{  } & \qw	\slice{n=4}   & \qw & \ctrl{1} 	& \targ{  }  & \qw	\slice{n=5}   & \qw 	 & \rstick{} \\
		\lstick{\ket{x}} & \gate{H} 	& \targ{ } 	& \ctrl{-1} 	& \qw	              & \qw & \targ{ } 	& \ctrl{-1} & \qw	              & \qw & \targ{ } 	& \ctrl{-1} 	& \qw	              & \qw & \targ{ } 	& \ctrl{-1} & \qw	              & \qw & \targ{ } 	& \ctrl{-1}  & \qw	              & \qw 	 & \rstick{}
	\end{quantikz}
}

\newcommand{\attackSACtwo}{
	\begin{quantikz} [row sep= \rowSep, column sep= \colSep, transparent]
		\lstick{\ket{1}} & \gate{H} 	& \ctrl{1} 	& \targ{  } 	& \qw	\slice{n=1}   & \qw & \ctrl{1} 	& \targ{  } & \qw	\slice{n=2}   & \qw & \ctrl{1} 	& \targ{  } 	& \qw	\slice{n=3}   & \qw & \ctrl{1} 	& \targ{  } & \qw	\slice{n=4} & \qw 	 & \rstick{} \\
		\lstick{\ket{x}} & \gate{H} 	& \targ{ } 	& \ctrl{-1} 	& \qw	              & \qw & \targ{ } 	& \ctrl{-1} & \qw	              & \qw & \targ{ } 	& \ctrl{-1} 	& \qw	              & \qw & \targ{ } 	& \ctrl{-1} & \qw	            & \qw 	 & \rstick{}
	\end{quantikz}
}

\newcommand{\attackAPC}{
	\begin{quantikz} [row sep= \rowSep, column sep= \colSep, transparent]
		\lstick{\ket{1}} & \gate{H} & \ctrl{1} 	& \gate{R\textsubscript{Y}(\pi)} 	& \ctrl{1} 						 & \qw	\slice{n=1}   & \qw & \targ{  } & \ctrl{1} 								& \gate{R\textsubscript{Z}(\pi)} 	& \qw	\slice{n = 2} & \qw & \ctrl{1} 	& \gate{R\textsubscript{Y}(\pi)}	& \ctrl{1} 						 & \qw	\slice{n = 3} & \qw 	& \rstick{} \\
		\lstick{\ket{x}} & \gate{H} & \targ{ } 	& \ctrl{-1} 						& \gate{R\textsubscript{Z}(\pi)} & \qw	              & \qw & \ctrl{-1} & \gate{R\textsubscript{Y}(\pi)} 	    & \ctrl{-1} 						& \qw	              & \qw & \targ{ } 	& \ctrl{-1} 						& \gate{R\textsubscript{Z}(\pi)} & \qw	              & \qw  	& \rstick{}
	\end{quantikz}
}

\newcommand{\attackAPCtwo}{
	\begin{quantikz} [row sep= \rowSep, column sep= \colSep, transparent]
		\lstick{\ket{1}} & \gate{H} & \ctrl{1} 	& \gate{R\textsubscript{Y}(\pi)} 	& \ctrl{1} 						 & \qw	\slice{n=1}   & \qw & \targ{  } & \ctrl{1} 								& \gate{R\textsubscript{Z}(\pi)} 	& \qw	\slice{n = 2} & \qw & \rstick{} \\
		\lstick{\ket{x}} & \gate{H} & \targ{ } 	& \ctrl{-1} 						& \gate{R\textsubscript{Z}(\pi)} & \qw	              & \qw & \ctrl{-1} & \gate{R\textsubscript{Y}(\pi)} 	    & \ctrl{-1} 						& \qw	              & \qw	& \rstick{}
	\end{quantikz}
}
